Multigrid Methods for the Computation of Propagators in Gauge Fields

NOTE: this is a shortened version of the abstract of the paper. Multigrid methods for propagators in gauge fields are investigated. Gauge fields are incorporated in algorithms in a covariant way. This avoids the necessity for gauge fixing in computations of propagators. The kernel $C$ of the restriction operator which averages from one grid to the next coarser grid is defined by projection on the ground- state of a local Hamiltonian. The idea behind this definition is that the appropriate notion of smoothness depends on the dynamics. The ground-state projection choice of $C$ is usable in arbitrary space-time dimension $d$ and for arbitrary gauge group. We discuss proper averaging operations for bosons and for staggered fermions. The averaging kernels $C$ can be used not only in deterministic multigrid computations, but also in multigrid Monte Carlo simulations, and for the definition of block spins and blocked gauge fields in Monte Carlo renormalization group studies of gauge theories. Actual numerical computations of kernels and propagators are performed in compact four-dimensional $SU(2)$ gauge fields. A central result of the present work is that {\em the multigrid method works in arbitrarily disordered gauge fields, in principle\/}.

==> 9212021.2 <==


 {}From now on we will write $\chi$ instead of $\phi$ when we explicitly
 deal with staggered fermion fields.
 {\em Let us first consider the free case.\/}
 Becher and Joos \cite{BecJoo} showed that the formal continuum limit
 of the staggered Dirac operator is equivalent to the
 Dirac-K\"ahler operator.
 The Dirac-K\"ahler equation is a differential geometric equation for
 continuum fermions.
 There Dirac fields are described by differential forms.
 For this reason the lattice discretization is straightforward.
 Joos and Schaefer \cite{JooSch} studied the symmetry group of staggered
 fermions in great detail, see also Ref.~\cite{Gol}.
 We call this group $\G_a$.
 Joos and Schaefer pointed out that $\G_a$ is a restriction of the
 continuum symmetry group of Dirac-K\"ahler fermions.
 We require that a blocking for staggered fermions is defined in such a
 way that as much as possible is preserved of the residual lattice
 symmetries.
 This means that the symmetry group $\G_{L_b a}$ on the staggered
 block lattice $\LLah$ should be a subgroup of~$\G_a$.

 The fine-to-coarse blocking step maps $\chi$ which lives on $\Lah$
 onto a field $\bfchi$ on the block lattice $\LLah$ of lattice spacing
 $L_b a/2$, with an integer scale factor $L_b > 1$:
%------------------- equation ------------------------------------------
 \begin{equation}
   \bfchi ( x ) = \int_{z\in\Lah} C(x,z)\,\chi(z) \esp
 \label{BSchi}
 \end{equation}
%------------------- equation ------------------------------------------
 The adjoint spinor $\bar{\chi}(z)$ is an independent Grassmannian
 integration variable.
 Its block spin can be defined by
%------------------- equation ------------------------------------------
 \begin{equation}
   \bar{\bfchi} ( x ) = \int_{z\in\Lah} \bar{\chi}(z) \Cstar(z,x) \esk
 \label{BSbarchi}
 \end{equation}
%------------------- equation ------------------------------------------
 where $\Cstar (z,x)$ is the adjoint of the kernel $C$ which appears
 in \equ{BSchi}.
 This does not contradict the statement of G. Mai in Ref.~\cite{Mai}
 that one needs different blocking procedures for adjoints.
 She considered blockings from the continuum to the lattice.
 The subtlety which she encountered is hidden in the fact that
 pseudoflavor $H$ for $\chi$ and for $\bar{\chi}$ does not have
 the same physical meaning in terms of spin and flavor.

%..............
 \Subsubsection{Emergence of odd $\L$}
%..............
 The first result which we derive from symmetry considerations is
 that {\em $L_b$ must be odd\/}, i.~e.\ $L_b = 3 , 5 , \ldots$, but
 {\em not\/} $L_b = 2$.
 This results arises as follows.
 On the lattice translations by integer multiples $\vec{n}a$ of $a$
 (not $a/2$) survive as true translation symmetries.
 Pure flavor transformations do not survive as symmetries at all.
 What survives are certain combinations $\epsilon d^H$ of flavor
 transformations and translations by $\frac{1}{2}e_H$, where $\epsilon
 = \pm 1$.
 We call them pseudoflavor transformations.
 The square $(d^H)^2 $ of any such transformation is a true lattice
 translation by $-e_H$.
 To keep track of the dependence on the lattice spacing, we write
 $T_a(\ast)$ for the action of an element $\ast$ of $\G_a$.
 The action of translations is the obvious one.
 In particular, translations by the vectors $e_H$ in $\Lambda_a$ act as
%------------------- equation ------------------------------------------
  \begin{equation}
    (T_a (e_H)\,\chi)(z) = \chi(z-e_H)  \esp
  \label{Translation}
  \end{equation}
%------------------- equation ------------------------------------------
 Pseudoflavor transformations $\epsilon d^H$ act on the staggered
 fermion field as
%------------------- equation ------------------------------------------
  \begin{equation}
   (T_a(\epsilon d^K)\,\chi)(z) =
     \epsilon\,\check{\rho}_{H,K}\,\chi (z + \txeh e_K) \esk\quad
       \mbox{if $z \in \Lambda_a^H$}\esp
  \label{PFtransformation}
  \end{equation}
%------------------- equation ------------------------------------------
 $\check{\rho}_{H,K}$ is a sign factor which is the same as that which
 appears in the Clifford product $\vee$ of forms, defined by
 $dx^{\mu} \vee dx^{\nu} = dx^{\mu} \wedge dx^{\nu} + \delta^{\mu\nu}$,
 and
%------------------- equation ------------------------------------------
  \begin{equation}
   dx^H \vee dx^K = \check{\rho}_{H,K} \ dx^{H \triangle K} \esp
  \label{SignFactor}
  \end{equation}
%------------------- equation ------------------------------------------
 $H \triangle K$ denotes the symmetric difference $H \triangle K =
 (H\cup K) \setminus (H\cap K)$, and
 $dx^H = dx^{\mu_1} \wedge \cdots \wedge dx^{\mu_h}$.
 The sign factors $\etamu$ in the Diracian \equ{Dirac} are special
 $\check{\rho}$-factors:
 $\etamu (z) = \check{\rho}_{H,K}$ for $z\in\Lambda_a^K$ and
 $H=\{\mu\}$.

 In the following, primed quantities refer to the block lattice.
 We write $e_{\mu}^{\prime}$ for the lattice vectors of length $L_b a$
 in $\LLa$, and similarly for $e_H^{\prime}$, etc.
 Thus,
%------------------- equation ------------------------------------------
  \begin{equation}
   e_H^{\prime} = L_b\,e_H  \esp
  \label{BVcoarse}
  \end{equation}
%------------------- equation ------------------------------------------
 The elementary pseudoflavor transformations $d^{\prime\,K}$ on $\LLah$
 must be linear combinations of pseudoflavor transformations $d^K$ and
 translations $e$ on $\Lah$.
 {}From~\equ{PFtransformation}, it can be seen that $d^{\prime\,K}$
 contains an admixture of translation by $-\txeh e_K^{\prime}$.
 Since $d^K$ contains an admixture of a translation by $\txeh e_K$,
 we must have
%------------------- equation ------------------------------------------
  \begin{equation}
   -\frac{1}{2} e^{\prime}_K = -\frac{1}{2} e_H + e  \quad\mbox{with}
    \quad e = \sum_{\mu} n_{\mu} e_{\mu}\esk n_{\mu}\in\bbbn
  \label{ReasonOddL}
  \end{equation}
%------------------- equation ------------------------------------------
 for some $H$.
 Because of \equ{BVcoarse}, this is only possible if $H=K$, and
 $e=\txeh (L_b - 1) e_K$.
 This requires that $L_b$ is odd,
%------------------- equation ------------------------------------------
  \begin{equation}
     \L = 3,5,\ldots
  \label{oddL}
  \end{equation}
%------------------- equation ------------------------------------------
 The result \equ{oddL} might have been expected, since only for odd
 $L_b$ the pseudoflavors on the fine lattice $\Lah$ and on the block
 lattice $\LLah$ match nicely when we regard $\LLah$ as a sublattice of
 $\Lah$. (See Fig.~\NextFig\ below).

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 \SubSubsection{The Averaging Kernel $C(x,z)$ in Trivial Gauge Fields}
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 Now we turn to the averaging kernel $C(x,z)$ for free staggered
 fermions.
 Since the blocking should be consistent with the symmetries, we
 require that $C$ commutes with the action of the surviving symmetries
 on the block lattice.
 For translations and pseudoflavor transformations this means
%------------------- equation ------------------------------------------
  \begin{eqnarray}
    T_{L_b a}(e^{\prime}_K)\ C & = & C \  T_a(L_b e_K) \esk
  \label{CommutivityT} \\
  & & \nonumber\\
    T_{L_b a}(\epsilon d^{\prime\,K}) \ C & = & C\ T_a(\epsilon d^K)
                                 \  T_a(\txeh (L_b - 1)\,e_K)\esp
  \label{CommutivityPFT}
  \end{eqnarray}
%------------------- equation ------------------------------------------
 Eqs.~\equ{CommutivityT} and~\equ{CommutivityPFT} are fulfilled if
 $C$ is translation invariant,
%------------------- equation ------------------------------------------
 \begin{equation}
   C( x + e_H^{\prime}\,,\,z + L_b e_H) = C(x,z)\esk
 \label{TranslInv}
 \end{equation}
%------------------- equation ------------------------------------------
 and if in addition $C$ has the support property
%------------------- equation ------------------------------------------
 \begin{equation}
   C(x,z) = 0
   \quad\mbox{unless $x$ and $z$ carry the same pseudoflavor.}
 \label{SupportC}
 \end{equation}
%------------------- equation ------------------------------------------
 In words, the support property states the following.
 If $x\in\LLa^H$\,, then the staggered block spin $\bfchi(x)$ is a
 weighted sum of fields $\chi(z)$ at sites with the same pseudoflavor
 $H$.
 Blockings with such a property were also considered by Ben-Av et al.\
 \cite{BenBraSol,HaretalLAT90,Benetal,Benthesis,PTMG_GMD,LauWit}.
 However, they chose a scale factor $L_b=2$, and this forces them to
 treat different pseudoflavors on different footings.
 Another blocking procedure with non-overlapping blocks was used by
 Hulsebos et al.\ \cite{HSVLAT90,HSVNP,HSVJulich,Vin,VinLAT91}.
 But in their proposal one does not retain the successful pure gauge
 limit.

%..............
 \Subsubsection{Blocking procedure for staggered fermions}
%..............
 The blocking procedure which is consistent with the symmetries of
 free staggered fermions is as follows.
 With each site $x$ of the block lattice $\Lambda_{L_b a/2}$ we
 associate a hypercube $X \subset \Lambda_{a/2}$ of sidelength
 $L_b a$, that is $2 L_b$ lattice spacings $a/2$.
 When considered as a site in $\Lambda_{a/2}$, $x$ will be the point
 in the center of this hypercube.
 These hypercubes $X$ overlap.
 If $x\in \Lambda^H_{L_b a}$ then we call $z \in X$ an active site if
 $z\in \Lambda^H_{a}$, i.\ e.\ if it carries the same pseudoflavor as
 the central point $x$ of the hypercube $X$.
 Every point $z$ in $\Lambda_{a/2}$ is active site in exactly
 one hypercube $X$.
 Every hypercube $X$ contains $L_b^d$ active sites.
 Our choice of blocks is illustrated in Fig.~\NextFig.
%#######################################################################
%  BEGIN   ---      PICTURE  BLOCKING FOR STAGGERED FERMIONS
%#######################################################################
 \setlength{\unitlength}{1.0mm}
 \begin{figure}
 \begin{minipage}{16.5 cm}{}
 \begin{center}
 \begin{picture}(115,115)(10.0,10.0)
 \multiput(10,10)(16,0){8}{\Huge$\bullet$}
 \multiput(18,10)(16,0){7}{\Huge$\circ$}
 \multiput(10,18)(16,0){8}{\Huge$\diamond$}
 \multiput(18,18)(16,0){7}{\Huge$\ast$}
 \multiput(10,26)(16,0){8}{\Huge$\bullet$}
 \multiput(18,26)(16,0){7}{\Huge$\circ$}
 \multiput(10,34)(16,0){8}{\Huge$\diamond$}
 \multiput(18,34)(16,0){7}{\Huge$\ast$}
 \multiput(10,42)(16,0){8}{\Huge$\bullet$}
 \multiput(18,42)(16,0){7}{\Huge$\circ$}
 \multiput(10,50)(16,0){8}{\Huge$\diamond$}
 \multiput(18,50)(16,0){7}{\Huge$\ast$}
 \multiput(10,58)(16,0){8}{\Huge$\bullet$}
 \multiput(18,58)(16,0){7}{\Huge$\circ$}
 \multiput(10,66)(16,0){8}{\Huge$\diamond$}
 \multiput(18,66)(16,0){7}{\Huge$\ast$}
 \multiput(10,74)(16,0){8}{\Huge$\bullet$}
 \multiput(18,74)(16,0){7}{\Huge$\circ$}
 \multiput(10,82)(16,0){8}{\Huge$\diamond$}
 \multiput(18,82)(16,0){7}{\Huge$\ast$}
 \multiput(10,90)(16,0){8}{\Huge$\bullet$}
 \multiput(18,90)(16,0){7}{\Huge$\circ$}
 \multiput(10,98)(16,0){8}{\Huge$\diamond$}
 \multiput(18,98)(16,0){7}{\Huge$\ast$}
 \multiput(10,106)(16,0){8}{\Huge$\bullet$}
 \multiput(18,106)(16,0){7}{\Huge$\circ$}
 \multiput(10,114)(16,0){8}{\Huge$\diamond$}
 \multiput(18,114)(16,0){7}{\Huge$\ast$}
 \multiput(10,122)(16,0){8}{\Huge$\bullet$}
 \multiput(18,122)(16,0){7}{\Huge$\circ$}
%.......................................
 \thicklines
 \multiput(19.75,19.95)(24,0){5}{\circle{6}}
 \multiput(19.75,43.95)(24,0){5}{\circle{6}}
 \multiput(19.75,67.95)(24,0){5}{\circle{6}}
 \multiput(19.75,91.95)(24,0){5}{\circle{6}}
 \multiput(19.75,115.95)(24,0){5}{\circle{6}}
 \put(24.5,24.5){\framebox(38,38){\mbox}}
 \put(24.5,72.5){\framebox(38,38){\mbox}}
 \put(72.5,24.5){\framebox(38,38){\mbox}}
 \put(72.5,72.5){\framebox(38,38){\mbox}}
 \put(48.5,23.5){\dashbox{0.7}(38,40){\mbox}}
 \put(48.5,71.5){\dashbox{0.7}(38,40){\mbox}}
 \thinlines
 \put(47.0,48.5){\framebox(41,38){\mbox}}
%.......................................
 \end{picture}
 \end{center}
 \end{minipage}
 \caption{{\protect\small{\em
          The good choice of blocks to average over in a two-dimensional
          pseudoflavor lattice.
          This blocking leads to staggered fermions on the coarse
          lattice again.
          Block centers $\hat{x}$ are encircled (for $L_b = 3$).
          The boundaries of seven blocks are marked.
          The averaging kernel $C(x,z)$ for free staggered fermions
          (and in nontrivial gauge fields for the ``Laplacian choice'';
          see below) is only nonvanishing if site~$z$ has the same
          pseudoflavor (symbol) as the block center~$\hat{x}$.
          Therefore the seemingly overlapping blocks have actually
          no sites in common in these cases.}}}
 \end{figure}
%#######################################################################
%    END   ---      PICTURE  BLOCKING FOR STAGGERED FERMIONS
%#######################################################################
 The block boundaries in Fig.~\PreviousFig\ may be shifted away from
 the block centers by $a/2$ without any effect.
 Doing so would result in an agreement with the hypercubes $X$
 discussed above, but the figure were harder to read.

 It is necessary to admit overlapping blocks $x$ if one insists
 that $\chi (z)$ makes a contribution to some block spin $\bfchi (x)$
 for any $z$, i.\ e.\ in order that every $z$ is active site of some
 block (no decimation).

%..............
 \Subsubsection{``Piecewise-constant'' kernels for free
                staggered fermions}
%..............
 If $x\in\LLa^H$ then we set
%------------------- equation ------------------------------------------
 \begin{equation}
   C (x,z) =  \left\{ \begin{array}{cl}
  (L_b a/2)^{-d} \cdot 1 & \quad \mbox{if $z \in x\cap\Lambda_a^H$}\esk
                                                            \\
     0                 & \quad \mbox{otherwise}\esp \end{array} \right.
 \label{CwithoutGFSF}
 \end{equation}
%------------------- equation ------------------------------------------
 $C(x,z)$ is only nonvanishing on active sites $z$ of hypercube $X$,
 so that it has disjoint support in $z$ for different $x$.
 Conditions \equ{TranslInv} and \equ{SupportC} are fulfilled.

 We remark that from the point of view of computation of propagators,
 the equation $(-\Dirac^2 + m^2)\,\chi = f$ is in the absence of gauge
 fields equivalent to computing $2^d$ uncoupled free bosonic
 propagators, one for each pseudoflavor.
 The choice \equ{CwithoutGFSF} is the natural fermionic analog to
 the bosonic choice \equ{CwithoutGF}.

 A variant of the blocking procedure described above was first
 introduced by G.\,Mai \cite{Mai}.
 She considered blocking from the continuum to a lattice.

%..............
 \Subsubsection{Eigenvalue equation for $C$ and Neumann \bc
                for staggered fermions}
%..............
 The kernel \equ{CwithoutGFSF} can also be defined as solution of an
 eigenvalue equation, analogously to Eq.~\equ{EVequationC},
%------------------- equation ------------------------------------------
  \begin{equation}
  ( -\LAPN \Cstar ) ( z , x )  = \lambdanull\,\Cstar (z,x) \esk
  \label{EVequationCSF}
  \end{equation}
%------------------- equation ------------------------------------------
 where $\lambdanull$ is again the lowest eigenvalue of $-\LAPN$.
 However, the choice for the fermionic analog of the bosonic $\LAPN$
 has to be made with some care.
 In the absence of gauge fields the square of the Diracian \equ{Dirac}
 equals a Laplacian (as in the continuum),
%------------------- equation ------------------------------------------
 \begin{equation}
   (\Delta \chi )(z) = \frac{1}{a^2}
   \sum_{\stackrel{{\scriptstyle \mu = -d}}{\mu\neq 0}}^d
              \left[ \chi ( z + \emu ) - \chi (z) \right] \esp
 \label{SFlaplacian}
 \end{equation}
%------------------- equation ------------------------------------------
 This $\Delta$ couples only sites $z$ with the same pseudoflavor.
 The kernel \equ{CwithoutGFSF} satisfies Eq.~\equ{EVequationCSF} if we
 choose the Laplacian \equ{SFlaplacian}, and if we define Neumann
 boundary conditions as follows.
 If $x\in\LLa^H$, then $\LAPN$ is defined by the same formula
 \equ{SFlaplacian} as $\Delta$, except that those terms in the sum
 are omitted where $z$ and $z+\emu$ are both in $\Lambda_a^H$, but one
 is in block~$x$ and the other one is outside~$x$\@.
 (Cf.\ the discussion in Sec.~\ref{SecGSP}.)
 We also have to impose the subsidiary condition $C(x,z)=0$ if
 $z\not\in x$, and the normalization condition $C\Cstar=\bbbone$.

 \smallskip
 So far we have imposed the requirement \equ{SupportC} as a separate
 condition.
 However, this condition could also be regarded as a consequence of the
 eigenvalue equation.
 If we restrict attention to sublattices $\Lambda_a^K$ with $K\neq H$,
 then the modification of $\Delta$ through ``Neumann boundary
 conditions'' as stated above becomes inoperative, and the only solution
 of the eigenvalue equation \equ{EVequationCSF} which vanishes
 outside $x$ is $C(z,x)=0$.
 This way of specifying the solution amounts to supplementing the
 Neumann boundary conditions on $\Lambda_a^H$ by Dirichlet boundary
 conditions on $\Lambda_a^K$\,,$K\neq H$.

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 \SubSubsection{The Averaging Kernel $C(x,z)$ in Nontrivial Gauge
                Fields}
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 We have to discuss now what happens when gauge fields are included.

%..............
 \Subsubsection{Square of the covariant Dirac operator}
%..............
 In this case the square of the Diracian is no longer just a
 Laplacian, but instead
%------------------- equation ------------------------------------------
 \begin{equation}
   (-\Dirac^2 \chi )(z) = \left( [-\Delta - \sum_{|\mu |\neq |\nu |}
    \sigma_{\mu\nu} (z) F_{\mu\nu}^{\ast} (z) ] \chi\right) (z) \esp
 \label{DiracSquared}
 \end{equation}
%------------------- equation ------------------------------------------
 Indices $\mu$, $\nu$ are summed over positive and negative values, but
 $| \mu | \neq |\nu |$.
 The gauge covariant Laplacian for staggered fermions is given by
%------------------- equation ------------------------------------------
 \begin{equation}
   (\Delta \chi )(z) = \frac{1}{a^2}
   \sum_{\stackrel{{\scriptstyle \mu = -d}}{\mu\neq 0}}^d
   \left[ U(z,2\mu )\,\chi ( z + \emu ) - U(z,\pm\mu )\,\chi (z) \right]
   \esk
 \label{SFcovLaplacian}
 \end{equation}
%------------------- equation ------------------------------------------
 where $U(z,2\mu ) \equiv U(z,z+\txeh\emu )\,U(z+\txeh\emu , z+\emu )$
 and $U(z,\pm\mu ) \equiv U(z,z+\txeh\emu )\,U(z+\txeh\emu , z)$.
 The ``forward-backward'' parallel transport $U(z,\pm\mu )$ equals
 $\bbbone$ for ordinary gauge fields, but this is not true when one
 admits dielectric gauge fields.
 \newline
 $F_{\mu\nu}$ in Eq.~\equ{DiracSquared} is the natural definition of the
 field strength on the lattice \cite{MacDLGT},
%------------------- equation ------------------------------------------
 \begin{eqnarray}
  a^2 F_{\mu\nu} (z) & = &
             \ \   U(z + \txeh \emu + \txeh \enu\,,\,z + \txeh \emu )\,%
                   U(z + \txeh \emu\,,\,z )\nonumber\\
     & &         - U(z + \txeh \emu + \txeh \enu\,,\,z + \txeh \enu )\,%
                   U(z + \txeh \enu\,,\,z ) \esp
 \label{Fmunu}
 \end{eqnarray}
%------------------- equation ------------------------------------------
 $\sigma_{\mu\nu}$ is a commutator of $\eta$-factors.

 Eq.~\equ{DiracSquared} is the lattice analog of the continuum
 equation $-\Dirac^2 = -D_{\mu}^2 - \txeh g \sigma_{\mu\nu}F_{\mu\nu}$
 with the usual definition of the covariant derivative $D_{\mu} =
 \partial_{\mu} + i g A_{\mu}$ and the Yang-Mills field strength
 $F_{\mu\nu} = [ D_{\mu} , D_{\nu} ] / (ig)$, and $\sigma_{\mu\nu} =
 \txeh i [ \gamma_{\mu} , \gamma_{\nu} ]$.

%..............
 \Subsubsection{The Laplacian choice of $C(x,z)$}
%..............
 For nonvanishing field strength (i.\ e.\ nontrivial gauge fields)
 it remains true that $\Delta$ couples only sites with the
 same pseudoflavor, but the same is not true of $\Dirac^2$.
 One possible generalization of \equ{EVequationCSF} is now as follows.
 If we insist in retaining the support property \equ{SupportC} for the
 averaging kernel $C$, we could simply replace \equ{SFlaplacian}
 by the covariant Laplacian \equ{SFcovLaplacian}.
 We call this the ``Laplacian choice of $C$''.
 [$-\LAPN$ is a positive semidefinite operator, considered as acting on
 functions which vanish on sites $z \not\in \Lambda_a^H$ when $x \in
 \LLa^H$.]
 In order make the definition of $C$ unique and gauge covariant, we
 have also to impose the normalization condition $C \Cstar = \bbbone$
 and the covariance condition \equ{CovarianceCondition}.

 The kernel $C$ of the Laplacian choice can be computed numerically
 with the same efficiency as the averaging kernel \equ{EVequationC}
 for bosons (see Sec.~\ref{SecAlgorithmC}).
 One can also use the same computer program, the only changes which
 have to be made are replacements of address lists and of parallel
 transporters in the Laplacian.
 In Sec.~\ref{SecOptA} we will see that the Laplacian choice of $C$
 defines a good block spin in the sense described in the previous
 section.
 Probability distributions of $\normC$ in four-dimensional $SU(2)$ gauge
 fields are shown in Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{8.0cm}
        {Averaging kernel $C$ of the Laplacian choice for staggered
         fermions:
         Probability distributions of the dimensionless quantity
         $(L_b a/2)^d\,\normC$\,, $z\!\in\!x\cap\Lah^H$ for $x\in
         \Lah^H$, in four-di\-men\-sion\-al pure $SU(2)$ gauge theory.
         The norm equals $\normC = [ \frac{1}{2} \Tr C(x,z)^{\dagger}
         C(x,z) ]^{1/2}$.
         The four curves shown correspond to $\beta = 10.0$, $5.0$,
         $3.0$, $2.7$, with increasing width.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%..............
 \Subsubsection{The Diracian choice of $C(x,z)$}
%..............
 The authors of Ref.~\cite{HaretalLAT90} make the statement that it
 is compulsory for the averaging map~$C$ to have the support property
 \equ{SupportC} also in the presence of gauge fields.
 We do not agree with this.
 As an alternative to the above scheme one could think of using the
 square of the Dirac operator in place of the Laplacian in the
 eigenvalue equation \equ{EVequationCSF}.
 This may seem more natural and is closer to the philosophy of
 ground-state projection MG, but it leads to a much greater
 computational complexity and storage space requirements.
 Let us discuss these points in more detail.

 We may define $\Dirac_{N,x}\chi(z)$ for $z\in x$ by \equ{Dirac} with
 with the modification that those terms in the sum over $\mu$ are
 omitted for which $z \pm\txeh \emu$ are  both in $\Lambda_a^H$, but one
 is in block $x$ while the other is not in $x$.
 Setting
%------------------- equation ------------------------------------------
 \begin{equation}
     -\Dirac_{N,x}^2 = \Dirac_{N,x}^{\ast} \Dirac_{N,x} \esk
 \label{DiracN}
 \end{equation}
%------------------- equation ------------------------------------------
 one finds that $-\Dirac_{N,x}^2 \chi (z)$ agrees with $-\LAPN \chi (z)$
 for $z\in  \Lambda_a^H$ when $F_{\mu\nu}(z) = 0$.
 We might require that the averaging kernel $C$ is a solution of the
 eigenvalue equation \equ{EVequationCSF} with $-\Dirac_{N,x}^2$
 substituted for $-\LAPN$.
 But the square of the Dirac operator couples sites with different
 pseudoflavors.
 Therefore it is in general not consistent with the eigenvalue equation
 to require the support property \equ{SupportC}.
 Instead we should supplement the boundary conditions.
 The requirement that $C(x,z) $ should vanish for sites outside $x$
 but not in $\Lambda_a^H$ can be built into the eigenvalue equation as
 an additional boundary condition by setting
%------------------- equation ------------------------------------------
 \begin{equation}
   \Dirac_{N,D,x}^2 = \Theta_x \Dirac_{N,x}^2 \Theta_x \esk
 \label{DiracND}
 \end{equation}
%------------------- equation ------------------------------------------
 where $\Theta_x \chi (z) = \chi (z)$ if $z \in x \cup \Lambda_a^H$,
 and $=0$ otherwise.

 The eigenvalue equation becomes
%------------------- equation ------------------------------------------
 \begin{equation}
   (-\Dirac_{N,D,x}^2 \Cstar )(z,x) = \lambdanull\,\Cstar (z,x) \esk
 \label{EVequationCDirac}
 \end{equation}
%------------------- equation ------------------------------------------
 where $\lambdanull$ is the lowest eigenvalue of the positive
 semidefinite operator $-\Dirac_{N,D,x}^2$ (considered as acting on
 functions which vanish on odd sites $z$ if $x$ is odd and on even sites
 otherwise).
 We call this the ``Diracian choice of $C$''.

 We seek solutions which vanish outside $x$.
 In general the solution will not vanish when $x$ and $z$ carry
 different pseudoflavor.
 In the presence of a gauge field, the Dirac operator is no longer
 translation invariant.
 Since pseudoflavor transformations contain an admixture of
 translations, it is also not invariant under pseudoflavor
 transformations.
 For this reason we cannot rely on symmetry to rule out the
 possibility that Eq.~\equ{SupportC} is violated.
 If we call $z$ an active site of block $x$ when $C(x,z) \neq 0$,
 then it is no longer true that any site $z$ is an active site
 of exactly one block.
 In this sense, the blocks will overlap in a nontrivial way.
 In numerical applications to MG computations of nearly massless
 propagators for staggered fermions in a gauge field $U$ this leads to
 a great increase in computational complexity and in storage space
 requirements.

 The overlap problem could be ameliorated, but not eliminated
 completely, by introducing non-overlapping blocks $[x]$ and
 requiring that $C(x,z)$ vanishes outside $[x]$ when $z \not\in
 \Lambda_a^H$.
 This is implemented by redefining $\Theta_x$ in Eq.~\equ{DiracND}:
 $\Theta_x \chi (z) = \chi (z)$ for $z\in [x] \cup \Lambda_a^H$, and
 $=0$ otherwise.
 The redefinition amounts to imposing Neumann boundary conditions
 on larger blocks $x$ in $\LLa^H$ and Dirichlet boundary conditions on
 smaller blocks $[x]$ in $\LLa^K$, $K\neq H$.
 (Remember that $H$ is fixed by $x$).
 Proceeding in this way, the old solution for $C$ is retained in
 the limit of a pure gauge, and therefore the blocking is
 consistent with the symmetries in the limit of a pure gauge.

 The maximal non-overlapping hypercubes $[x]$ are given by%
 \footnote{$\|\cdot\|_{\infty}$ denotes the Chebyshev norm, as usual,
           i.\ e.\ ${\d\| w \|_{\infty} = \max_{\mu} | w_{\mu} |}$.}
 $z \in [x]$ if $\| z - [\hat{x}] \|_{\infty} \leq \txeh (L_b -1)\txah$.
 The overlap problem is eliminated if we choose $[x]=\emptyset$ instead.
 But this leads back to the Laplacian form of the eigenvalue
 equation which was considered before.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Blocked Gauge Fields
 \label{SecUblock}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Gauge Covariant Block Spins}}
          {{\rm\thesubsection.}\ {\sl Blocked Gauge Fields}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl It is proposed to define blocked gauge fields by using
      interpolation or averaging kernels for matter fields.
      The blocked gauge fields are of ``dielectric'' type, but they
      may be brought back into the gauge group by performing a
      polar decomposition \cite{MacDLGT}.}
 \smallskip

 Remember that the kernels of the Laplacian and of the Dirac operator,
 Eqs.~\equ{LaplaceKernel} and \equ{DiracKernel}, contain the lattice
 gauge field $U$.
 A block spin definition for matter fields gives us the effective
 operators on coarser layers, $\Delta_{\subs{eff}} = \A^* \Delta \A$ and
 $\Dirac_{\subs{eff}} = \A^* \Dirac \A$.
 Given $\Delta_{\subs{eff}}$ or $\Dirac_{\subs{eff}}$\,, we have
 candidates for gauge fields $\U$ on the block lattice,
%------------------- equation ------------------------------------------
 \begin{eqnarray}
  & \U (x,y) = & (L_b a)^{d+2}\Delta_{\subs{eff}}(x,y)\quad
                \mbox{for $x,y$ nearest neighbors,} \nonumber\\
  & & \label{Ublock} \\
  \mbox{and} &
  \U (x,y) =  & (L_b a)^{d+1} \Dirac_{\subs{eff}}(x,y)\,/\,\eta_{\mu}(x)
                \quad \mbox{if $y=x + L_b \txeh e_{\mu}$} \esk\nonumber
 \end{eqnarray}
%------------------- equation ------------------------------------------
 respectively.
 These expressions for $\U (x,y)$ have the correct gauge covariance
 property.

 We add some comments on the Dirac case.
 Since we use odd $L_b$\,, the staggered block lattice can be regarded
 as a sublattice of $\Lah$ in which the pseudoflavor of a site does
 not depend on whether we regard it as a site of the fundamental or
 the block lattice, and the same is true of its property of being even
 or odd.
 The kernel $\A$ will always have the property that $\A (z,x)=0$ unless
 $z$ and $x$ are both even or both odd.
 Therefore $\Dirac_{eff}$ connects even to odd sites.
 The factor $\eta_{\mu}(x)^{-1}$ can be regarded as defined by
 regarding $x$ as a point in a sublattice of the fundamental lattice.
 This agrees with the natural definition on the block lattice.
 Note also that  $\eta_{\mu}(z)$ is independent of the $\mu$-component
 $z_{\mu}$ of $z$.

 \smallskip
 If one makes the variational choice $\A = \Cstar$, the above
 definition of $\U$, for instance for gauge fields interacting with
 bosons, reads explicitly:
%------------------- equation ------------------------------------------
 \begin{equation}
   \U (x,y ) = L_b^{-d} \sum_{(z,z'): z\in x, z'\in y}
               C(x,z)\,U(z,z')\,C(y,z')^{\dagger} \esp
 \label{UDeltaEff}
 \end{equation}
%------------------- equation ------------------------------------------
 Summation is over those links $(z,z')$ where $z$ is in block $x$
 and $z'$ is in the neighboring block $y$.
 (These are the ``thin'' links in
  Fig.~\theSecBlockBose.\theFigBlockBose.)

 \smallskip
 The blocked gauge fields $\U (x,y)$ are actually ``dielectric'' gauge
 fields~\cite{MacDLGT}.
 In case of gauge group $SU(2)$ they are equal to an $SU(2)$ lattice
 gauge field multiplied with a fluctuating positive real factor
 (``fluctuating length'').
 [In renormalization group studies the occurrence of blocked fields
  which are not of the same kind as those in the original theory
  is not uncommon \cite{MacRGandME,MacCargese}.]
 The dielectric gauge fields may be brought back into the gauge group
 by multiplying with a positive real number (for $U(1)$ and $SU(2)$)
 or with a positive matrix (for $U(N), N> 2$).

 \smallskip
 A different choice of block spin for gauge fields was introduced
 by Ba{\l}aban and used in rigorous renormalization group work
 \cite{BalProp,BalLGT}, see also \cite{BalJaf}, and \cite{GliJaf}.%
 \footnote{Readers (including the present author) who find Ba{\l}aban's
           works hard to read, may seek comfort in A.S.\,Wightman's
           words in Ref.~\cite{Wig}.
           An easier-to-read introduction to constructive gauge
           theories are Imbrie's Les Houches lectures \cite{Imb}.
           There is also a recent text book on constructive field
           theory by Rivasseau \cite{Riv}.}

 Another possible definition of dielectric block spins for gauge
 fields, which is similar to Ba{\l}aban's choice, involves $C$ and is as
 follows.
%------------------- equation ------------------------------------------
 \begin{equation}
  \U (x + L_b \emu , x) = (L_b a )^d \int_{z \in x}
   C ( x + L_b \emu\,,\,z + L_b \emu )\,%
   U ( z + L_b \emu , z)\,C(x,z)^{\dagger}\esk
 \label{BSBal}
 \end{equation}
%------------------- equation ------------------------------------------
 where $U ( z + L_b \emu , z)$ denotes the path-ordered product of link
 variables along the straight line from $z$ to $z + L \emu$.
 Actually, Eq.~\equ{BSBal} defines a blocked gauge field interacting
 with bosons.
 In case of $U$ coupled to staggered fermions, one has to replace
 $\emu$ by $\txeh\emu$ (of course).

 Finally, we note that the definitions given in this section for
 blocked gauge fields have the property that a pure gauge $U$ on the
 finer lattice is mapped onto a pure gauge $\U$ on the coarser lattice.
 In that case, $\U (x,y)$ equals (up to a constant factor) the
 parallel transport along an arbitrary path from $\hat{y}$ to
 $\hat{x}$.
 [It is the path-independence of parallel transporters which
 characterizes a pure gauge in dielectric gauge fields, rather than
 the definition given in footnote~{\protect\small\ref{footnotePG}},
 page~\pageref{footnotePG}.]

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Computation of Averaging Kernels
 \label{SecAlgorithmC}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Gauge Covariant Block Spins}}
          {{\rm\thesubsection.}\ {\sl Computation of Averaging Kernels}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl In numerical applications the averaging kernel $C$ has to be
      recomputed whenever the gauge field~$U$ has been updated.
      An efficient algorithm is presented in this section which allows
      to compute the solution of the eigenvalue equation
      \equ{EVequationC} numerically.
      This algorithm has also been described in Ref.~\cite{KalNP2}.
      The same algorithm can be used to compute the kernel~$C$ of the
      Laplacian choice for staggered fermions.
      There the algorithm has the same efficiency, and one can also use
      the same computer program; the only changes which have to be made
      are replacements of address lists and of parallel transporters in
      the Laplacian.
      The relevance of the eigenvalue spectrum of $-\LAPN$ for the
      efficiency of the algorithm will be pointed out.
      Results of the numerical implementation will be reported.}
 \smallskip

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 \SubSubsection{An Algorithm for the Solution of the Eigenvalue
                Equation \protect\equ{EVequationC}}
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 The eigenvalue problem \equ{EVequationC} will be solved by means of
 Wielandt or inverse iteration.
 In each stage of this algorithm one has to solve a linear system
 of equations.
 Its solution will be determined by using the CG algorithm.
 The efficiency of the inverse iteration method depends on the quality
 of the estimate for the eigenvalue corresponding to the sought
 eigenvector.
 When determining the $C$-kernel, this estimate shall be close to the
 lowest eigenvalue $\lambdanull$ of $-\LAPN$, but we must demand that it
 is not greater than $\lambdanull$.
 An efficient method for bounding eigenvalues from below is
 provided by Temple's Theorem.

%..............
 \Subsubsection{Inverse iteration}
%..............
 Inverse iteration is a method by which one can determine all
 eigenvalues and eigenvectors of a quadratic matrix%
  \footnote{The matrix need not be normal or normalizable.}
 $A$, provided that sufficiently good approximate values for the
 eigenvalues are known.

 Let $\la_0 , \ldots , \la_m$ be the eigenvalues of $A$.
 Suppose that we know a good approximation $\la$ to $\la_j$, say,
 i.\,e.\ $| \la_j - \la | \ll |\la_k - \la |$ for all $\la_k \neq
 \la_j$, but $\la \neq \la_j$.
 For finding an eigenvector $x_j$ with eigenvalue $\la_j$,
 one starts with an arbitrary vector $x^{(0)}$ and computes a
 sequence of vectors $x^{(1)}, x^{(2)}, \ldots$, according to
%------------------- equation ------------------------------------------
 \begin{equation}
  ( A - \la ) x^{(i)} = x^{(i-1)}\esk \quad i=1,2,3,\ldots \esp
 \label{II}
 \end{equation}
%------------------- equation ------------------------------------------
 It is easy to see by expanding the $x^{(i)}$ in terms of eigenvectors%
  \footnote{If $A$ is defective one expands in terms of eigenvectors and
            principal vectors \cite{StoBul,WilRei}.}
 of $A$ that the iteration prescription \equ{II} yields an eigenvector
 $x_j$.
 If there is a degeneracy in $\lambda_j$, one obtains a linear
 combination of eigenvectors with eigenvalue $\lambda_j$.
 If the condition $| \la_j - \la | \ll |\la_k - \la |$ for all
 $\la_k \neq \la_j$ cannot be fulfilled (i.~e.\ if $\lambda_j$ is
 nearly degenerate with one $\lambda_k$), the efficiency of inverse
 iteration is lessened.
 One would need more iterations in that case.
 \newline
 See Refs.~\cite{StoBul,WilRei,Preetal} for a more comprehensive
 discussion on the method of inverse iteration.

%..............
 \Subsubsection{Application of the method for solving
                Eq.~\equ{EVequationC}}
%..............
 We shall modify the rudimentary method \equ{II} a little bit.
 In order to keep the components of the iterated vectors finite,
 it is advisable to normalize them.
 Also, the rate of convergence of the inverse iteration is faster
 the closer $\la$ is to $\la_j$.
 One can therefore try to accelerate the method by updating the
 estimate $\la$ in course of the procedure.
 To solve Eq.~\equ{EVequationC} we are thus led to the following form of
 inverse iteration:
 Choose a normalized $\Cstarx{(0)} = C^{\ast (0)}(\,\cdot\,,x)$
 for every block $x$ and iterate
%------------------- equation ------------------------------------------
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\theequation}{\thesection.\arabic{equation}\alph{abc}}
 \setcounter{abc}{1}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \begin{eqnarray}
 \left( - \LAPN - \la^{(i)}(x) \right)\,\Vx & = & \Cstarx{(i-1)} \esk
 \label{IICa} \\
 \addtocounter{abc}{1}\addtocounter{equation}{-1}
 \Cstarx{(i)} & = & \frac{\Vx}{\| \Vx \|_x}
 \label{IICb}
 \end{eqnarray}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\theequation}{\thesection.\arabic{equation}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
%------------------- equation ------------------------------------------
 \hspace*{-0.5em}for $i = 1,2,3,\ldots$.
 $\la^{(i)}(x)$ is an estimate of $\lambdanull$ in the $i$-th iteration.
 The norm $\| \cdot \|_x$ is induced by the scalar product
%------------------- equation ------------------------------------------
 \begin{equation}
 < V_1 , V_2 >_x\ =\ L_b^{-d} \sum_{z \in x}
  \frac{1}{\Nc} \re\Tr[V_1 (x,z)^{\dagger} V_2 (x,z)] \esp
 \label{ScalarProductKernel}
 \end{equation}
%------------------- equation ------------------------------------------

 Recall that strictly speaking the vectors $\Cstarx{(i-1)}$ and $\Vx$
 are actually $(\L^d \cdot \Nc \times \Nc)$ matrices.
 In our numerical implementation (Sec.~\ref{SecNumImpl}), however,
 these matrices are represented by ``true'' (one-column) vectors.

 Proper choices for $\la^{(1)}(x)$ and for $\Cstarx{(0)}$,
 and the updating procedure $\la^{(i)}(x) \rightarrow \la^{(i+1)}(x)$
 will be discussed below.
 Before that we discuss how the system \equ{IICa} is solved.
 The solution will be computed by means of the CG method \equ{CG} with
 the obvious replacements $D \rightarrow  (- \LAPN - \la^{(i)}(x))$,
 $f \rightarrow \Cstarx{(i-1)}$, and $\phi \rightarrow \Vx$.
 Also, the scalar product \equ{ScalarProduct} is of course replaced
 by \equ{ScalarProductKernel}.

 On a vector computer Eq.~\equ{IICa} is solved for all blocks in
 parallel by vectorizing over the block index $x$.
 The solution will be obtained quite fast because CG solves
 Eq.~\equ{IICa} in at most $L_b^d$ iterations.
 In order that the operators $(- \LAPN - \la^{(i)}(x))$ are positive
 definite, every $\la^{(i)}(x)$ must be less than the smallest
 eigenvalue $\lambdanull$ of $- \LAPN$.
 Since $-\LAPN$ is positive semidefinite, we can for example choose
 $\la^{(i)}(x) =  - \varepsilon$ with a small positive $\varepsilon$.
 But we can do better.

%..............
 \Subsubsection{Estimation of eigenvalues by the Rayleigh quotient}
%..............
 One starts inverse iteration with some lower bound $\lae$ for
 $\lambdanull$ and gets a first approximation $\Cstarx{(1)}$ of
 $\Cstarx{} = C^{\ast}(\,\cdot\,,x)$.
 We wish to replace $\lae$ by an improved estimate $\laz$
 which is closer to $\lambdanull$, so that the components orthogonal to
 $\Cstarx{}$ become more strongly suppressed in going from
 $\Cstarx{(1)}$ to $\Cstarx{(2)}$ than they were in the step
 $\Cstarx{(0)} \rightarrow \Cstarx{(1)}$.
 \newline
 Having solved Eq.~\equ{IICa} for $i=1$, we obtain an estimate for
 $\lambdanull$ by computing the Rayleigh quotient of $\Vx$ which is
 defined through
%------------------- equation ------------------------------------------
 \begin{equation}
  R [ \Vx ]\ =\ \frac{< \Vx\,,\,-\LAPN \Vx >_x}{< \Vx\,,\,\Vx >_x} \esp
 \label{RQ}
 \end{equation}
%------------------- equation ------------------------------------------

 In numerical analysis the Rayleigh quotient is the standard estimate
 for an eigenvalue from an eigenvector approximation \cite{ColEWA}.
 $R$ has the property that the eigenvalues of $-\LAPN$ are its
 stationary points which are obtained when the corresponding
 eigenvectors are plugged in.
 One has $R [ \Vx ] = \lambdanull + O(\delta^2 )$, where $\delta =
 (\lambdanull - \lai ) / (\laei - \lai )$;
 $\laei$ is the second lowest eigenvalue of $-\LAPN$.

 Unfortunately, in order to have $(-\LAPN - \lai )$ positive
 to guarantee convergence of the CG algorithm, we must
 demand $\lai < \lambdanull$.
 But $\lambdanull$ is the absolute
 minimum of $R$, which means that always $R [ \Vx ] \geq \lambdanull$.
 In principle there is a simple way to circumvent this problem.
 Simply multiply both sides of Eq.~\equ{IICa} by
 $(-\LAPN - \la^{(i)}(x))$.
 But for this variant the CG method is substantially slower, because
 the computational labor is doubled in each iteration.
 Also, it is not a priori clear that a trial $\la^{(i+1)}(x) =
 R [ \Vx ]$ is strictly smaller than $\frac{1}{2} ( \lambdanull +
 \la_{1}(x) )$, which is a necessary condition for convergence of the
 inverse iteration towards $\Cstarx{}$.

%..............
 \Subsubsection{Bounding eigenvalues by Temple's Theorem}
%..............
 A way out of the dilemma is furnished by a bounding theorem for
 eigenvalues which is known as Temple's Theorem.

 \begin{quotation}\noindent
          {\sc Temple's Theorem} \cite{ColFA}:\protect\newline
   {\em Let $T$ be a self-adjoint operator in a Hilbert space $H$ with
        scalar product\newline $< \cdot\,,\,\cdot >$.
        Let $f^{(0)}$ and $f^{(1)}$ be two elements of $H \setminus
        \{ 0 \}$ with $T f^{(1)}\!=\!f^{(0)}$.\newline
        Compute the Schwarz constants}
%------------------- equation ------------------------------------------
 \begin{equation}
  a_0 =\ < f^{(0)}\,,\,f^{(0)} > \quad , \quad
  a_1 =\ < f^{(0)}\,,\,f^{(1)} > \quad , \quad
  a_2 =\ < f^{(1)}\,,\,f^{(1)} > \quad ,
 \label{SchwarzConstants}
 \end{equation}
%------------------- equation ------------------------------------------
   {\em and for a real number $t$ the Temple quotient}
%------------------- equation ------------------------------------------
 \begin{equation}
  \vartheta (t) = \frac{a_0 - t a_1}{a_1 - t a_2} \esp
 \label{TempleQuotinet}
 \end{equation}
%------------------- equation ------------------------------------------
   {\em If the interior of the interval $(p,q)$ contains
        $\mu_2 \equiv a_1 / a_2$ and exactly one isolated eigenvalue
        $\la$ and no other element of the spectrum of $T$, then}
%------------------- equation ------------------------------------------
 \begin{equation}
  \vartheta (q)  \leq \la \leq \vartheta (p) \esp
 \label{TempleBound}
 \end{equation}
%------------------- equation ------------------------------------------
 \end{quotation}

 See Ref.~\cite{ColFA} for a proof.

%..............
 \Subsubsection{A corollary for operators with a lowest eigenvalue}
%..............
 A corollary of Temple's Theorem is the following.
 Suppose $T$ has a lowest eigenvalue $\la_0$, which may also be
 degenerate, and one knows a lower bound $l_1$ for the second lowest
 eigenvalue $\la_1$ with $\mu_2 < l_1 \leq \la_1$.
 Then Temple's theorem is used with the interval $(-\infty , l_1)$
 and one obtains
%------------------- equation ------------------------------------------
 \begin{equation}
  \mu_2 \frac{\mu_1 - l_1}{\mu_2 - l_1}\ =\ \mu_2 - \frac{\mu_1 - \mu_2}
  {\frac{l_1}{\mu_2} - 1}\ \leq\ \la_0\ \leq\ \mu_2 \esk
 \label{TempleCor}
 \end{equation}
%------------------- equation ------------------------------------------
 where $\mu_1 \equiv a_0 / a_1$.

%..............
 \Subsubsection{Application of the corollary to \equ{IICa}}
%..............
 When we apply the corollary to the inverse iteration \equ{IICa}
 we obtain the bounds
%------------------- equation ------------------------------------------
 \begin{equation}
  \tau ( \li )\ \equiv\ \lai + \muz\,\frac{\mue - \li}{\muz  - \li}\
  \leq\ \lambdanull\ \leq\ \lai + \muz\ =\ R [ \Vx ] \esk
 \label{TAU}
 \end{equation}
%------------------- equation ------------------------------------------
 where
%------------------- equation ------------------------------------------
 \begin{eqnarray}
  \mue = \frac{1}{< \Cstarx{(i-1)}\,,\,\Vx >_x} & , &
  \muz = \frac{< \Cstarx{(i-1)}\,,\,\Vx >_x}{< \Vx\,,\,\Vx >_x}
  \nonumber\\ & & \label{TempleBounds}  \\
  \li = \tilde{\la}_{1}(x) - \lai & , &
  \tilde{\la}_{1}(x) \leq \la_{1}(x) \esp \nonumber
 \end{eqnarray}
%------------------- equation ------------------------------------------

 Of course, the question arises how one obtains a lower bound
 $\tilde{\la}_{1}(x)$ for the second lowest eigenvalue $\la_{1}(x)$
 of $-\LAPN$.
 In Ref.~\cite{ColEWA} it is discussed how to overcome this difficulty
 in general eigenvalue problems either by comparison with a soluble
 problem exploiting Courant's maximum-minimum-principle \cite{CouHil}
 or by means of a Ritz method.
 For $-\LAPN$ there is a simpler solution as will be shown below.
 Suppose for the moment that we know an appropriate
 $\tilde{\la}_{1}(x)$.
 Then we perform the updating of $\lai$ according to the following.
%------------------- equation ------------------------------------------
 \begin{eqnarray}
  & (i) & \mbox{If $\mu_{2}^{(i)}(x) \geq\ \li$}\esk
        \quad\mbox{then}\quad\lambda^{(i+1)}(x) = \lai\esp \nonumber\\
  & & \label{UpdateTemple}\\
  & (ii) & \mbox{Else compute $\tau ( \li )$ and set $\la^{(i+1)}(x) =
        \max \left( \lai , \tau ( \li ) \right)\esp$} \nonumber
 \end{eqnarray}
%------------------- equation ------------------------------------------

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 \SubSubsectiontocentry{Relevance of the Eigenvalue Spectrum of
                        $-\LAPN$ for the Efficiency of the Algorithm}
                       {Relevance of the Eigenvalue Spectrum of $-\LAPN$
                        \protect\\
                        for the Efficiency of the Algorithm}
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 In order to make use of the updating prescription \equ{UpdateTemple}
 we need a lower bound $\tilde{\la}_{1}(x)$ for the second lowest
 eigenvalue $\la_{1}(x)$ of $-\LAPN$.
 How do we get it?
 Also, it was already mentioned that the performance of inverse
 iteration might be bad when there is a degeneracy in the eigenvalue
 spectrum.
 So let us look at the spectrum of low-lying eigenvalues of $-\LAPN$.

%..............
 \Subsubsection{Spectrum of eigenvalues of $-\LAPN$ in pure gauges}
%..............
 In case of pure gauges the spectrum of $-\LAPN$ is known analytically.
 It is summarized in Table~\NextTable\ for $L_b = 3$ in four
 dimensions.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|}
 \hline
 Eigenvalue & 0.& 1.& 2.& 3.& 4.& 5.& 6.& 7.& 8.& 9.& 10.& 12. \\
 \hline
 Degeneracy & 1 & 4 & 6 & 8 & 13 & 12 & 10 & 12 & 6 & 4 & 4 & 1 \\
 \hline
 \end{tabular}}
       {The spectrum of $-\LAPN$ in $d=4$ dimensions without gauge
        field for block size $L_b = 3$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 The spectrum is the same for any gauge group $G$, except for an
 (additional) $\Nc$-fold degeneracy of each eigenvalue.

%..............
 \Subsubsection{Spectrum of low-lying eigenvalues of $-\LAPN$
                in nontrivial gauge fields}
%..............
 In nontrivial gauge field configurations the shape of the spectra
 will change, but the sum of all eigenvalues is invariant and equals
 always $\Nc \cdot 2\,d\,\L^{d-1} (\L-1)$. (This is $\Tr [ -\LAPN ] =$
 twice the number of links within the block).

 The distribution of the five lowest eigenvalues was determined
 numerically on a $3^4$ lattice with periodic boundary conditions in
 four-dimensional pure $SU(2)$ gauge theory with Wilson action.
 The results are shown in Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{13.0cm}
        {Expectation values of the five lowest eigenvalues (modulo
         two-fold degeneracy) of $-\LAPN$ for gauge group $SU(2)$ in
         pure gauge theory on a $3^4$ lattice as a function of $\beta$.
         In pure gauges ($\beta=\infty$), $\lambdanull = 0$
         and the other four eigenvalues are degenerate with value $1.0$.
         The indicated strong and weak coupling expansion of $\langle
         \lambdanull \rangle$ derived from the numerical data is
         $1.2284(7) - \beta \cdot 0.2163(15)$ and $\beta^{-1}
         \cdot 0.830(7)$, respectively.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 The eigenvalues $\la_2 (x)$, $\la_3 (x)$, and $\la_4 (x)$ have no
 impact on the performance of our algorithm, but it is interesting to
 see how the degeneracy of $\la_1 (x), \ldots , \la_4 (x)$ is lifted in
 nontrivial gauge fields.

 The Monte Carlo method implemented for updating the gauge field
 was Creutz's heat bath algorithm \cite{CreHB}.
 The eigenvalues were computed by means of existing libraries
 \cite{NAGLIB}.
 These computations were done on the computers of the University of
 Hamburg \cite{UniRechner} and of DESY \cite{DESYIBM}.
 One thousand sweeps with measurements were performed after discarding
 1000 sweeps to ensure thermalization.

 It is interesting to note that $\lambdanull$ behaves similar to
 the plaquette energy $\langle 1 - \frac{1}{2} \Tr U(P) \rangle$
 which has strong coupling expansion $1 - \beta / 4 + O(\beta^3)$
 and weak coupling expansion $3 / (4 \beta )$ \cite{CrePlaquette},
 and which exhibits a crossover from strong to weak coupling at $\beta$
 around $2.0$.
 This crossover manifests itself also in the behavior of $\langle
 \lambdanull \rangle$, and through a kind of blowing up of the band
 width of $\langle\la_{1}(x)\rangle , \ldots , \langle\la_{4}(x)
 \rangle$.

%..............
 \Subsubsection{Implications for practical computations}
%..............
 Fig.~\PreviousFig\ is very promising, because we are mainly interested
 in the region of larger $\beta$-values where a distinct gap exists
 between $\lambdanull$ and $\la_{1}(x)$.
 This permits to compute the kernels with only two inverse iterations
 (at least for $\beta \geq 1.8$ where numerical investigations were
 performed, see below).

 We note that the relatively large gap between $\lambdanull$ and
 $\la_1 (x)$ will also be present for other gauge groups at large
 $\beta$.
 This is so because the gap equals 1 for $\beta = \infty$, and $\langle
 \lambdanull \rangle$ will always have a weak coupling expansion
 $\mbox{{\em const}} \cdot \beta^{-1}$, whereas $\langle \la_1 (x)
 \rangle$ will stay close to~1\@.

 One might speculate how the picture looks like when one implements
 the Diracian proposal for staggered fermions.
 In pure gauges the Diracian proposal reduces to the Laplacian choice,
 so that the gap between $\la_0$ and $\la_1$ will also equal~1 at
 $\beta = \infty$.
 The question is what happens at finite values of~$\beta$.

%..............
 \Subsubsection{Finite size effects}
%..............
 When one determines $\langle \lambdanull \rangle$ on the 81 blocks of
 a $9^4$ lattice one observes some finite size effects as shown in
 Table~\NextTable.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|c|c|c|}
 \hline
 $\beta$ & $\langle \lambdanull \rangle$ on $3^4$ lattice
 & $\langle \lambdanull \rangle$ on $3^4$ blocks in a $9^4$ lattice \\
 \hline
 \hline
  $1.8$ & $0.7469 \pm 0.0034$ &  $0.7542 \pm 0.0008$ \\
  $1.9$ & $0.6924 \pm 0.0044$ &  $0.7068 \pm 0.0008$ \\
  $2.0$ & $0.6284 \pm 0.0062$ &  $0.6538 \pm 0.0014$ \\
  $2.1$ & $0.5537 \pm 0.0055$ &  $0.5923 \pm 0.0008$ \\
  $2.2$ & $0.4868 \pm 0.0037$ &  $0.5331 \pm 0.0012$ \\
  $2.3$ & $0.4435 \pm 0.0025$ &  $0.4747 \pm 0.0010$ \\
  $2.4$ & $0.4082 \pm 0.0025$ &  $0.4280 \pm 0.0006$ \\
  $2.5$ & $0.3780 \pm 0.0016$ &  $0.3943 \pm 0.0005$ \\
  $2.6$ & $0.3592 \pm 0.0016$ &  $0.3683 \pm 0.0004$ \\
  $2.7$ & $0.3372 \pm 0.0016$ &  $0.3466 \pm 0.0004$ \\
 \hline
 \end{tabular}}
       {Finite size effect:
        Expectation values of the lowest eigenvalue $\lambdanull$
        of $-\LAPN$ on a $3^4$ lattice and on the 81 blocks of size
        $3^4$ embedded in a $9^4$ lattice.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 The values on the $9^4$ lattice were determined by means of the Temple
 bounds.

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 \SubSubsection{Numerical Implementation of the Algorithm}
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 The numerical implementation of the algorithm proposed above will
 now be explained.

%..............
 \Subsubsection{Choice for lower bounds of eigenvalues}
%..............
 The result for the low-lying eigenvalue spectrum of $-\LAPN$ provides
 us with lower bounds $\la^{(1)}(x)$ and $\tilde{\la}_{1}(x)$.
 {}From the measured distribution of eigenvalues (not expectation
 values!) one can extract lower bounds for $\lambdanull$ and $\la_{1}(x)
 $ which have a confidence level very close to $100 \%$\@.
 These bounds are used for $\lae$ and $\tle$.
 In the course of the inverse iteration \equ{IICa}, $\tle$ will not be
 changed and will retain its $x$-independent value%
 \footnote{Note that $\taul$ is a monotonically increasing function
           of $\tle$, but the dependence on $\tle$ is weak.
           It was checked that one can retain $\taul < \lambdanull$,
           when $\tle$ is greater than a practically $100 \%$ c.\ l.\
           upper bound for $\la_{1}(x)$.
           This means that $\taul$ is a very stable lower bound
           for $\lambdanull$.},
 whereas $\lai$ is updated according to \equ{UpdateTemple} and is only
 $x$-independent for $i\!=\!1$.

%..............
 \Subsubsection{Initialization of $C$}
%..............
 It remains to fix a normalized $\Cstarx{(0)}$.
 Two different choices were tested, a gauge variant and a gauge
 covariant choice.
 The first one is trivial initialization $(L_b a)^d C^{\ast (0)}(z,x) =
 \bbbone$ for all $z \in x$.
 The second choice is Ba{\l}aban's radial gauge \cite{BalLGT},
 where one sums up with equal weights all parallel transporters along
 the taxi-driver paths (paths of shortest length) from $\hat{x}$ to $z$,
 for all $z \in x$; the result is brought back into the gauge group by
 polar decomposition \cite{MacDLGT}.

 By computing the Rayleigh quotient of $\Cstarx{(0)}$ one finds that
 the component proportional to the sought eigenvector $\Cstarx{}$ is
 clearly dominating in Ba{\l}aban's gauge, because in this case $R [
 \Cstarx{(0)}]$ lies between $\lambdanull$ and $\la_{1}(x)$.
 For a trivially initialized $\Cstarx{(0)}$ the components orthogonal
 to $\Cstarx{}$ dominate.
 A priori this does not imply anything for the rate of convergence
 of inverse iteration, but the finding is that it is more
 efficient to use Ba{\l}aban's gauge for $\Cstarx{(0)}$.

%..............
 \Subsubsection{Performance of the algorithm}
%..............
 We conclude this section with some remarks on the performance of
 the algorithm described above.

 The CG method was used with initialization of $V_x$ to zero.
 In this case one needs less than 27 (29) CG iterations in the
 first (second) inverse iteration to solve Eq.~\equ{IICa} sufficiently.
 The CG algorithm was stopped when the root mean square (RMS) residuals
 of all blocks were reduced by $10^{-4}$.
 In general, a small residual does not mean that one is close to the
 solution, but the above criterion is good enough for the present case.
 This is demonstrated by explicitly computing $R [ \Cstarx{(i)} ]\
 =\  < \Cstarx{(i)}\,,-\LAPN \Cstarx{(i)} >$ and comparing with $\lai +
 \mu_{2}^{(i)}(x)$.
 Both results agree.

 The updating procedure \equ{UpdateTemple} always yields an improved
 estimate of $\lambdanull$ for the second inverse iteration if $\beta
 \gsim 2.15$.
 This is not the case if $\Cstarx{(0)}$ is trivially initialized;
 either the condition $\mu_{2}^{(i)}(x) < \li$ is not fulfilled
 or if it is fulfilled $\taul$ might not be larger than $\lai$.
 \newline
 Due to fluctuations, for $\beta \lsim 2.15$ the lower bound $\tle$
 of $\la_{1}(x)$ is not always greater than $\lambdanull$, so that the
 necessary condition $\mu_{2}^{(i)}(x) \geq \li$ for getting an
 improved $\la^{(i+1)}(x)$ may be violated if $\lambdanull \geq \tle$.
 Nevertheless, a second inverse iteration with a non-improved $\lai$
 is also sufficient (at least down to $\beta = 1.8$).

 After two inverse iterations the components orthogonal to $\Cstarx{}$
 are practically eliminated.
 This is proved by inspecting the Temple bounds $\la^{(3)}(x)$ and $R [
 \Cstarx{(2)} ]$ for $\lambdanull$, and by comparing $R [ \Cstarx{(2)}
 ]$ with $|| -\LAPN \Cstarx{(2)} ||$.
 The difference $R [ \Cstarx{(2)} ] - \la^{(3)}(x)$ is typically less
 than $10^{-5}$ for larger values of $\beta$, while it becomes slightly
 greater for smaller $\beta$-values where $\lae$ or $\laz$ is not always
 improved.
 However, $R [ \Cstarx{(2)} ]$ and $|| -\LAPN \Cstarx{(2)} ||$
 practically coincide in the examined $\beta$-range from $1.8$
 to $2.7$, which shows that $\Cstarx{(2)} = \Cstarx{}$ to a very high
 precision.

 Finally we report the performance on a CRAY Y-MP \cite{CRAY}.
 The routines are completely vectorizable (vectorization over
 the block index).
 In case of a $9^4$ lattice and block size $L_b^d = 3^4$
 (vector length of 81) the CPU time needed to compute $\Cstarx{(2)}$
 is $5.7$ $m$sec per block.
 An average rate of 230 MFLOPS is achieved.
 The CPU time required to compute $\Cstarx{(2)}$ for all blocks
 is comparable with that needed for one standard Monte Carlo sweep
 through the lattice.
 Thus, {\em the projective definition of block spins is numerically
 implementable for non-Abelian gauge theories\/}.
 It is not necessary to sacrifice the gauge covariance of the
 ground-state projection method by employing a particular gauge
 fixing condition (which also costs CPU time).

 \smallskip
%..............
 \Subsubsection{Concluding remarks}
%..............
 In Ref.~\cite{KalNP2} the author reported some results of a Monte
 Carlo renormalization group (RG) study, using the averaging kernel
 \equ{EVequationC} for gauge covariant blocking.
 He also considered a Laplacian with Dirichlet boundary
 conditions on block boundaries in \cite{KalNP2}.
 The results are very promising.
 They indicate that the projective RG transformation might be fruitful
 when it is studied in the framework of color dielectric models
 \cite{Pir}, and also when it is used for RG investigations with block
 gauge field in the gauge group \cite{CalPet,PatGup}.
 For details the reader is referred to Ref.~\cite{KalNP2}.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsectiontocentry{Optimal Interpolation Kernels
                     in the Presence of Gauge Fields}
                    {Optimal Interpolation Kernels in the \protect\\
                     Presence of Gauge Fields
 \label{SecOptA}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Gauge Covariant Block Spins}}
          {{\rm\thesubsection.}\ {\sl Optimal Interpolation Kernels in
                                      the Presence of Gauge Fields}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl The gauge covariant generalization of the optimal
      Gaw\c{e}dzki-Kupiainen interpolation kernel~$\A$ for bosons
      and for staggered fermions is studied in this subsection.
      The optimal kernel $\A$ decays exponentially for {\em any}
      value of the gauge field coupling.
      Therefore {\em ground-state projection (with the Laplacian choice
      of the fermionic~$C$) defines a good block spin in arbitrarily
      disordered gauge fields.}}
 \smallskip

 It was mentioned earlier that a good choice of block spin, i.~e.\ of~%
 $C$, means that the associated optimal interpolation kernel $\A$
 decays exponentially.
 We claimed already that ground-state projection \equ{EVequationC},
 \equ{EVequationCSF} is such a good choice in the presence of gauge
 fields.

%..............
 \Subsubsection{Optimal $\A$ for free massless bosons and fermions}
%..............
 When no gauge fields are present, the fall-off properties of~$\A$
 can be proven analytically.
 This is done by using the Fourier representation of~$\A$, and
 shifting the path of the momentum integration into the complex plane
 \cite{GawKup}.

 In order to verify the decay property of $\A$ explicitly by giving
 numbers, $\A$ was computed as the solution of Eq.~\equ{optimalA}
 for massless free bosons and staggered fermions.
 (Eq.~\equ{optimalA} was solved by means of CG.)
 Since $\Dirac^2$ decomposes into $2^d$ independent Laplacians on the
 pseudoflavor sublattices when $U$ is trivial, the optimal $\A$ fulfills
 $\A (z,x) = 0$ if $z$ and $x$ have different pseudoflavor.
 If $z$ and $x$ have the same pseudoflavor, then $\A (z,x)$ equals the
 bosonic $\A$-kernel on an $N^d$ lattice if the staggered lattice has
 volume $(2N)^d$.
 This serves as a good check for consistency of the computer programs.

 Bosonic $\A$-kernels for $9^4$, $12^4$, and $18^4$ lattices (with
 periodic boundary conditions) are given in the first three tables
 of Appendix~\theappKernels.3.
 These tables contain values of $\A (z,x)$ for $U\equiv\bbbone$.
 One sees an exponentially damped oscillating fall-off.
 In other trivial gauge fields (pure gauges), $\A (z,x)$ gets
 multiplied with the parallel transporter from $\hat{x}$ to $z$.
 Kernels on $18^4$ lattices are visualized in Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \DoubleFigure{10.5cm}
        {Optimal interpolation kernel $\A (z,0)$ in trivial gauge fields
         on $18^4$ lattices ($L_b = 3$), for bosons (top) and staggered
         fermions (bottom).
         A two-dimensional cut through the block center $x=0$ is shown,
         $z_3$ and $z_4$ are fixed.
         The vertical axis gives the norm of $\A (z,x)$.
         The fermionic kernel is the one which is associated with the
         Laplacian choice of~$C$.
         The fall-off properties of this~$\A$ are relevant for work on
         renormalization group transformations for fermi fields.
         Note the support properties of the fermionic~$\A$.
         It has support only on one particular pseudoflavor sublattice,
         where it equals the bosonic~$\A$ for a $9^4$ lattice.
         (G.\,Mai \protect\cite{Mai} investigated a renormalization
          group transformation where she blocked free continuum
          fermions to staggered fermions; G.\,Mai showed analytically
          that the optimal~$\A$ associated with her blocking procedure
          has exponential fall-off, cf.\ the remarks in
          Sec.~\protect\ref{SecBSforSF}.)}
              {9.0cm}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \DoubleFigure{10.5cm}
        {Optimal interpolation kernel $\A (z,0)$ in a quenched
         four-dimensional $SU(2)$ gauge field at $\beta=2.7$ on $18^4$
         lattices ($L_b = 3$), for bosons (top) and staggered
         fermions (bottom).
         A two-dimensional cut through the block center $x=0$ is shown,
         $z_3$ and $z_4$ are fixed.
         The vertical axis gives the trace norm of $\A (z,x)$.
         (Remember that $\A (z,x) \in \bbbr \cdot SU(2)$.)
         The fermionic kernel is the one which is associated with the
         Laplacian choice of $C$.
         Note the support properties of this $\A$.
         It has support on all even lattice sites and is vanishing on
         all odd sites.
         The increased support compared to the case $\beta = \infty$
         is due to the non-vanishing field strength at finite $\beta$.}
              {10.5cm}
 \setcounter{FigAbose}{\value{figure}}
 \setcounter{SecAkernel}{\value{section}}
%\setcounter{FigAfermi}{\value{figure}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%..............
 \Subsubsection{Optimal $\A$ for bosons and fermions in nontrivial
                gauge fields}
%..............
 Next the $\A$-kernels were computed in nontrivial four-dimensional
 quenched $SU(2)$ gauge fields at various values of $\beta = 4/g^2$,
 including the case of a completely random gauge field ($\beta = 0$).
 The operator $D$ in Eq.~\equ{optimalA} was $D=-\Delta + m^2$ with
 $m^2 = \mcr$ in case of bosons,%
 \footnote{Values of $\mcr$ will be given in Secs.~\ref{SecSmoothness}
           and~\ref{SecProof}.}
 while for fermions $D = -\Dirac^2+m^2$ with $m^2=0$.
 It was verified that for {\em any} $\beta$-value the definition of the
 averaging kernel $C$ as a solution of a gauge covariant Laplace
 eigenvalue equation~\equ{EVequationC}, \equ{EVequationCSF}
 yields a good choice of block spin in the sense described above.
 This is true both for bosons and for staggered fermions.
 Examples are in Fig.~$3.8$.
 $\A$ decays exponentially over distance $L_b a$ (nearly) as fast
 in the presence of gauge fields than in their absence.
 For this reason the more intricate Diracian choice of $C$ has not been
 implemented numerically yet.

 \smallskip
 The effective coarse grid operators which are associated with the
 optimal $\A$-kernels decay also exponentially.
 Therefore they are to a good approximation also of (next) nearest
 neighbor form.
 Examples are given in Tables~B.4--B.6, B.9, and B.10 of
 Appendix~\theappKernels.3.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Short Review of Ba{\l}aban's Analytical Work}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Gauge Covariant Block Spins}}
          {{\rm\thesubsection.}\ {\sl Short Review of Ba{\l}aban's
                                      Analytical Work}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl Ba{\l}aban's analytical work on the decay properties of
      gauge covariant propagators is briefly outlined.}
 \smallskip

 There exists analytical work on exponential decay of propagators
 in gauge fields.
 We repeat here an outline which was given in Ref.~\cite{KalMacSpe}.

 Ba{\l}aban presented a method to study fall-off properties of gauge
 covariant propagators \cite{BalProp}, see also \cite{BalJaf}.
 He considered gauge covariant bosonic ``fluctuation field''
 propagators
%------------------- equation ------------------------------------------
  \begin{equation}
    \Gamma = \left( -\Delta + m^2 + \kappa\,\Cstar C \right)^{-1} \esk
  \label{GammaCov}
  \end{equation}
%------------------- equation ------------------------------------------
 cf.\ Eq.~\equ{Gamma} in Appendix~\theappKernels.
 Ba{\l}aban showed exponential decay of $\Gamma$ under general
 assumptions on $C$, and for sufficiently small gauge field coupling.
 He required $\Cstar C$ to be a projector on constant functions in
 the absence of gauge fields; this requirement is fulfilled by our
 choice of $C$.
 It is instructive to see what difficulties arise when one
 tries to generalize Ba{\l}aban's proof to staggered fermions.
 $\Delta$ gets replaced by the square of the Dirac operator.

 In the bosonic case Ba{\l}aban proceeds by writing down a
 generalized random walk expansion for $\Gamma$.
 Ba{\l}aban considers a covering of $\bbbr^d$ by hypercubes $\Box_j$ of
 side length $2L$, $L\in\bbbz$ which are centered at $L j$,
 $j\in\bbbz^d$.
 Two hypercubes $\Box_i$ and $\Box_j$ have the property that they
 overlap iff $\| i - j \|_{\infty} \leq 1$.
 Every site $z \in \bbbz^d$ is contained in exactly $2^d$ hypercubes
 $\Box_j$.
 Ba{\l}aban also introduces functions $h_j (z)$ whose supports are
 within $\Box_j$ and whose squares are a partition of unity:
 $\sum_j h_j^2 = 1$.
 The leading term of Ba{\l}aban's generalized random walk expansion
 for $\Gamma$ is
%------------------- equation ------------------------------------------
  \begin{equation}
   \sum_j h_j\,\Gamma^0_j\,h_j \quad\mbox{where}\quad
   \Gamma^0_j = \left( -\LAPNj + m^2 + \kappa\,\Cstar C \right)^{-1}\esk
  \end{equation}
%------------------- equation ------------------------------------------
 and $\LAPNj$ is the Laplacian with Neumann boundary conditions on
 boundary of the hypercube $\Box_j$.
 It is defined as in Eq.~\equ{LAPN} except that $x$ has to be replaced
 by $\Box_j$.
 The full expansion is of the form
%------------------- equation ------------------------------------------
  \begin{equation}
   \Gamma\   =\   \sum_j h_j\,\Gamma^0_j\,h_j\
                 + \sum_{j_0,j_1,j_2}
                         h_{j_0}\,\Gamma^0_{j_0}\,R_{j_1,j_2}\,%
                                  \Gamma^0_{j_2}\,h_{j_2}\
                 + \sum_{j_0, \ldots ,j_4}
                         h_{j_0}\,\Gamma^0_{j_0}\,R_{j_1,j_2}\,%
                                  \Gamma^0_{j_2}\,h_{j_2}\,%
                                  R_{j_3,j_4}\,\Gamma^0_{j_4}\,h_{j_4}\
                                                           +\ \cdots
 \label{RWexpansion}
  \end{equation}
%------------------- equation ------------------------------------------
 where $R_{i,j}$ are operators which satisfy certain bounds on
 their norms, and whose kernels $R_{i,j} (z,w)$ are only nonvanishing
 when $z,w$ are in neighboring hypercubes $\Box_i$ and $\Box_j$.
 [The operator $R_{i,j}$ contains $h_i^2$ and $h_j$.]
 Only random walks $\{ j_0 , j_1 , \ldots , j_{2n} \}$ contribute to
 the expansion \equ{RWexpansion} where $\| j_{2i} - j_{2i+1}
 \|_{\infty} \leq 1$, $i = 0 , 1 , \ldots$

 The Neumann boundary conditions lead to a decoupling such that
%------------------- equation ------------------------------------------
  \begin{equation}
  \Gamma^0_j (z,w) = 0
    \quad\mbox{unless $z$, $w$ are in the same hypercube $\Box_j$.}
  \label{supportGamma0}
  \end{equation}
%------------------- equation ------------------------------------------
 It follows that the contributions to the series \equ{RWexpansion}
 up to $n$-th order make contributions to $\Gamma(z' , w')$ only
 if $z'$ and $w'$ are no further than $n-1$ hypercubes away from each
 other, i. e. if $|z' -w' | < n\,L\,a$.
 Therefore the propagator $\Gamma$ will have exponential decay
 if the Neumann series \equ{RWexpansion} converges.

 Given the bounds on the norms of $R_{i,j}$, convergence will hold if
 the lowest eigenvalues of
%------------------- equation ------------------------------------------
  \begin{displaymath}
    - \LAPNj + \kappa \Cstar C
  \end{displaymath}
%------------------- equation ------------------------------------------
 stays sufficiently far away from~$0$.
 $-\LAPNj$ has at most one eigenvalue close to zero, and if $\Cstar C$
 is the projector on this eigenmode and $\kappa$ is not too small, then
 the lowest eigenvalue of $- \LAPNj + \kappa \Cstar C$ is equal to the
 second lowest eigenvalue of $-\LAPNj$ (which is at least of order
 $(\pi / L )^{2}$).

 In conclusion, there are two essential ingredients.
 Neumann boundary conditions decouple between different hypercubes, and
 the lowest eigenvalues of $- \LAPNj + \kappa \Cstar C$ are not too
 close to zero.

 \smallskip
 In case of staggered fermions we want to replace the Laplacian
 $\Delta$ by the square of the Dirac operator $\Dirac^2$ on $\Lah$.
 The trouble is that blocks $x$ will overlap.
 This is innocuous in case of a pure gauge.
 In this case $\Dirac^2$ does not couple sites with different
 pseudoflavors $H$, and block spins $(C\chi )(x)$ receive contributions
 only from $\chi (z)$ when $z$ carries the same pseudoflavor as $x$.
 As a result, one can proceed as in the bosonic case.

 But this is no longer true when we have a nontrivial gauge field.
 One way out could be to retain $- \LAPNj + \kappa \Cstar C$ as $0$-th
 order term, where $\LAPNj$ is still the Laplacian.
 But this means that the $F_{\mu\nu}$ term in $\Dirac^2$
 has to be absorbed into $R_{i,j}$.
 If we use the Laplacian definition \equ{EVequationCSF} of $C$, then the
 lowest eigenvalue of $- \LAPNj + \kappa \Cstar C$ is as big as we can
 hope to make it, and decoupling holds also, but a good enough bound on
 $R_{i,j}$ will require that $F_{\mu\nu}$ is small enough.

 \smallskip
 The results of Sec.~\ref{SecOptA} give a numerical proof
 that gauge covariant propagators decay exponentially for arbitrary
 gauge coupling, both in the bosonic and in the fermionic case.
 Hence the effect of the $F_{\mu\nu}$-term is reasonably mild.
 Thus the numerical results can be considered as an encouragement
 for analytical calculations in fermionic gauge theories.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Smoothness in Gauge Theories
 \label{SecSmoothness}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Gauge Covariant Block Spins}}
          {{\rm\thesubsection.}\ {\sl Smoothness in Gauge Theories}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl The question is discussed what ``smoothness'' means in bosonic
      and fermionic gauge theories.
      The discussion supplies another argument why the generalized
      Gaw\c{e}dzki-Kupiainen interpolation kernel~$\A$ is ``optimal''.}
 \smallskip

 A central notion for MG methods is that of smoothness.
 Therefore it is crucial to answer the question:
 {\em What is a smooth function in the presence of gauge fields, or
      more generally in disordered systems?}
 This question is also discussed in
 Refs.~\cite{KalMacSpe,KalPL,MacKalPalSpe,BaeKalMacSpe}.

 We require to have a gauge invariant definition
 of smoothness, i.\ e.\ if a field configuration is smooth
 in a particular gauge it is also smooth in any other gauge.
 The standard definition of smoothness on length scale $a$ of some
 function~$e$ would be that its derivative is small,
%------------------- equation ------------------------------------------
 \begin{equation}
 \| \nabla_{\!\mu}\,e \|^2\ \equiv\ <\nabla_{\!\mu}\,e,\nabla_{\!\mu}\,e
 > \ =\ < e\,,\,-\Delta\,e >\quad \ll\quad < e\,,\,e >\ \equiv\ \|e\|^2
 \label{smoothness}
 \end{equation}
%------------------- equation ------------------------------------------
 (in units $a = 1$).

%..............
 \Subsubsection{Bosonic theories}
%..............
 In bosonic theories \equ{smoothness} is equivalent to saying that the
 Rayleigh quotient $R[e]$ is small.
 When $\nabla_{\mu}$ are ordinary derivatives then the definition
 \equ{smoothness} of smoothness is not gauge invariant.
 We could take covariant derivatives instead.
 In the bosonic case this gives indeed a natural gauge invariant notion
 of smoothness.

 The lowest eigenvalue of the covariant negative Laplacian is a natural
 measure of disorder.
 Except for a pure gauge, the lowest eigenvalue of $-\Delta$ is
 strictly positive.
 Thus, in a disordered gauge field there is a limit to how smooth
 a function can be.
 When disorder is big, then there are no smooth functions at length
 scale $a$ in the sense of \equ{smoothness}.
 But in this case one does not really need them either in realistic
 problems, because propagators $(-\Delta + m^2)^{-1}(z,w)$ for
 $m^2 \geq 0$ fall off fast anyway and there will be no critical
 slowing down when one applies standard methods, and hence there
 will be no need for MG\@.

 Some values of $\mcr$ (the lowest eigenvalue of $-\Delta$) in
 four-dimensional $SU(2)$ gauge fields are plotted in Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
        {Critical bosonic masses squared $\mcr$ of $SU(2)$ gauge field
         configurations in $d = 4$ dimensions.
         Open circles represent values on $9^4$ lattices, while filled
         symbols are values on $18^4$ lattices.
         In a pure gauge ($\beta = \infty$), $\mcr = 0$ for any
         lattice size.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 These values were determined by means of inverse iteration.

%..............
 \Subsubsection{Theories with staggered fermions}
%..............
 In the case of staggered fermions the situation is different.
 There are now two seemingly reasonable definitions.
 We may take for $\Delta$ in \equ{smoothness} the covariant
 Laplacian as defined in Eq.~\equ{SFcovLaplacian}, or substitute the
 square of the Dirac operator for it.
 We call these two possibilities the definitions of ``Laplacian
 smoothness'' and ``Diracian smoothness'', respectively.

 Unfortunately, both definitions are qualitatively different,
 except in the case of a pure gauge.
 Laplacian smoothness of a function $\chi(z)$ implies only
 restrictions which relate the values of $\chi(z)$ at points
 $z\in \Lah^H$ with the {\em same} pseudoflavor $H$.
 The same is {\em not} true of Diracian smoothness.
 Moreover, if the gauge field is fairly disordered, then there will be
 no functions with Laplacian smoothness.
 But it is {\em not} true in general that a propagator $(-\Dirac^2 + m^2
 )^{-1}(z,w)$ cannot have slow decay for $m \approx 0$.

%..............
 \Subsubsection{Smoothness of the optimal interpolation kernel~$\A$}
%..............
 The foregoing discussion of smoothness in gauge theories supplies
 another argument for using the optimal $\A$-kernel in MG computations.
 According to the MG philosophy $\A$ should map functions on $\Lone$
 into smooth functions on $\Lnull$.
 The optimal $\A$-kernel is characterized by requiring that for every
 function $\Phi$ on $\Lone$, $\phi = \A \Phi$ minimizes the action $\H\
 =\ < \phi\,,\,D_0\,\phi >$ subject to the constraint $C \phi = \Phi$.
 With the definition of smoothness that (covariant) derivatives are
 small, this can be rephrased:
 the interpolation $\phi = \A \Phi$ yields the smoothest possible
 function with prescribed block average $\Phi = C \phi$.

 When one follows the spirit of ground-state projection MG,
 then one should use the Diracian definition of smoothness for fermions,
 i.~e.\ one should substitute $\Dirac^2$ for $\Delta$ in
 \equ{smoothness}.
 In case of staggered fermions the gauge invariant norm $\| \Dirac e
 \| \equiv < e\,,-\Dirac^2\,e >^{1/2}$ of a low mode of $\Dirac$ is
 always small compared with $\| e \|$,
 but the same is not true of $< e\,,-\Delta\,e >^{1/2}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \Section{Computation of Free Propagators
 \label{SecFreePropagators}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}{}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl Now we turn to the numerical computation of propagators.
      We begin in this section with the simple free case (this means
      arbitrary pure gauge) where the bosonic and fermionic problems
      are equivalent.
      Computation of propagators in nontrivial gauge fields will
      be reported in the subsequent three sections.

      {\em Secs.~\ref{SecComputationalDetails} and~\ref{SecNumImpl}
      apply to all propagator computations.}}
 \medskip

 \begin{quotation}
%..............
 \Subsubsection{Summary of results}
%..............
 In trivial gauge fields the following results emerged:
 The convergence properties of the CG algorithm exhibit a
 substantial volume dependence for a given mass~$m^2$.
 No such volume dependence is found for relaxation algorithms.
 The theoretical predictions for conventional one-grid relaxation
 algorithms could be verified to a very high precision.
 In particular, it was confirmed that the convergence behavior
 depends only on $m^2$ and {\em not} on the lattice size.
 Variational MG with ``ground-state projection'' $\equiv$
 ``piecewise-constant'' interpolation, and the ``optimal'' MG
 scheme are both successful in eliminating the $1/\Dm$ divergence
 of relaxation times~$\tau$ on lattices of fixed size.
 No dramatic difference between variational MG and optimal MG is seen.
 It takes only a few iterations until errors decay exponentially.
 The variational MG method was investigated for various lattice
 sizes, and {\em no volume dependence was found\/}.
 {\em Hence, CSD is completely eliminated by MG for pure gauges.}
 It was found that a necessary condition for the elimination of
 CSD is an ``almost'' correct interpolation of the lowest mode
 (i.~e.\ of a constant function).
 The inclusion of the ``updating on a last site'', as discussed in
 Sec.~\ref{SecLP}, cannot improve the performance of MG algorithms
 any further for pure gauges.
 The result of its inclusion in traditional one-grid relaxation
 algorithms is interesting.
 CSD of {\em asymptotic} relaxation times can be eliminated in this way.
 Surprisingly this is only the case when the matrix $\Omega$ in
 \equ{rescaleBOSE} is chosen such that the energy functional gets
 minimized.
 No effect is seen when $\Omega$ is chosen such that the norm of the
 residual is minimized.
 However, a volume effect remains with respect to how many iterations
 it takes until the asymptotic regime is reached.
 This volume effect is similar to the one which shows up in the CG
 algorithm.
 \end{quotation}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Computational Details
 \label{SecComputationalDetails}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl Computational Details}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 All computations which will be reported in the sequel were performed
 on four-di\-men\-sion\-al hypercubic lattices.
 The \rhs $f$ of Eq.~\equ{propagator} was always a Kronecker-$\delta$.
 (Other choices yield the same values for relaxation times.)
 The initial guess for the propagator is zero in case of CG, and
 $\delta_{z,0}\,\omega / (8 + m^2)$ for the relaxation algorithms.
 The term ``trivial gauge field'' always means arbitrary pure gauge,
 and ``nontrivial gauge fields'' are always quenched $SU(2)$ gauge
 fields at finite gauge coupling.
 The gauge field configurations at finite $\beta$ were generated with
 the Wilson action \cite{Wil} by means of Creutz's heat bath algorithm
 \cite{CreHB}.

 As remarked at the end of Sec.~\ref{SecMGalgorithms},
 we take advantage of the facts that we work in four dimensions and
 that $L_b = 3$ is chosen, so that twogrid algorithms
 are sufficient to offer a big improvement if they are successful,
 because the second twogrid layer has 81 times fewer points.

 Residual equations on the block lattice are always solved exactly
 (i.~e.\ reducing the initial residual by $10^{-10}$) by the CG
 algorithm.
 Hence, there is no relaxation parameter for the block lattice, and
 the value quoted for $\omega$ is always the relaxation parameter
 on the finer lattice.

 Relaxation times $\tau$ in computations of propagators and number of
 iterations are always measured in units of cycles which involve only
 one sweep through the finest lattice.
 It was checked that values of $\tau$ practically do not depend on the
 numbers $\nu_1$ and $\nu_2$ of pre-smoothing and post-smoothing sweeps
 when $\tau$'s are properly rescaled.
 Relaxation times were determined as follows.
 The RMS (root mean square) residuals $\| r^{(n)} \| \equiv
 \left( | \Lnull |^{-1}\!\sum_{z\in\Lnull}\!\frac{1}{2} \Tr\left[
 r^{(n)}(z)^{\dagger} r^{(n)}(z) \right] \right)^{1/2}$
 were computed, and $\tau$ was determined from an
 exponential fit after $\| r^{(n+1)} \| / \| r^{(n)} \|$ has become
 constant for several iterations with an accuracy of better than
 $10^{-4}$.

 If not stated otherwise, SOR was always done in lexicographic
 ordering, except for bosons on $12^4$ and $18^4$ lattices where
 updating was performed in checkerboard fashion.

 Concerning the aspect of computational labor we note that
 the (non-optimized) implementations of the MG programs require a
 factor of $2.1$/$4.5$ (bosons/staggered fermions) more arithmetic
 operations than CG.
 When updating on an MG layer consisting of a single site
 (Secs.~\ref{SecLP},\ref{SecLPfermi}) is included, the factor is
 $3.2$/$7.8$.
 The amount of work for the averaging kernel~$C$ on the whole lattice
 is equivalent to less than 20 CG iterations.

 Finally, we note that {\em all computer programs were checked for
 gauge covariance.}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Numerical Implementations
 \label{SecNumImpl}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl Numerical Implementations}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The numerical implementation used for storing $SU(2)$ gauge fields
 and performing multiplications of (multiples of) $SU(2)$ matrices is
 based on the well-known isomorphism between $SU(2)$ and the unit
 sphere $S^3$ in four dimensions.
 Let $\bbbone$ denote the $2 \times 2$ unit matrix, and $\sigma_k$,
 $k=1,2,3$, the three Pauli matrices.
 Any $SU(2)$ matrix $U$ can be represented as
%------------------- equation ------------------------------------------
 \begin{equation}
   U = a_0 \bbbone + i \sum_{k=1}^3 a_k \sigma_k \esk
 \label{isomorphism}
 \end{equation}
%------------------- equation ------------------------------------------
 with real numbers $a_0$, $a_k$ which fulfill $a_0^2 + \sum_k
 a_k^2 = 1$.
 There exists no constraint on $a_0$, $a_k$ for matrices $U$ in
 $\mbox{span}\{SU(2)\}$.

 On the computer link variables, kernels, propagators etc.\ are
 stored by the four numbers $a_0$, $a_k$.
 Multiplication of two elements of $\mbox{span}\{SU(2)\}$ is
 implemented through statement functions.
 In the 4-vector representation the norm $\txeh \Tr
 [U^{\dagger}U]^{1/2}$ of a multiple $U$ of an $SU(2)$ matrix is simply
 given by $\sqrt{a_0^2 + \sum_k a_k^2}$.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Conjugate Gradient Algorithm
  \label{SecCGPG}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl Conjugate Gradient Algorithm}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The convergence behavior of the (unpreconditioned) CG algorithm on an
 $18^4$ lattice is shown in Fig.~\NextFig\ below, where it is compared
 with variational MG ($\A = \Cstar$).
 The CG algorithm has a complicated convergence behavior.
 Note that the norm of the residual is not monotonically decreased
 for small values of $m^2$.
 The reason is that CG decreases the energy functional in every
 iteration, but this does not necessarily mean that $\| \rn \|$ also
 decreases.

 It might be that the convergence behavior for small $m^2$ is
 affected by finite size effects, because the correlation length of the
 matter field (inverse mass) is not small compared to the linear
 extension of the lattice.
 However, this question could not be answered.

 It should also be noted that CG exhibits a volume effect.
 At fixed $m^2$ CG needs more iterations to converge to a given
 precision the larger the lattice becomes.
 This is true for all values of $m^2$, not only for artificially small
 ones.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{One-Grid Relaxation Algorithms
 \label{SecFreePropagators3}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl One-Grid Relaxation Algorithms}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The theoretical predictions for conventional relaxation algorithms
 which were discussed in Sec.~\ref{SecCSD1grid} could be confirmed
 to a very high precision.
 In particular, it was confirmed that the convergence behavior
 depends only on $m^2$ and {\em not} on the lattice size.
 For instance, in case of Jacobi iteration Eq.~\equ{scalingJac}
 predicts $\tau = 80\,000.5 + O( m^2 )$ for $m^2 = 10^{-4}$,
 whilst the numerical result is $\tau = 80\,000.50 \pm 0.26$.
 Also the $\omega$-dependence in Eq.~\equ{scalingJac} could be
 monitored very well.
 The predictions for SOR were also verified.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Variational Multigrid
 \label{SecFreePropagators4}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl Variational Multigrid}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 An advantage of variational MG with $\A = \Cstar$ (``piecewise-%
 constant interpolation'') is that the effective Laplacian is of the
 same nearest neighbor form as $\Delta$ on the finest lattice.
 This simple MG algorithm is able to eliminate CSD completely, i.\ e.\
 no mass dependence is observed for $m^2 \leq10^{-2}$,
 and no volume dependence is observed at fixed~$m^2$.
 Relaxation times $\tau$ are short.
 Hence, CG is clearly outperformed.
 Results are in Fig.~\NextFig\ and Table~\NextTable.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
         {Convergence of computations of propagators
          $(-\Delta + m^2)^{-1}$ in trivial gauge
          fields on an $18^4$ non-staggered lattice.
          The three (seven) curves of filled (open) symbols are results
          of variational MG (CG) computations.
          {}From left to right the curves belong to $m^2 =1, \ m^2= 0.1$
          and  $m^2 \leq 10^{-2}$ in case of MG, and $m^2 = 1$, $0.01$,
          $0.01$, \ldots , $10^{-6}$ in case of CG.
          No volume dependence was found for MG, whereas at fixed $m^2$
          CG needs more iterations to converge to a given precision
          the larger the lattice becomes.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|l||c|c||c|c|c|c|}
 \hline
 algorithm and & optimal & optimal  &
       \multicolumn{4}{|c|}{relaxation time $\tau$ for $m^2 =$} \\
 lattice size & $\delta$ & $\omega$ &
  $1.0$ & $0.1$ & $0.01$ & $10^{-3}, \ldots , 10^{-10}$ \\
 \hline\hline
 MG Jacobi on $9^4$  & $1.8$ & $0.96$ & $3.6$ & $6.4$ & $7.1$ & $7.2$\\
 \hline
 MG Jacobi on $18^4$ & $1.8$ & $0.94$ & $4.0$ & $6.4$ & $6.9$ & $7.0$\\
 \hline
 MG SOR on $18^4$    & $1.7$ & $1.09$ & $2.3$ & $2.5$ & $2.8$ & $2.9$\\
 \hline
 \end{tabular}}
       {Variational MG\@:
        Optimum values of $\delta$ and $\omega$ in a
        four-dimensional pure gauge ($\mcr = 0$) and demonstration of
        elimination of CSD.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 Table \PreviousTable\ contains a parameter $\delta$ which is defined
 as follows.
 We wish to approximate the ideal MG algorithm as well as possible.
 Without knowing the exact kernel $\A$, one cannot compute the exact
 ``effective difference operator'' $D_1$.
 Knowing that $D_1$ is approximately of nearest neighbor form
 (see Appendix~\theappKernels), one can try to approximate it.
 The choice
%------------------- equation ------------------------------------------
 \begin{equation}
   D_1 = \delta^{-1} C D_0 \Cstar
 \label{delta}
 \end{equation}
%------------------- equation ------------------------------------------
 yields another dielectric lattice gauge field $D_1 (x,y)$ which
 also has the right gauge covariance properties.
 Its fluctuating length can be adjusted to fluctuate around the
 ``right'' value (of the ideal $D_1 (x,y)$) by adjusting the real
 parameter $\delta$.
 In trivial gauge fields the influence of $\delta$ on $\tau$ is very
 weak, but a tuning of $\delta$ in nontrivial gauge fields can
 accelerate convergence substantially.
 The same is true of the relaxation parameter $\omega$.
 Dependences on $\delta$ and $\omega$ in the two-grid algorithm in
 trivial gauge fields are given in Table~\NextTable.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{
 \begin{tabular}{|c||r|r|r|r|r|r|r|r|}
 \hline
 \multicolumn{9}{|c|}{Dependence on $\delta$} \\
 \hline
 $\delta$ & $0.0$ & $0.45$ & $0.9$ & $1.35$ & $1.8$ & $1.9$ &
            $2.0$ & $2.1$ \\
 \hline
 $\tau$(Jacobi) & $800.5$ & $15.7$ & $15.7$ & $15.7$ &
                   $15.6$ & $15.6$ & $45.7$ & div. \\
 \hline
    $\tau$(Gauss-Seidel) & $400.2$ & $6.2$ & $4.4$ & $3.8$ &
                   $4.3$ & $8.5$ & $46.6$ & div. \\
 \hline
 \end{tabular}

 \vspace{0.5cm}
 \begin{tabular}{|r|r||r|r|}
 \hline
 \multicolumn{4}{|c|}{Dependence on $\omega$} \\
 \multicolumn{4}{|c|}{for $\delta = 1.8$ with}  \\
 \multicolumn{4}{|c|}{Jacobi relaxation} \\
 \hline
 $\omega$ & $\tau$ & $\omega$ & $\tau$ \\
 \hline
  $1.0$ & $15.6$ & $0.9$ & $8.0$ \\
 $0.99$ & $11.8$ & $0.8$ & $9.1$ \\
 $0.98$ & $9.4$  & $0.7$ & $10.5$ \\
 $0.97$ & $7.7$  & $0.6$ & $12.4$ \\
 $0.96$ & $7.4$  & $0.5$ & $14.9$ \\
 $0.95$ & $7.6$  & $0.4$ & $18.5$ \\
 $0.94$ & $7.6$  & $0.3$ & $24.1$ \\
 $0.93$ & $7.7$  & $0.2$ & $33.8$ \\
 $0.92$ & $7.8$  & $0.1$ & $54.8$ \\
 $0.91$ & $7.9$  &       &       \\
 \hline
 \end{tabular}
 \hspace{1.0cm}
 \begin{tabular}{|r|r||r|r|}
 \hline
 \multicolumn{4}{|c|}{Dependence on $\omega$} \\
 \multicolumn{4}{|c|}{for $\delta = 1.7$ with} \\
 \multicolumn{4}{|c|}{checkerboard SOR} \\
 \hline
 $\omega$ & $\tau$ & $\omega$ & $\tau$ \\
 \hline
  $1.9$ & $9.4$  & $0.9$ & $4.5$ \\
  $1.8$ & $4.5$  & $0.8$ & $5.5$ \\
  $1.7$ & $3.4$  & $0.7$ & $6.8$ \\
  $1.6$ & $3.3$  & $0.6$ & $8.4$ \\
  $1.5$ & $4.6$  & $0.5$ & $10.6$ \\
  $1.4$ & $4.5$  & $0.4$ & $13.7$ \\
  $1.3$ & $4.3$  & $0.3$ & $18.7$ \\
  $1.2$ & $4.2$  & $0.2$ & $27.6$ \\
  $1.1$ & $3.0$  & $0.1$ & $43.9$ \\
  $1.0$ & $3.6$  &       &       \\
 \hline
 \end{tabular}
              }
       {Variational MG\@:
        Dependences on $\delta$ and $\omega$ in four-dimensional pure
        gauges for $m^2 = 0.01$.
        For $\delta = 0$ one has the traditional one-grid algorithms.
        ``div.''\ means that the algorithm diverges.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 We anticipate (cf.\ Sec.~\ref{SecFreePropagators7})
 that the parameter $\delta$ need not be introduced
 when the improved correction scheme \equ{ImprovedCorr} is used.
 There the $\Nc \times \Nc$ matrix $\Theta$ takes the role of the
 real number $\delta$.
 The scheme \equ{ImprovedCorr} has the advantage that $\Theta$ need not
 be chosen by hand, rather it is determined by the algorithm itself
 through the requirement of minimalization of the energy functional
 \equ{EnergyFunctional}.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Optimal Multigrid}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl Optimal Multigrid}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 When no gauge fields are present, the lowest mode of $-\Delta$
 is a constant.
 In this case the simple variational MG scheme is successful, because
 then $\Cstar$ interpolates the lowest mode of $-\Delta$ correctly.
 The same is true for the optimal $\A$, since it fulfills
 $(L_b a)^4 \sum_{y \in \Lone} \A (z,y) = 1$ for all $z \in \Lnull$
 (Eq.~\equ{CorrectConstant} in Appendix~\theappKernels).
 In the trivial case $U = \bbbone$ the interpolation of a constant
 function on $\Lone$ with this $\A$ is unnecessarily complex, because
 there are nonvanishing contributions from all $y \in \Lone$.
 However, it will be shown in the following sections that indeed more
 complicated choices of $D_1$ {\em and} of the interpolation map $\A$
 are necessary to eliminate CSD in nontrivial gauge fields.

 Numerical results with the optimal MG scheme are as follows.
 Compared with variational MG, the convergence rate in trivial gauge
 fields is not improved in case of Jacobi relaxation, but convergence
 speed is doubled in case of SOR\@.
 Results with lexicographic SOR are contained in Table~$5.2$
 of the next section.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsectiontocentry{Importance of (Almost) Correct Interpolation
                     of the Lowest Mode}
                    {Importance of (Almost) Correct Interpolation
                     \protect\\ of the Lowest Mode}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl Importance of (Almost) Correct
                                      Interpolation of the Lowest Mode}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 We have just argued that variational MG with piecewise-constant
 interpolation works only because it interpolates the lowest mode
 of $-\Delta$ correctly.
 The relevance of the lowest eigenvector was also pointed out by
 Edwards~\cite{Edw}.
 {}From the marriage of MG with neural net methods~\cite{HerKroPal}
 one obtains a similar conclusion
 \cite{MacKalPalSpe,BaeKalMacSpe,MacSpe,Bae}.
 It follows from neural net optimization criteria that the interpolation
 kernel $\A$ should have the property that the lowest eigenmode
 $\phi_0$ of $D_0 = D$ should admit a representation of the form
 $\phi_0 = \A \Phi$ with a suitable $\Phi$ to a good accuracy.

 The (adjoint of the) kernel \equ{CwithoutGF} fulfills this requirement.
 The alternative proposal of \cite{KalNP2}, to define $\A$ through the
 eigenvalue equation \equ{EVequationC} with $\LAPN$ \equ{LAPN}
 replaced by $\LAPD$ \equ{LAPD} does not meet this requirement.
 The lowest mode of the negative Laplacian with Dirichlet boundary
 conditions on boundaries of blocks~$x$ $-\LAPD$ is a (lattice) sine
 wave, namely $\mbox{{\em const}}\,\prod_{\mu} \sin\left(\frac{\pi
 z_{\mu}/a}{\L +1} \right)$, $z_{\mu} = 1 , \ldots , \L$.
 Only for block size $\L = 2$ is this a constant on blocks, as in case
 of Neumann boundary conditions.

 Numerical results confirm the theoretical considerations.
 If one uses the lowest mode of $-\LAPD$ for interpolation, CSD in
 the computation of free propagators is not eliminated.
 (Remember that we chose $\L = 3$.)
 The critical exponent $z$ retains its value of~2.

 In Sec.~\ref{SecApproxA} numerical computations will be reported
 which show that CSD in computations of free propagators can be
 eliminated, even if the lowest mode of $-\Delta$ is {\em not}
 interpolated exactly.
 Therefore the above mentioned requirement that $\phi_0 = \A \Phi$ with
 a suitable $\Phi$ ``to a good accuracy'' does not mean
 ``exactly''.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsectiontocentry{Updating on a Multigrid Layer Consisting of a
                     Single Site and Related Improvements}
                    {Updating on a Multigrid Layer Consisting of a
                     Single Site \protect\\
                     and Related Improvements
 \label{SecFreePropagators7}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Free Propagators}}
          {{\rm\thesubsection.}\ {\sl Updating on a Single-Site MG
                                        Layer and Related Improvements}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%..............
 \Subsubsection{MG algorithms}
%..............
 By including the rescaling \equ{rescaleBOSE} in MG algorithms
 the performances are not improved any further, neither in variational
 MG nor in optimal MG\@.
 The improved correction scheme \equ{ImprovedCorr}, however, is able
 to halve $\tau$ and to bring it close to 1.
 Note that the parameter $\delta$ of \equ{delta} is eliminated
 when \equ{ImprovedCorr} is used.

%..............
 \Subsubsection{Conventional one-grid relaxation algorithms}
%..............
 By including \equ{rescaleBOSE} in conventional one-grid relaxation
 algorithms, CSD is eliminated in the sense that {\em asymptotic}
 relaxation times do not depend on $m^2$ (and on the lattice size).
 This is shown in Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
        {One-grid SOR plus \protect\equ{rescaleBOSE} eliminates CSD of
         {\em asymptotic} relaxation times, shown here for a pure gauge.
         ($\omega\!=\!1.90$, checkerboard updating)
         The six curves correspond to $m^2 = 0.1, 0.01, \ldots ,
         10^{-6}$ on a $12^4$ (non-stag\-ger\-ed) lattice, with $m$
         decreasing from left to right.
         A small volume effect remains, not for $\tau$ (i.~e.\ the
         asymptotic decay rate) but with respect to how long it takes
         until the asymptotic regime is reached: e.\ g.\ on an $18^4$
         lattice the number of iterations needed to obtain a given
         accuracy of $\| r \|$ for $m^2 = 10^{-6}$ is increased by
         $\sim 20$.
         The figure looks the same for bosons in nontrivial gauge
         fields when $m^2$ is replaced by $\protect\Dm$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 {\em The figure looks the same for bosons in nontrivial gauge
 fields when $m^2$ is replaced by $\protect\Dm$.}

 The norm of the residual is not monotonically decreased for small
 $m^2$.
 This feature also shows up in CG which minimizes the energy
 functional~$K$ (i.\ e.\ the residual $r$ in the norm induced by the
 scalar product $<\,\cdot\,,D^{-1}\,\cdot\,>$) rather than $|| r ||$
 itself (cf.\ Fig.~$4.1$).
 This is an interesting point:
 Instead of~\equ{rescaleBOSE}, one could think of rescaling $\phin$ by
 another matrix $\Omega'$ which is chosen such that not the energy
 functional but the norm of the residual $|| \rn ||$ is minimized.
 However, in this case there is no difference to one-grid relaxation.
 {\em This remains true in nontrivial gauge fields.}

 When one increases the lattice size there is a small volume effect
 with respect to how long it takes until errors decay exponentially;
 see caption of Fig.~\PreviousFig.
 However, the asymptotic slope of the curves is independent of
 $| \Lambda |$.
 Therefore it seems that CSD of {\em asymptotic} relaxation times is
 eliminated.

%..............
 \Subsubsection{Inefficiency of \equ{rescaleBOSE} as soon as errors
                decay exponentially}
%..............
 Finally we note that practically $\Omega = \bbbone$ as soon as
 $|| r ||$ decays exponentially.
 Then the step \equ{rescaleBOSE} could be switched off.
 {\em This statement holds also in nontrivial gauge fields and for MG
 algorithms.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \Sectiontocentry{Proof that the Multigrid Method Works in Disordered
                                     Systems}
                 {Proof that the Multigrid Method Works
                  \protect\\ in Disordered Systems
 \label{SecProof}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \markboth{{\rm\thesection.}\ {\sc Proof that the Multigrid Method Works
                                   in Disordered Systems}}{}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl This section contains the central result that the MG method
      works in disordered systems.}
%\smallskip

 \begin{quotation}
%..............
 \Subsubsection{Summary of results}
%..............
      MG computations of propagators in nontrivial gauge fields do not
      suffer from CSD, when the optimal interpolation kernel~$\A$
      and the optimal effective coarse grid operator are used.
      This statement is true for {\em any} value of the gauge coupling,
      including the case of completely random gauge fields ($\beta =0$).
      These computations were reported for the first time in
      Ref.~\cite{KalPL}.
      Unfortunately, the optimal MG scheme is not practical for
      production runs because of computational complexity and
      storage space requirements.
 \end{quotation}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Unpracticality of the Optimal $\A$ for Production Runs}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Proof that the Multigrid Method Works
                                   in Disordered Systems}}
          {{\rm\thesubsection.}\ {\sl Unpracticality of the Optimal $\A$
                                      for Production Runs}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The optimal interpolation kernel $\A (z,y)$ decays exponentially,
 but it is nonvanishing for all arguments $(z,y)$;
 cf.\ Figs.~$3.7$ and $3.8$, and the tables in Appendix~\theappKernels.
 When no gauge fields are present $\A$ is translational invariant, but
 this is no longer true in nontrivial gauge fields.
 Therefore storage of this kernel in a computer requires $\Nc^2 \cdot
 | \Lnull | \cdot | \Lone |$ numbers.%
 \footnote{In case of staggered fermions, one can halve this number
           because the even and odd sublattices are not coupled both
           for the Laplacian and for the Diracian choice of the
           averaging kernel~$C$.
           Nevertheless, the storage space requirement is still much too
           large.\label{footnote17}}
 Needless to say that because of this and computational complexity
 the use of the ideal MG algorithm is not practical for production runs.
 However, it is very important to answer questions of principle.
 Therefore the optimal MG scheme was implemented, and tested for bosonic
 propagators on $9^4$ lattices.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Computation of Optimal Interpolation Kernels $\A$}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Proof that the Multigrid Method Works
                                   in Disordered Systems}}
          {{\rm\thesubsection.}\ {\sl Computation of Optimal
                                      Interpolation Kernels $\A$}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The MG method is of interest near criticality, i.\ e.\ for slowly
 decaying propagators.
 For nontrivial gauge fields we have to enforce slow decay by choosing
 $m^2$ negative and very close to the negative of the lowest eigenvalue
 $-\mcr > 0$ of $-\Delta$.
 Values of $\mcr$ were determined by inverse iteration to an accuracy of
 $10^{-7}$ or better (this can be seen from the data in Fig.~$6.4$
 of Sec.~\ref{SecBosonicPropagators}).
 For each investigated gauge field configuration one $\A$-kernel was
 computed as the solution of the equation
%------------------- equation ------------------------------------------
 \begin{equation}
  \left( [ - \Delta + \mcr + \kappa\,\Cstar C ] \A \right) (z,y)
  = \kappa\,\Cstar (z,y)
 \label{BoseA}
 \end{equation}
%------------------- equation ------------------------------------------
 for large $\kappa$\,; cf.\ Eqs.~\equ{optimalA}, \equ{A}.
 This equation was solved by means of CG\@.
 In practice $\kappa$-independence is reached for $\kappa \gsim
 O(10^4)$.

 {\em Actually, one should compute and use a new $\A$-kernel for each
     different value of $m^2$. i.\ e.\ one should have $m^2$ in place of
     $\mcr$ in Eq.~\equ{BoseA}.
     But it turned out that it is sufficient to use the ``critical''
     $\A$-kernel \equ{BoseA} for any $m^2 > \mcr$.}
 This $\A$ was computed for $SU(2)$ gauge fields on $9^4$ lattices
 at $\beta = \infty$, $2.7$, $2.5$, $2.2$, $1.8$, and~$0$.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Numerical Results of the Idealized Multigrid Algorithm}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Proof that the Multigrid Method Works
                                   in Disordered Systems}}
          {{\rm\thesubsection.}\ {\sl Numerical Results of the Idealized
                                      Multigrid Algorithm}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 Propagators $(-\Delta + m^2)^{-1}$ were computed for values of
 $m^2$ close to criticality,
 $m^2 = \mcr + \Dm$, $\Dm = 1$, $0.1$, $0.01$, $\ldots$ , $10^{-6}$.

 It turned out that {\em CSD is completely eliminated at any value of
 $\beta$} (i.~e.\ also in completely disordered gauge fields)
 when $D_1 = C D_0 \A \equiv \Astar D_0 \A$ {\em and} $e_1$ is
 interpolated by $\A$.
 Results are in Table~\NextTable\ and Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|c|c|c|c|}
 \hline
 $\beta$ & $\mcr$ & optimal $\omega$ & $\tau$ for $\Dm \leq 10^{-3}$ \\
 \hline\hline
 $\infty$ & $0$          & $1.27$ & $1.6$ \\
 \hline
 $2.7$    & $-0.8210607$ & $1.38$ & $1.9$ \\
 \hline
 $2.5$    & $-0.9477085$ & $1.40$ & $1.9$ \\
 \hline
 $2.2$    & $-1.2218471$ & $1.45$ & $1.9$ \\
 \hline
 $1.8$    & $-1.7567164$ & $1.57$ & $2.5$ \\
 \hline
 $0$      & $-2.7480401$ & $1.69$ & $5.2$ \\
 \hline
 \end{tabular}}
       {Results of the idealized MG algorithm with lexicographic SOR
        for bosonic propagators in six different gauge field
        configurations on $9^4$ lattices $\Lnull$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
         {Convergence of the optimal MG algorithm for bosons on $9^4$
          lattices in quenched $SU(2)$ gauge fields at $\beta =
          \infty$, $2.7$, and $0.0$.
          The curves shown for each $\beta$-value correspond from left
          to right to $\Dm = 0.1$, $\Dm \leq 0.01$ for $\beta = \infty$
          and $\beta = 2.7$, and to $\Dm = 0.1$, $\Dm = 0.01$, $\Dm
          \leq 0.001$ for $\beta = 0.0$.
          The relaxation parameter $\omega$ has the optimal value
          quoted in Table~\PreviousTable.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 In order to be sure about the correct determination of $\mcr$\,, it was
 checked that simple one-grid relaxation algorithms exhibited CSD with
 $z=2$, i.~e.\ relaxation times diverged proportional to $1/\Dm$.
 It was also checked that the coarse grid operator $C D_0 \A$ with the
 optimal $\A$ is indeed Hermitean and equals $\Astar D_0 \A$\@.
 Numerical inaccuracies (round-off errors) are less than $10^{-9}$.

 The dependence of relaxation times on $\omega$ is shown in
 Table~\NextTable.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|c||r|r|r|r|r|r|r|r|r|r|}
 \hline
 $\omega$ &                 $1.0$ & $1.1$ & $1.2$ & $1.3$ & $1.4$ &
                            $1.5$ & $1.6$ & $1.7$ & $1.8$ & $1.9$ \\
 \hline\hline
 $\tau (\beta = \infty )$ & $2.8$ & $2.4$ & $2.0$ & $1.6$ & $1.9$ &
                            $2.4$ & $3.1$ & $4.2$ & $6.2$ & $11.9$ \\
 \hline
 $\tau (\beta = 2.7    )$ & $4.6$ & $3.8$ & $3.0$ & $2.4$ & $2.0$ &
                            $2.4$ & $3.0$ & $3.9$ & $5.5$ & $10.4$ \\
 \hline
 $\tau (\beta = 2.5    )$ & $4.6$ & $3.7$ & $3.0$ & $2.3$ & $1.8$ &
                            $2.2$ & $2.8$ & $3.8$ & $5.5$ & $10.4$ \\
 \hline
 $\tau (\beta = 2.2    )$ & $5.4$ & $4.4$ & $3.5$ & $2.8$ & $2.1$ &
                            $2.1$ & $2.6$ & $3.5$ & $5.1$ & $10.0$ \\
 \hline
 $\tau (\beta = 1.8    )$ & $8.6$ & $7.2$ & $6.0$ & $4.8$ & $3.8$ &
                            $2.9$ & $2.4$ & $3.2$ & $5.0$ & $10.2$ \\
 \hline
 $\tau (\beta = 0.0    )$ &$19.9$ &$16.4$ &$13.4$ &$10.9$ & $8.7$ &
                            $6.7$ & $5.0$ & $4.1$ & $7.7$ & div.   \\
 \hline
 \end{tabular}}
       {Dependence of relaxation times $\tau$ on $\omega$ in the
        ideal MG algorithm with lexicographic SOR for computing bosonic
        propagators on $9^4$ lattices with $\Dm = 0.01$.
        The algorithm does not converge for $\omega = 2.0$, and for
        $\omega = 1.9$ at $\beta = 0$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 This dependence is weak\-er than in variational MG, cf.\
 Sec.~\ref{SecBoseVMG}.

 {\em In order to be precise, it must be pointed out that the results
      reported here prove only that the idealized MG algorithm is able
      to eliminate the $1/\Dm$ divergence of relaxation times on
      lattices of a fixed size.
      However, we believe that no volume dependence would emerge
      if one were able to implement the optimal MG scheme on larger
      lattices.
      This belief is based on the fact that with the idealized MG
      algorithm the convergence behavior in nontrivial gauge fields
      is nearly the same as convergence in pure gauges.
      Exponential decay of errors sets in after only a few iterations.
      In pure gauges no volume dependence of convergence was found.
      Therefore it is reasonable to expect the same result for the
      idealized MG method.}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Implications of the Numerical Results}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Proof that the Multigrid Method Works
                                   in Disordered Systems}}
          {{\rm\thesubsection.}\ {\sl Implications of the Numerical
                                      Results}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The result that CSD is completely eliminated in the idealized MG
 algorithm proves three things:
 \begin{itemize}
  \item[(i)] {\em The MG method can cope in principle with the
              frustration (disorder) which is inherent in non-Abelian
              gauge fields.}
  \item[(ii)] {\em There exists an appropriate notion of smoothness
               in disordered cases as described in
               Sec.~\ref{SecSmoothness}}.
               The ideal $\A$ is the smoothest kernel which obeys
               $C \A = \bbbone$.
  \item[(iii)] {\em Ground-state projection is a good choice of $C$
               (i.~e.\ of a smooth block spin of the low frequency
               components) in gauge theories}.
              This statement is now confirmed directly from MG
              computations, not only from the point of view of the
              renormalization group as argued in Sec.~\ref{SecOptA}.
 \end{itemize}

 The success of the idealized MG algorithm is especially remarkable
 in view of the fact that variational MG is not able to
 eliminate CSD in nontrivial gauge fields.
 This will be shown in Secs.~\ref{SecBoseVMG} and \ref{SecFermiVMG}.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Approximations to the Idealized Multigrid Algorithm}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Proof that the Multigrid Method Works
                                   in Disordered Systems}}
          {{\rm\thesubsection.}\ {\sl Approximations to the Idealized
                                      Multigrid Algorithm}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 It was found that the convergence speed of MG is very sensitive to
 details of the interpolation.
 Typically CSD is not eliminated in nontrivial gauge fields when not
 all ingredients are optimal.
 Choosing either%
 \footnote{Cf.\ Eq.~\equ{delta}, no damping parameter $\delta$ is
           required in the optimal MG scheme.}
 $D_1 = \delta^{-1} C D_0 \A$ but using $\Cstar$ instead of $\A$ for
 interpolation, or approximating $D_1 = \delta^{-1} C D_0 \Cstar$ but
 retaining $\A$ for interpolation, both fail to eliminate CSD at finite
 $\beta$.
 This is unlike the case $\beta = \infty$, where also these
 two modifications of the idealized algorithm succeed in fighting CSD.

 For the question of approximations to the ideal $\A$ with a finite
 support (truncating the exponential tails) we refer to
 Sec.~\ref{SecApproxA}.

 We remark that in our computations where we used only one
 $\A$-kernel for all values of $m^2$, the correctness of the value of
 $\mcr$ in Eq.~\equ{BoseA} has influence on the performance.
 For instance, if one replaces $\mcr$ in \equ{BoseA} by $\mcr \pm 0.01$,
 relaxation times stay constant and short for $\Dm \geq 10^{-3}$,
 but the algorithm diverges for $\Dm \leq 10^{-4}$.
 (In these investigations we used the coarse grid operator $\Astar D_0
 \A$).
 Recall, however, the remark about the mass term after Eq.~\equ{BoseA}.
 A priori one can only hope for elimination of CSD when $\A$ is
 computed with the correct $m^2$.
 Yet, if one were able to employ the idealized MG algorithm for
 production runs one would have a fixed $m^2$, and therefore one would
 solve Eq.~\equ{BoseA} with this $m^2$.
 As a result, there is no problem with the choice of the mass in $\A$
 and CSD would always be eliminated in practice.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Idealized Multigrid Algorithm for Staggered Fermions}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Proof that the Multigrid Method Works
                                   in Disordered Systems}}
          {{\rm\thesubsection.}\ {\sl Idealized Multigrid Algorithm for
                                      Staggered Fermions}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The idealized MG algorithm has not been implemented yet for
 staggered fermions.
 There the computational complexity and the storage space requirement
 are even larger than for bosons.
 We mentioned in footnote~{\protect\small\ref{footnote17}} that one can
 halve the required storage space in case of fermions compared with
 bosons.
 On the other hand, effectively fermionic lattices need to be larger by
 a factor of~16.
 Nevertheless, in order to answer questions of principle also for
 fermions, idealized MG computations are planned for the near future.
 We have little doubt that they will be as successful as the bosonic
 computations reported here.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \Sectiontocentry{Computation of Gauge Covariant Bosonic Propagators
                  \protect\\ in Four-Dimensional
                  \mbox{\protect\boldmath $SU$}(2) Gauge Fields}
                 {Computation of Gauge Covariant Bosonic \protect\\
                  Propagators in Four-Dimensional
                  {SU}\/(2) Gauge Fields
 \label{SecBosonicPropagators}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
                              {}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl We turn now to practical algorithms for bosonic propagators.
      First we look at the CG algorithm, and at one-grid relaxation
      methods.
      The MG methods discussed thereafter are: $(i)$ variational MG,
      $(ii)$ algorithms with approximations to the ideal $\A$-kernel,
      $(iii)$ inclusion of updating on an MG layer consisting of a
      single site, and $(iv)$ the related improvements of
      Sec.~\ref{SecRelatedImpr}.
      There is also a subsection with a remark concerning the use of
      SOR in MG computations.}
 \medskip

 \begin{quotation}
%..............
 \Subsubsection{Summary of results}
%..............
 The CG algorithm is very sensitive to the disorder in the gauge field.
 For a given value of $\Dm$, CG needs more iterations to converge to
 a given precision the more disordered the gauge field becomes.

 The theoretical considerations of Sec.~\ref{SecCSD1grid} predict
 that this is different in conventional one-grid relaxation
 algorithms.
 This prediction could be confirmed numerically.
 In one-grid relaxation methods convergence is almost the same, no
 matter how strong the disorder of the gauge field is, as long as equal
 values of $\Dm$ are compared.
 There is also no volume dependence in practice, whereas at fixed
 $\beta$ and fixed $\Dm$ CG needs more iterations to converge the
 larger the lattice size is.

 The variational MG algorithm is sensitive to the disorder of the
 gauge field, but not as strongly as the CG algorithm.
 Convergence of variational MG does not only depend on $\Dm$, but also
 on $\beta$ and on the lattice size.
 In contrast to the case of pure gauges, variational MG is not able
 to eliminate CSD in nontrivial gauge fields.
 However, the variational MG method considered here is able to
 outperform the CG algorithm in CPU time on lattices $\gsim 18^4$.

 An MG algorithm with an ``approximated optimal'' interpolation
 kernel~$\A$ was tested.
 This $\A$-kernel does not fulfill the requirement that it interpolates
 the lowest mode of the Laplacian correctly.
 Despite this, CSD is completely eliminated in trivial gauge fields.
 Hence, for the success of an MG algorithm it is not a necessary
 condition that the lowest mode is interpolated exactly.
 The result might be taken as an indication that an overlap of blocks
 is more important.
 However, in nontrivial gauge fields CSD is not eliminated with
 the approximated $\A$-kernel.

 The inclusion of ``updating on a last site'' as discussed in
 Sec.~\ref{SecLP} leads to a method which eliminates CSD  of
 {\em asymptotic\/} relaxation times.
 What remains, however, is a small volume effect with respect to
 how long it takes until errors decay exponentially.

 The implementation of the further related improvements of
 Sec.~\ref{SecRelatedImpr} does not pay.
 \end{quotation}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{The Competitor: Conjugate Gradient Algorithm
 \label{SecCGBosons}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
          {{\rm\thesubsection.}\ {\sl The Competitor: Conjugate
                                      Gradient Algorithm}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The algorithm which is to be beaten is CG \equ{CG}.
 Its behavior in case of bosonic propagators is shown in
 Fig.~\NextFig\ where we compare convergence at $\beta = \infty$
 with $\beta = 2.7$.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{8.6cm}
         {Convergence of CG for bosonic propagators
          $(-\Delta + \mcr + \Dm )^{-1}$ on an $18^4$ lattice.
          Curves of open symbols are results of computations in a pure
          gauge field ($\mcr = 0$), while curves of solid symbols are
          obtained in the background of a quenched $SU(2)$ gauge field
          at $\beta = 2.7$. ($\mcr = -0.7554339$.)
          Within each of the two families the curves are parameterized
          by $\Dm = 1, 10^{-1}, \ldots , 10^{-6}$, with $\Dm$ decreasing
          from left to right
          The initial guess for the propagator is zero in all cases.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 No preconditioning is employed.

 Recall what was said in Sec.~\ref{SecCGPG} about the convergence for
 small values of $m^2$, or $\Dm$ respectively.
 The norm of residuals is not necessarily decreased monotonically.
 The volume effect which was mentioned in Sec.~\ref{SecCGPG} is larger
 the smaller $\beta$ becomes.
 For fixed $\beta$ and fixed $\Dm$, CG needs longer to converge
 the larger the lattice size is.

 Also, the CG algorithm is very sensitive to the disorder in the gauge
 field.
 For a given value of $\Dm$, CG needs more iterations to converge to
 a given precision the more disordered the gauge field becomes.
 It is worth to emphasize that this is not the case in
 conventional one-grid relaxation algorithms.
 There convergence is practically the same, no matter how strong the
 disorder of the gauge field is, as long as equal values of $\Dm$ are
 compared.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{One-Grid Relaxation Algorithms
 \label{SecBose1Grid}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
          {{\rm\thesubsection.}\ {\sl One-Grid Relaxation Algorithms}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 Values of $\tau$ for relaxations on a single grid
 (Sec.~\ref{SecCSD1grid}) agree extremely well with our numerical
 results, also in nontrivial gauge fields at various values of $\beta$.

 In particular, it must be emphasized again that one-grid relaxation
 algorithms are nearly insensitive to the disorder of the gauge field.
 Their convergence behavior depends only on the value of~$\Dm$.
 There is also practically no dependence on the lattice size.
 Cf.\ the discussion in Sec.~\ref{SecCSD1grid}.

 As an example for the numerical verification of another theoretical
 prediction we quote the following.
 Remember the prediction for SOR (page~\pageref{SORprediction}):
 $\omega = 1.91$ is optimal for $\Dm \sim 0.009$.
 Hence, $\tau = -1.0 / \ln (0.91) = 10.6$ for $\Dm \geq 0.009$,
 and one has CSD with $z=2$ for smaller values of $\Dm$.
 This behavior shows up in a distinct way in the data presented in
 Fig.~$6.4$ below.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Variational Multigrid
 \label{SecBoseVMG}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
          {{\rm\thesubsection.}\ {\sl Variational MG}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

%..............
 \Subsubsection{Existing literature}
%..............
 The most practical MG method is variational coarsening (sometimes
 called ``Galerkin definition''), because in this method coarse grid
 operators retain the property that at most nearest neighbors are
 coupled.
 For this reason variational MG is by far the most popular MG method.
 It is used exclusively in the literature
 \cite{BenBraSol,BRVGSP,HaretalLAT90,HSVLAT90,HSVNP,BRVvariational,%
      BMRV,Benetal,Vya,HSVJulich,BERV,Vin,Hulthesis,Benthesis,VinLAT91,%
      PTMG_GMD,LauWit,VyaSU3}.

 Ground-state projection MG computations for propagators were done
 before in two-\-di\-men\-sion\-al $U(1)$ \cite{BRVGSP,HSVLAT90,HSVNP}
 and (approximate ground-state projections with gauge fixing) in
 two-dimensional and four-dimensional $U(1)$, and two-dimensional
 $SU(2)$ gauge fields
 \cite{BRVvariational,BMRV,HSVJulich,BERV,Vin,VinLAT91}.
 The first ground-state projection MG computation of gauge covariant
 propagators in four-dimensional non-Abelian gauge fields (for gauge
 group $SU(2)$) was presented by the present author in
 Ref.~\cite{KalPL}.
 Besides ground-state projection there are two other approaches for
 choosing the averaging kernel $C$.
 One alternative approach is called ``parallel transported MG''\@.
 It is based on the representation~\equ{SumofPaths} and was studied
 in Refs.~\cite{BenBraSol,HaretalLAT90,Benetal,PTMG_GMD,LauWit}
 by Ben-Av et al.
 The second alternative approach is pursued by Vyas \cite{Vya,VyaSU3}.
 He determines $C$ by means of a Migdal-Kadanoff renormalization
 group transformation.

%..............
 \Subsubsection{Gauge covariant procedure of the present work}
%..............
 In all computations reported in this thesis exact ground-state
 projecting averaging kernels $C$ were used exclusively.
 The advantage of this procedure is that no gauge fixing is necessary,
 because the method is gauge covariant.
 The algorithm for computing $C$ on the whole lattice
 (Sec.~\ref{SecAlgorithmC}) is so efficient that it merely costs CPU
 time of the order of one heat bath sweep for the gauge field.
 [Cf.\ Sec.~\ref{SecAlgorithmC}.
  It might well be that the eigenvalue equation is solved well enough
 with fewer CG iterations; however, this question has not been
 investigated.]
 Thus, it is not too expensive to solve~\equ{EVequationC}, and it is not
 necessary to sacrifice gauge covariance by working with gauge field
 independent kernels in gauge-fixed $U$-configurations.
 (Gauge fixing costs also CPU time.)

 \smallskip
 Numerical work was done on $9^4$, $12^4$, and $18^4$ lattices $\Lambda$
 with $SU(2)$ gauge fields at various values of~$\beta$.
 The computational details mentioned in
 Sec.~\ref{SecComputationalDetails} apply here as well.
 The definition of the Galerkin operator contains the factor $\delta$
 which was introduced in~\equ{delta}.

%..............
 \Subsubsection{Numerical results}
%..............
 Optimum values of $\omega$ and $\delta$ are:
 $(i)$ $\beta = 10.0$\,: $\delta \sim 2.3$, $\omega \sim 0.99$, $0.96$,
       $1.25$ for MG Jacobi on a $9^4$, on an $18^4$, and for MG SOR on
       an $18^4$ lattice, respectively.
 $(ii)$ $\beta = 2.7$\,: $\delta \sim 2.8$, $\omega \sim 0.99$, $0.99$,
        $1.51$ for algorithms as above.
 These values were determined at $\Dm = 0.01$ and retained for all
 values of $m^2$.

 For pure gauges, performance of the MG schemes depends little on
 $\delta$ (cf.\ Table~$4.2$), but for disordered gauge fields the
 relaxation time decreased with increasing $\delta$ up to a maximum
 value where the MG algorithms start to diverge suddenly.
 Also, in nontrivial gauge fields relaxation times in variational MG
 are stronger dependent on $\omega$ than in case of free propagators.
 Examples are in  Table~\NextTable;
 see also the remarks in Sec.~\ref{SecRemarkSOR} below.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|c||r|r|r|r|r|r|r|}
 \hline
 \multicolumn{8}{|c|}{Dependence on $\delta$} \\
 \hline
 $\delta$ &                 $0.45$ & $0.9$ & $1.35$ & $1.8$ & $2.25$ &
                            $2.7$ & $3.15$ \\
 \hline
 $\tau (\beta = 2.7 , \omega = 1.0 )$
                          &$83.8$ &$62.1$ &$51.0$ &$45.0$ &$40.5$ &
                           $37.7$ & div.  \\
 \hline\hline
 \multicolumn{8}{|c|}{Dependence on $\omega$} \\
 \hline
 $\omega$ &                 $1.0$ & $1.1$ & $1.2$ & $1.3$ & $1.4$ &
                            $1.5$ & $1.6$ \\
 \hline\hline
 $\tau (\beta = 2.7 , \delta = 2.9)$
                          &$37.0$ &$29.0$ &$22.3$ &$16.5$ &$11.3$ &
                            $6.0$ & div.  \\
 \hline
 \end{tabular}}
       {Dependence of relaxation times $\tau$ on $\delta$ and on
        $\omega$ in variational MG SOR for computing bosonic
        propagators on $18^4$ lattices with $\Dm = 0.01$.
        ``div.'' means that the algorithm does not converge.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 In Figs.~\NextFig\ and \NextNextFig\ we compare the approach to
 convergence of three one-grid algorithms, namely damped Jacobi (Jac),
 SOR and CG, and two versions of twogrid cycles, MG Jacobi and MG SOR\@.
 Values of $\omega$ and $\delta$ in MG algorithms are the optimal ones
 as given above, and $\omega = 0.99$ in one-grid Jacobi, $\omega =
 1.91$ in one-grid SOR\@.
 In the literature, convergence is considered achieved when the
 natural logarithm of the RMS residual has gone down by 10
 \cite{BitetalLAT91}
 (dashed line in Figs.~$6.2$ and~$6.3$).
 It is seen that MG SOR outperforms CG, not only with respect to
 number of iterations, but also with respect to CPU time.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \DoubleFigure{12.0cm}
        {Computation of bosonic propagators $(-\Delta + \mcr + \Dm
         )^{-1}$:
         Convergence on an $18^4$ lattice in a quenched $SU(2)$ gauge
         field at $\beta = 10.0$, with $\mcr = -0.1533739$.
         (MG with $\A = \Cstar$.)}
              {12.0cm}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \DoubleFigure{12.0cm}
        {Computation of bosonic propagators $(-\Delta + \mcr + \Dm
         )^{-1}$:
         Convergence on an $18^4$ lattice in a quenched $SU(2)$ gauge
         field at $\beta = 2.7$, with $\mcr = -0.7554339$.
         (MG with $\A = \Cstar$.)}
              {12.0cm}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 Small values of $\Dm$ may seem to be of no practical importance
 on $18^4$ lattices because the correlation length determined by the
 propagator becomes comparable to or larger than the lattice extension.
 But it is nevertheless important to study very small $\Dm$ in order

 \clearpage
 to understand the operation and limits of the MG algorithms.
 We recall the remarks of Sec.~\ref{SecCautionaryRemark}.
 If one had a $1/\Dm$ divergence of relaxation times on lattices of
 fixed size with a constant of proportionality which is independent of
 $| \Lambda |$, one would be able to definitely predict non-reduction
 of CSD under conditions where $1/\triangle m$ and the lattice size
 are changed proportionally.

 In one-grid relaxation algorithms it was found that convergence
 at fixed $\Dm$ does practically not depend on $\beta$ and on the
 lattice size~$| \Lambda |$.
 Whether this continues to hold for MG relaxation algorithms was
 investigated numerically.
 The result is that at fixed $\beta$ convergence of MG is not
 independent of the lattice volume.
 However, no common trend was found how the convergence speed in number
 of iterations behaves at fixed values of $\Dm$ and $\beta$ when $|
 \Lambda |$ is increased.

 In contrast to relaxation on one grid, it was also found numerically
 that the variational MG method is sensitive to the disorder of the
 gauge field.
 Convergence speed depends also on $\beta$, see below.

 In Fig.~\NextFig\ the relaxation times for various algorithms are shown
 as a function of $\Dm$, at $\beta = 2.7$.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
        {Computation of bosonic propagators $(-\Delta + \mcr + \Dm
         )^{-1}$:
         Relaxation times $\tau$ (in comparable work units) of
         iterative algorithms on an $18^4$ lattice in a quenched $SU(2)$
         gauge field at $\beta = 2.7$  with $\mcr = -0.7554339$.
         (MG with $\A = \Cstar$).}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 One sees that CSD  is not eliminated in the MG modes.
 This is unlike the pure gauge case, Sec.~\ref{SecFreePropagators4}.
 The relaxation time behaves like $\tau \propto (\Dm)^{-z/2}$
 with $z=2$ both for MG Jacobi and MG SOR\@.
 One could think of adjusting the mass term in $D_1$, but it turned out
 that this leads to no more than a $\sim 5 \%$ acceleration of
 convergence.

 At $\beta = 10.0$ the same qualitative behavior was found as in
 Fig.~\PreviousFig.
 Computations at other values of $\beta$ down to $2.2$ were also done.
 Surprisingly it was found that the value of $\Dm$ at which
 CSD sets in (i.\ e.\ $\tau$ starts to increase) depends little
 on $\beta$.
 This contradicts the scaling hypothesis of~\cite{BERV}.
 Basically the only dependence on $\beta$ was found for the constant
 of proportionality in the scaling relation of $\tau$.
 Compared with $\beta = 2.7$, its value is nearly doubled for $\beta =
 2.2$, and roughly reduced by a factor of 3 at $\beta = 10.0$.

%..............
 \Subsubsection{Conclusions}
%..............
 A tentative interpretation of the permanence of CSD might be
 as follows.
 $\mcr$ is a natural gauge invariant measure of smoothness
 as discussed in Sec.~\ref{SecSmoothness}.
 For $\beta \leq 10$ the lowest eigenvalue $-\mcr$ of $-\Delta$ appears
 to be too large to consider any function as smooth (cf.\ Fig.~$3.9$).
 Therefore the basic hypothesis of the MG method, namely smoothness
 of the slow modes, is not fulfilled, and therefore one cannot
 expect MG to work in an optimal fashion.
 There would be no problem if one had restricted attention to
 propagators $(-\Delta + m^2 )^{-1}$ with $m^2 \geq 0$.
 This propagator is critical only when $-\Delta$ has a very low
 eigenvalue, and then smooth functions exist.
 One might believe that basically one is paying the prize for having
 introduced criticality artificially into a frustrated system.
 However, the investigations with the optimal interpolation kernel
 $\A$ which were reported in Sec.~\ref{SecProof} showed that this is
 not the case.
 It seems that the variational MG method considered here is simply a
 too crude scheme in nontrivial gauge fields.

 It would be interesting to investigate the question whether the
 situation improves when one uses overlapping blocks.
 Hasenbusch and Meyer found in their MG Monte Carlo
 simulations of two-dimensional asymptotically free models
 \cite{HasMey} that it is essential for the elimination/reduction of CSD
 to use overlapping blocks.
 However, in gauge theories one has to take into account that the
 storage space requirements and computer time grow when blocks overlap.
 For this reason, a systematic investigation of the simpler schemes
 without overlap was done and is reported here.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsectiontocentry{A Remark Concerning the Use of SOR in Multigrid
                     Computations}
                    {A Remark Concerning the Use of SOR \protect\\
                     in Multigrid Computations
  \label{SecRemarkSOR}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
          {{\rm\thesubsection.}\ {\sl A Remark Concerning the Use of
                                      SOR in MG Computations}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 We remark that the use of a relaxation parameter $\omega \neq
 1$ in MG computations contradicts the conventional wisdom.
 According to this wisdom the only job of the relaxation procedure
 on $\Lnull$ is to smoothen the error, and this job is perfectly done
 by Gauss-Seidel or plain Jacobi iteration.

 This conventional wisdom is confirmed by numerical results in trivial
 gauge fields.
 However, the finding of the present thesis is that the picture
 changes in nontrivial gauge fields.
 In case of Jacobi relaxation one does in fact gain nothing (or very
 little) when $\omega$ is chosen different from 1 or $0.99$.
 But in case of SOR any over-relaxation in nontrivial gauge fields
 yields better performance than Gauss-Seidel, and much better
 performance than Jacobi or the minimal residual algorithm.
 A similar finding was reported in works on MG gauge fixing
 \cite{deForGup,HulLauSmi}.

 We refer to Tables~$4.2$, $5.2$, and $6.1$ for numerical results.
 Note that the idealized MG algorithm follows the conventional MG
 wisdom closer than variational MG\@.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Approximations to the Optimal Interpolation Kernel
 \label{SecApproxA}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
          {{\rm\thesubsection.}\ {\sl Approximations to the Optimal
                                      Interpolation Kernel}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The conclusion which can be drawn from the results of
 Secs.~\ref{SecProof} and~\ref{SecBoseVMG} is that one should find
 a compromise between the ideal MG algorithm and variational coarsening.
 One may try to approximate the optimal $\A$-kernel by a simpler choice
 with a finite support, i.\ e.\ one wants a kernel which fulfills
 $\A(z,x)=0$ for $z\not\in$ a certain neighborhood of block $x$.
 This neighborhood might be taken to be only the block $x$ itself;
 cf.\ the practicality condition \equ{practicality}.
 The coarse grid operator would be defined through $D_1 = \Astar D_0
 \A$.

%..............
 \Subsubsection{Naive attempt}
%..............
 A first very naive guess is to take simply the optimal $\A$ and to
 truncate it, i.\ e.\ setting $\A (z,y) = 0$ by hand for $a^{-1} | z -
 \hat{y} | > n$ where $n$ is some small integer number.
 (The ``taxi-driver'' norm $|\,\cdot\,| = \|\,\cdot\,\|_1$ is used.)
 However, this procedure fails.
 The explanation for the failure appears simple.
 We argued that in the absence of gauge fields the validity of
 Eq.~\equ{CorrectConstant} is a necessary condition for a successful MG
 algorithm for propagators.
 But this equation is violated when the optimal $\A$ is truncated,
 see Table~\NextTable.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|r||c|c|c|c|c|}
 \hline
  $n$ & $\geq 4$ & $3$ & $2$ & $1$ & $0$ \\
 \hline
  $\#$ blocks where $\A (z,x) \neq 0$ & $81$ & $65$ & $33$ & $9$ & $1$\\
 \hline
  $\d\max_{z\in\Lnull} | 1 - \int_x \A (z,x) |$ & $3.3 \cdot 10^{-10}$ &
  $4.3 \cdot 10^{-3}$ & $2.1 \cdot 10^{-2}$ & $6.2 \cdot 10^{-2}$ &
  $0.55$ \\
 \hline
 \end{tabular}}
       {Violation of Eq.~\protect\equ{CorrectConstant} on a $9^4$
        lattice in the absence of gauge fields, when the optimal
        $\A$-kernel is truncated at distance $n$, i.\ e.\ $\A (z,y) =
        0$ is set by hand if $a^{-1} | z - \hat{y} | > n$.
        The finite value for $n \geq 4$ is due to round-off errors.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 Also, by rude truncation the kernel loses its smoothness.

%..............
 \Subsubsection{The ``Ohrenkern''}
%..............
 As an alternative one may think of the following proposal which was
 made by Mack \cite{MacCargese}.
 We call this proposal ``Ohrenkern''.%
 \footnote{The author found no suitable translation for this German
           word.}
 It is defined as follows.
 Restrict the support of $\A (z,x)$ to block $x$ and its eight
 nearest neighbors, i.~e.\ $A (z,x) = 0$ unless $z \in x$ or $z \in$
 a nearest neighbor block of $x$.
 Compute an approximated interpolation kernel $\A$ as solution of
 Eq.~\equ{BoseA} with $\Delta$ replaced by the covariant Laplacian with
 Dirichlet boundary conditions on the boundary of the desired support
 of~$\A$.

 Intuitively, this $\A$ should be ``smoother'' than the truncated one.
 On the other hand the Ohrenkern also violates
 Eq.~\equ{CorrectConstant}.
 The violation is even larger than in case of the comparable
 truncated optimal $\A$-kernel ($n = 1$).
 One finds $\d\max_{z\in\Lnull} | 1 - \int_x \A (z,x) | =  9.95 \cdot
 10^{-2}$.

 The numerical result of computations of propagators is somewhat
 surprising.
 Despite violation of Eq.~\equ{CorrectConstant}, CSD is completely
 eliminated in trivial gauge fields.
 Hence, for the success of an MG algorithm it is not a necessary
 condition that the lowest mode is interpolated exactly.
 The result might be taken as an indication that an overlap of blocks
 is more important.
 However, CSD remains with the Ohrenkern in nontrivial gauge fields.

 Numerical values for the Ohrenkern in the absence of gauge fields
 are given in Table~B$.7$ of Appendix~\theappKernels.

 \smallskip
 The Ohrenkern was also used by Mack and Meyer \cite{MacCargese,MacMey}
 in MG simulations of $\phi^4$ theory.
 One might wonder whether their MG Monte Carlo simulations would have
 been more successful if they also tried the optimal $\A$-kernel.
 The answer to this speculation is probably negative.
 The analysis of Grabenstein and Pinn \cite{GraPin} indicates
 that CSD in $\phi^4$ theories cannot be beaten at all by MG algorithms
 (more precisely speaking, by the kind of unigrid algorithm they
 considered).

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsectiontocentry{Inclusion of Updating on a Multigrid Layer
                     Consisting of a Single Site}
                    {Inclusion of Updating on a Multigrid Layer
                     \protect\\ Consisting of a Single Site
 \label{SecLPbose}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
          {{\rm\thesubsection.}\ {\sl Inclusion of Updating on a
                                      Single-Site MG Layer}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%..............
 \Subsubsection{Conventional one-grid relaxation algorithms
                plus \equ{rescaleBOSE}}
%..............
 The remarks made in Sec.~\ref{SecFreePropagators7} about one-grid
 relaxation plus \equ{rescaleBOSE} apply in nontrivial gauge fields as
 well.
 Fig.~$4.2$ looks the same when $m^2$ is replaced by $\Dm$.
 At fixed lattice size $| \Lambda |$ the algorithm retains the property
 that it is practically not sensitive to the disorder of the gauge
 field, i.~e.\ convergence is only determined by $\Dm$, no matter what
 the value of $\beta$ is.
 However, there appears a volume effect, as stated in the caption
 of Fig.~$4.2$.

%..............
 \Subsubsection{MG algorithms plus \equ{rescaleBOSE}}
%..............
 Variational MG plus ``last point updating'' \equ{rescaleBOSE} seems to
 beat CSD of {\em asymptotic\/} relaxation times, too.
 Compared with CG and one-grid relaxation plus \equ{rescaleBOSE}, this
 modified MG performs better the more critical the system is.
 Convergence for $\Dm = 10^{-6}$ on $12^4$ and $18^4$ lattices is shown
 in Fig.~\NextFig.

 In a fixed volume the results for the $\Dm$-dependence of relaxation
 times in variational MG plus \equ{rescaleBOSE} look similar to those
 of one-grid plus \equ{rescaleBOSE}, except that fewer iterations are
 required to reach a given accuracy.
 The {\em asymptotic\/} slope of the curves is independent of $\Dm$ in a
 fixed volume.
 Fig.~$6.5$ shows that the asymptotic slope is also independent
 of the lattice size.
 {}From these findings we conclude, as in the case of trivial gauge
 fields, that {\em asymptotic} CSD seems to be eliminated.
 The volume effect with respect to how long it takes until errors
 decay exponentially is reasonably mild.

 It must be emphasized that $\Omega$ in \equ{rescaleBOSE} really needs
 to be a matrix.
 Simple rescaling of $\phin$ with a real number does not accelerate
 convergence.%
 \footnote{A remark about one-grid plus \equ{rescaleBOSE} is in order
           here:
           It can be proved by induction that in $SU(2)$ gauge fields
           $\Omega \propto \bbbone$ always holds if one starts
           relaxation with $\phi^{(0)} = 0$.
           However, $\Omega \propto \bbbone$ is not true in general.}

\clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
        {Convergence for bosonic propagators
         $(-\Delta + \mcr + \Dm )^{-1}$ with $\Dm = 10^{-6}$ in
         quenched four-dimensional $SU(2)$ gauge fields equilibrated
         with Wilson's action at $\beta = 2.7$.
         The numbers refer to the following algorithms:
         1/2: variational MG SOR ($\omega = 1.50$) plus
         \protect\equ{rescaleBOSE} on a $12^4$/$18^4$ lattice;
         3/4: one-grid SOR ($\omega = 1.91$) plus
         \protect\equ{rescaleBOSE} on a $12^4$/$18^4$ lattice;
         5/6: CG on a $12^4$/$18^4$ lattice.
         The critical masses are $\mcr = -0.7726281$/$-0.7554339$.
         Without \protect\equ{rescaleBOSE} MG SOR and one-grid SOR have
         relaxation times of $O(10^5)$ (Fig.~$6.4$).}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Inclusion of the Related Improvements of Section
             \protect\ref{SecRelatedImpr}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Bosonic Propagators}}
          {{\rm\thesubsection.}\ {\sl Inclusion of the Related
                                      Improvements of
                                  Section \protect\ref{SecRelatedImpr}}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The improved MG correction scheme \equ{ImprovedCorr} also beats CSD
 of asymptotic relaxation times.
 (Note that the parameter $\delta$ of \equ{delta} is eliminated
  when \equ{ImprovedCorr} is used.)
 However, at finite $\beta$ \equ{ImprovedCorr} is not able to halve
 relaxation times, in contrast to the trivial case.
 Therefore the increased computational labor does not pay.

 Another result with the improved coarse grid correction scheme
 \equ{ImprovedCorr} is the following.
 It was found that the performance of \equ{ImprovedCorr} with fixed
 $\Omega = \bbbone$ plus \equ{rescaleBOSE} is equivalent to
 \equ{ImprovedCorr} with automatic determination of $\Omega$\@.

 \smallskip
 Using the modified SOR version \equ{SOR} does not pay.
 If one fixes $\Xi = \bbbone$, one has nothing else but conventional
 Gauss-Seidel relaxation.
 Retaining $\Xi$ yields little difference in performance,
 because after a few iteration $\Xi \approx \bbbone$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \Sectiontocentry{Computation of Gauge Covariant Propagators
                  of Staggered Fermions \protect\\
                  in Four-Dimensional
                  \mbox{\protect\boldmath $SU$}(2) Gauge Fields}
                 {Computation of Gauge Covariant Propagators \protect\\
                  of Staggered Fermions \protect\\
                  in Four-Dimensional {SU}\/(2) Gauge Fields
 \label{SecFermionicPropagators}}
%                 \mbox{\protect\boldmath $SU$}(2) gauge fields}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}{}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl This section contains reports about computations of propagators
      of staggered fermions.
      We begin again with looking at the CG algorithm, and discuss
      one-grid relaxation algorithms after that.
      The MG methods discussed then are: $(i)$ variational MG,
      $(ii)$ a slightly different scheme with a non-Galerkin coarse
      grid operator, $(iii)$ inclusion of updating on an MG layer
      consisting of a single site, $(iv)$ modified minimal residual
      algorithms, and finally, $(v)$ we discuss the
      use of the $\sqrt{3}$ blocking scheme of Cordery, Gupta, and
      Novotny \cite{CorGupNov} in MG computations.
      In the section on point $(iii)$ we put special emphasis on the
      gauge covariance properties of the procedure.}

 \bigskip\noindent
 We recall that the computational details of
 Sec.~\ref{SecComputationalDetails} apply in this section as well.
 \newline
 If not stated explicitly, variational MG always means variational MG
 with the Laplacian choice of the averaging operator~$C$.
 \medskip

 \begin{quotation}
%..............
 \Subsubsection{Summary of results}
%..............
 The CG algorithm for propagators of staggered fermions shares the
 characteristic features with the bosonic case qualitatively.
 Quantitatively CG appears to be even more sensitive to the disorder of
 the gauge field.
 For given mass the convergence speed slows down considerable when
 $\beta$ is decreased, and when the lattice size is increased.

 For staggered fermions it was verified numerically that the scaling
 relation \equ{scalingtau} also holds for traditional one-grid
 relaxation algorithms, and for the variational MG algorithm with the
 Laplacian choice of~$C$.
 The critical exponent $z$ equals~2 (fixed~$\omega$).
 It was also verified numerically that the constant of proportionality
 in \equ{scalingtau} is {\em independent of the lattice size\/}.
 Hence, the two algorithms mentioned will have CSD under conditions
 where the inverse mass and the linear extension of the lattice are
 changed proportionally.

 The analytical predictions which can be made in case of traditional
 relaxation for bosonic propagators are not valid for staggered
 fermions (except Ostrowski's Theorem).
 In particular, the undamped Jacobi iteration does not converge in
 nontrivial gauge fields.
 This finding suggests that Jacobi is not a useful smoother in MG
 computations for fermionic propagators.

 Despite non-elimination of CSD, MG with variational coarsening works
 better than traditional relaxation methods, but on lattices up to
 $18^4$ this MG algorithm is not competitive with CG\@.
 We expect that the situation will be different on larger lattices.
 However, we cannot predict how large the lattices have to be.
 We speculate that $SU(2)$ gauge fields at realistic $\beta$-values
 are too disordered to make the Laplacian choice of the averaging
 operator~$C$ appropriate {\em in variational MG, i.~e.\ when
 $\A = \Cstar$\/}.

 An alternative definition of a coarse grid operator $D_1$ was
 investigated.
 In this alternative a coarse grid Dirac operator is defined through
 a gauge field on the block lattice as proposed in Sec.~\ref{SecUblock}.
 With the alternative $D_1$ the energy functional is not necessarily
 lowered in the coarse grid correction step.
 As a consequence we encounter the existence of problematic gauge
 field configurations where MG fails to converge.
 Similar results were also reported in
 Refs.~\cite{Benetal,PTMG_GMD,LauWit}.
 An improved gauge covariant coarse grid correction scheme is able to
 cope with the problematic gauge field configurations, but it is not
 competitive in computer time with variational MG, and therefore it is
 also not competitive with CG\@.

 In Sec.~\ref{SecLPfermi} a generalization of the ``updating on a last
 site'' as discussed for bosons in Sec.~\ref{SecLP} to the case of
 staggered fermions is proposed.
 The gauge covariance properties of the generalization are discussed in
 detail.
 However, the numerical results are disappointing.
 On lattices up to $18^4$ the method does not pay.
 The method is able to eliminate the asymptotic $1 / \Dm$ divergence
 of relaxation times in a fixed volume.
 But we feel unable to predict from numerical experiments whether
 the method will pay for staggered fermions on larger lattices of
 realizable sizes, because a volume effect which is larger than in case
 of bosons remains with respect to how long it takes until errors decay
 exponentially.
 Moreover, the asymptotic decay rate is not independent of the lattice
 size.
 Therefore it seems that not even CSD of {\em asymptotic} relaxation
 times is eliminated.
 A careful study of this question could not be done.

 In Sec.~\ref{SecMGMR} the performance of some modified MG minimal
 residual algorithms is reported.
 However, none of the tested modifications is able to improve the
 conventional minimal residual method in practice.

 Finally the use of the $\sqrt{3}$ blocking scheme of Cordery, Gupta,
 and Novotny \cite{CorGupNov} in MG computations was investigated.
 In this scheme blocks are overlapping.
 This overlap leads to a complication of variational MG, because the
 coarse grid operator is denser than the original fine grid operator.
 An approximation where the gauge field degrees of freedom are reduced
 by $1/9$ was implemented numerically.
 The results confirm the conjecture that an overlap of blocks
 accelerates the convergence speed.
 However, the costs of additional computational labor could not be
 outweighed.
 \end{quotation}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{The Competitor: Conjugate Gradient Algorithm}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}
          {{\rm\thesubsection.}\ {\sl The Competitor: Conjugate
                                      Gradient Algorithm}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 We begin also this section with looking at the competitor algorithm.
 Convergence of CG in case of staggered fermions is shown in
 Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
         {Convergence of CG for propagators of staggered fermions
          $(-\Dirac^2 + \mcr + \Dm )^{-1}$ on an $18^4$ lattice.
          Curves of open symbols are results of computations in a pure
          gauge field ($\mcr = 0$), while curves of solid symbols are
          obtained in the background of a quenched $SU(2)$ gauge field
          at $\beta = 2.7$. ($\mcr = -0.0096640$.)
          Within each of the two families the curves are parameterized
          by $\Dm = 0.1$, $0.01$, $\ldots , 10^{-6}$; $\Dm$ decreasing
          from left to right.
          The initial guess for the propagator is zero in all cases.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 Further results are in Table~$7.2$ below.
 No preconditioning of CG is employed because it turned out that
 preconditioning does not lead to an improvement in case of staggered
 fermions \cite{RosDav}.
 Hence it is the unpreconditioned CG algorithm which sets the standard.

 Qualitatively CG has the same features for propagators of
 staggered fermions than it has for bosons.
 This concerns the not necessarily monotonic decrease of $\| \rn \|$
 for small masses, and also the points how the lattice size and the
 disorder of the gauge field affect the convergence.
 Cf.\ Sec.~\ref{SecCGBosons}.
 Quantitatively it appears that CG for staggered fermions is more
 dependent on $\beta$ than it is for bosons.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{One-Grid Relaxation Algorithms
 \label{Sec1gridSF}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}
          {{\rm\thesubsection.}\ {\sl One-Grid Relaxation Algorithms}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
%..............
 \Subsubsection{Relevance of $\mcr$ in case of staggered fermions
                for a proper judging of CSD}
%..............
 In case of staggered fermions $\mcr$ is much closer to zero than
 in case of bosons.
 Actually, it is often assumed that the finite value of $\mcr$ can be
 neglected completely in \equ{scalingtau} so that $\tau \propto m^{-z}$.
 However, this neglect of $\mcr$ is not justified on lattices amenable
 in size to date.

 For bosons, scaling \equ{scalingtau} without violations
 is observed for $\Dm \lsim 0.01$ (practically independent of $|
 \Lambda |$ and $\beta$), Sec.~\ref{SecBoseVMG}.
 For staggered fermions it was verified numerically that the scaling
 relation \equ{scalingtau} also holds for traditional one-grid
 relaxation algorithms.
 The critical exponent $z$ equals 2 (fixed~$\omega$).
 It was also verified numerically that the constant of proportionality
 in \equ{scalingtau} is {\em independent of the lattice size\/}.
 Below it will be reported that this finding also holds for
 variational MG with the Laplacian choice of~$C$.

 {\em Hence, one-grid relaxation algorithms and the variational MG
      algorithm with the Laplacian choice of~$C$ will have CSD under
      conditions where the inverse mass and the linear extension of the
      lattice are changed proportionally.}

 To obtain these results requires a careful analysis of data.
 The subtle point is that for fermions \equ{scalingtau} is obeyed only
 for $\Dm \lsim 0.001$, and asymptotic decay in the sense that only the
 slowest mode governs convergence does not set in before 400 -- 500
 iterations in four-dimensional $SU(2)$ gauge fields.

 The lesson is that $\mcr$ must not be neglected, at least for lattices
 up to $18^4$.
 Otherwise one cannot study the phenomenon of CSD thoroughly.
 In practice this might mean that on such relatively small lattices
 $m^2$ must also be given small negative values.
 This is of course artificial, but it is necessary when one wants to
 obtain results which are reliable for predictions how algorithms
 perform on large lattices.
 (For larger $|\Lambda |$ the system becomes critical already for
 small and positive $m^2$; then there is no need to test algorithms
 with negative values of $m^2$.)
 We recall the discussion of Sec.~\ref{SecCautionaryRemark}.
 If one does not investigate systems close enough to criticality
 and if one does not take care that decay rates are really asymptotic,
 there is the danger of extracting wrong values for $z$, even in case
 of pure gauges.

%..............
 \Subsubsection{Analytical predictions for traditional relaxation
                methods}
%..............
 The elaborated mathematical theory which is applicable in case of
 bosonic propagators cannot be applied to fermions.
 The only thing which remains valid is the implication of Ostrowski's
 Theorem:
 SOR on one grid converges for $0 < \omega < 2$, because $(-\Dirac^2
 + m^2)$ is positive definite.
 However, $(-\Dirac^2 + m^2)$ is not a consistently ordered
 2-cyclic operator when the field strength term does not vanish,
 i.~e.\ as soon as the gauge field is not trivial.
 Therefore the conclusions, which were drawn for bosonic propagators
 in Sec.~\ref{SecCSD1grid} and checked in
 Secs.~\ref{SecFreePropagators3} and \ref{SecBose1Grid},
 do not hold for fermions.

 In particular, two points are worth mentioning.

 \begin{itemize}
 \item
 First, for given relaxation parameter $\omega$ (Jacobi or SOR) and
 given $\Dm$, convergence is the same in trivial and in any nontrivial
 gauge fields in case of bosons.
 The same is not true for fermions.
 \vspace*{-10pt}
 \item
 Second, the undamped Jacobi iteration does {\em not} converge
 for propagators of staggered fermions in nontrivial gauge fields.
 There is a threshold $< 1$ for the relaxation parameter $\omega$ below
 which damped Jacobi converges.
 The threshold coincides roughly with an optimal choice of $\omega$.
 This value of $\omega$ is picked automatically by the minimal residual
 algorithm.
 The threshold is lowered the more disordered the gauge field becomes.
 This fact suggests that {\em (undamped) Jacobi relaxation is not a
 useful smoother in MG computations with fermions.}
 \end{itemize}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Variational Multigrid
 \label{SecFermiVMG}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}
          {{\rm\thesubsection.}\ {\sl Variational MG}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The introductory remarks of Sec.~\ref{SecBoseVMG} should be
 recalled at this point.

%..............
 \Subsubsection{Numerical implementation of the Laplacian choice of $C$}
%..............
 The considerations concerning the choice of a good block spin in
 Sec.~\ref{SecBS} gave the hint that the Laplacian choice
 \equ{EVequationCSF} for $C$ is sufficient.
 The optimal interpolation kernel $\A$ associated with this $C$
 has the desired fall-off properties in nontrivial gauge fields;
 recall Sec.~\ref{SecOptA}.
 Therefore it does not seem to be necessary to implement the more
 intricate proposals discussed in Sec.~\ref{SecBSforSF}.
 Hence, only the Laplacian form of the averaging kernel has been
 implemented on a computer yet.
 But the problem of $\A$ remains -- if one puts $\A = \Cstar$ the
 problem is back.

 For the computation of $C$ we could use the same computer program as
 for bosons, except for a few marginal changes, namely replacements of
 address lists and of parallel transporters in the Laplacian.
 The efficiency of the computer program is retained for staggered
 fermions.
 [Perhaps some efficiency is lost when the algorithm will be used for
 the Diracian~$C$.
 The question is how the gap between the lowest and the second lowest
 eigenvalue, which equals~1 in pure gauges, decreases at finite values
 of~$\beta$; cf.\ the remarks in Sec.~\ref{SecAlgorithmC}.]

 The algorithm described in Sec.~\ref{SecAlgorithmC} depends essentially
 on the absence of degeneracies of the eigenvalues of $-\LAPN$ (modulo
 the intrinsic $\Nc$-fold degeneracy discussed in Sec.~\ref{SecGSP}).
 This nondegeneracy condition is preserved in our blocking procedure,
 because the averaging is chosen such that it leads to staggered
 fermions on the coarse lattice again
 (unlike \cite{HSVLAT90,HSVNP,HSVJulich,Vin,VinLAT91}).

%..............
 \Subsubsection{CSD of variational MG with the Laplacian choice of $C$}
%..............
 As mentioned in Sec.~\ref{Sec1gridSF}, the scaling relation
 \equ{scalingtau} also holds for variational MG with the Laplacian
 choice of~$C$ in case of staggered fermions, with $z=2$.
 Therefore we conclude that this algorithm will not be able to
 eliminate CSD on large lattices.

 If one is interested in the question how well algorithms perform on
 lattices of sizes that are used in present day simulations,
 the discussion in Sec.~\ref{Sec1gridSF} might appear too academic.
 It might appear more natural to ask how many iterations
 are needed to obtain a given accuracy.
 {}From this viewpoint it turned out that MG is competitive or even
 superior to conventional algorithms in two-dimensional models
 \cite{BenBraSol,HaretalLAT90,Benetal,BERV,PTMG_GMD,LauWit}.
 However, it is more difficult to reach decisive conclusions in $d=4$.
 Preliminary results on $16^4$ \cite{VinLAT91} and $18^4$
 \cite{KalLeipzig} lattices (both at $\beta = 2.7$) indicated that the
 MG methods tested so far will not be able to outperform the CG
 algorithm.

 The current status is as follows \cite{KalLAT92}.
 Despite non-elimination of CSD, MG with variational coarsening works
 better than traditional relaxation methods, but on lattices up to
 $18^4$ this MG algorithm is not competitive with CG\@.
 We expect that the situation will be different on larger lattices.
 However, we cannot predict how large the lattices have to be.

 Fig.~\NextFig\ shows convergence for propagators on $12^4$ and $18^4$
 lattices with $m^2 = 0.01$ and $m^2 = 0$.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \DoubleFigure{10.5cm}
        {Computation of propagators of staggered fermions
         $(-\Dirac^2 + m^2 )^{-1}$ for two different gauge fields
         on $12^4$ (top) and $18^4$ (bottom) lattices in quenched
         four-dimensional $SU(2)$ gauge fields at $\beta = 2.7$.
         The numbers refer to the following algorithms:
         1/2: variational MG SOR (lexicographic ordering) with $m^2 =
              0.01$/$0.0$, $\omega = 1.80$/$1.83$ (top),
              $\omega = 1.88$/$1.92$ (bottom);
         3/4: CG with $m^2 = 0.01$/$0.0$.
         The critical masses of the gauge fields are
         $\mcr = -0.0368447$ (top) and $\mcr = -0.0096640$ (bottom).}
              {10.5cm}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 Results for a propagator on an $18^4$ lattice with $m^2 =0$ using
 various algorithms
 \clearpage
 \noindent          are plotted in Fig.~\NextFig.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
        {Computation of a propagator of staggered fermions
         $(-\Dirac^2 + m^2 )^{-1}$ on an $18^4$
         lattice with $m^2 = 0$ in a quenched four-dimensional $SU(2)$
         gauge field at $\beta = 2.7$ ($\mcr = -0.0096640$).
         The numbers refer to the following algorithms:
         1/2: variational MG SOR with $\omega = 1.92$/$1.90$;
         3: MG minimal residual;
         4/5: one-grid SOR with $\omega = 1.80$/$1.91$;
         6: CG\@.
         The SOR algorithms are swept in lexicographic ordering.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 No damping parameter $\delta$ (Eq.~\equ{delta}) is used here.



==> 9212021.3 <==


 In Fig.~\PreviousFig\ results are shown for an MG minimal residual
 (MR) algorithm.
 In the MG MR algorithm, SOR on the fine lattice
 is replaced by the conventional MR algorithm.
 This algorithm works as follows.
 One replaces $\chin$ by $\chinpone = \chin + \alpha\,\rn$, where
 the number $\alpha$ is chosen such that the energy functional of
 $\chinpone$ is minimized.
 This algorithm is used by Hulsebos et al.\
 \cite{HSVLAT90,HSVNP,HSVJulich,Vin,VinLAT91}.

%..............
 \Subsubsection{Conclusions}
%..............
 The conclusions which can be drawn from Figs.~$7.2$ and $7.3$ are:
 \begin{itemize}
 \item[$(i)$] The best value for the relaxation parameter $\omega$ in
 variational MG SOR and one-grid SOR increases the more critical the
 system becomes.
 \item[$(ii)$] The (non-over-relaxed) MG minimal residual algorithm is
 clearly non-competitive with any other algorithm.
 \item[$(iii)$] When $\omega$ is not chosen close enough to its optimal
 value, it might be that even the simple one-grid SOR algorithm performs
 better than variational MG with the Laplacian choice of~$C$.
 \end{itemize}

 \clearpage
%..............
 \Subsubsection{The Laplacian choice of $C$ in variational MG might be
                inappropriate at $\beta$-values of interest}
%..............
 This last result $(iii)$ might be a warning sign that an $SU(2)$ gauge
 field at $\beta=2.7$ is still too disordered to make the Laplacian
 choice of the averaging operator~$C$ appropriate here,
 {\em i.~e.\ when one chooses $\A = \Cstar$\/}.
 Indeed, it might well be that the Laplacian choice works satisfactorily
 {\em in variational MG\/} only on extremely large lattices.
 Since the parallel transporters in the fermionic Laplacian
 \equ{SFcovLaplacian} are products of two link variables, disorder
 is in some sense enhanced compared to the bosonic case.
 This becomes obvious when we consider the lowest eigenvalues of
 $-\LAPN$ which were introduced as measures of disorder and of
 smoothness.
 Comparison is done in Table~\NextTable.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|c|c||c|c||c|c||c|c|}
 \hline
  & & \multicolumn{2}{|c||}{lower bounds for $\lambdanull$} &
  \multicolumn{2}{|c||}{average values $\langle\lambdanull\rangle$}&
  \multicolumn{2}{|c|}{upper bounds for $\lambdanull$} \\
  $\beta$ & $| \Lambda |$ & bosons & fermions & bosons & fermions &
                           bosons & fermions \\
 \hline\hline
  $\infty$ & any & 0 & 0 & 0 & 0 & 0 & 0 \\
 \hline
 $10.0$ & $18^4$ & $0.05$ & $0.14$ & $0.07$ & $0.19$ & $0.10$ & $0.24$\\
 \hline
  $5.0$ & $18^4$ & $0.12$ & $0.30$ & $0.16$ & $0.39$ & $0.21$ & $0.51$\\
 \hline
  $3.0$ & $18^4$ & $0.21$ & $0.56$ & $0.30$ & $0.70$ & $0.39$ & $0.86$\\
 \hline
  $2.7$ & $18^4$ & $0.26$ & $0.63$ & $0.35$ & $0.79$ & $0.46$ & $0.97$\\
 \hline
  $2.7$ & $12^4$ & $0.26$ & $0.66$ & $0.35$ & $0.79$ & $0.44$ & $0.96$\\
 \hline
 \end{tabular}}
       {Lowest eigenvalues $\lambdanull$ of $-\LAPN$ for bosons and
        staggered fermions in the same four-dimensional $SU(2)$ gauge
        field configurations.
        The scale factor is $L_b = 3$ in both cases.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 A similar comparison is provided by comparing Figs.~$3.2$ and $3.5$.
 These results suggest that Laplacian smoothness works equivalently
 in variational MG for bosons at $\beta = 2.7$, and for fermions at
 $\beta \sim 5$, etc.

 \smallskip
 {}From the conventional MG point of view the large value of the
 relaxation parameter $\omega$ which was found optimal in variational
 MG SOR, indicates that the Laplacian choice of $C$ is inappropriate
 here at $\beta$-values of interest.
 According to the conventional MG wisdom Gauss-Seidel relaxation
 ($\omega = 1$) should be a good smoother.
 We noted already in Sec.~\ref{SecRemarkSOR} that the picture changes
 in nontrivial gauge fields.
 In the idealized MG algorithm (Sec.~\ref{SecProof}) we found that the
 optimal value of $\omega$ increases the stronger the disorder in the
 gauge field becomes.
 In the variational MG method for bosonic propagators one needs even
 larger $\omega$'s than in the idealized algorithm in order to achieve
 peak performance.
 However, these values are by far not so large than those which were
 found optimal in case of variational MG for staggered fermions.

 \medskip
 A tentative conclusion from Fig.~$7.2$ and Table~\PreviousTable\ is
 that one nevertheless has to implement the Diracian choice of $C$ in
 order to get a competitive variational MG algorithm at $\beta$-values
 of interest.
 At least the spectrum of low-lying eigenvalues of $-\Dirac^2$ is not
 preserved by ground-state projection with $-\LAPN$,
 and this virtually contradicts our philosophy.
 However, the numerical implementation of the Diracian definition of~$C$
 has to be left for a future study.

 \clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Coarse Grid Dirac Operator via Blocked Gauge Field
 \label{SecDeffViaU}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}
          {{\rm\thesubsection.}\ {\sl Coarse Grid Dirac Operator via
                                      Blocked Gauge Field}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

%..............
 \Subsubsection{Definition of an alternative coarse grid operator}
%..............
 In Sec.~\ref{SecUblock} it was proposed to define gauge fields on
 coarser lattices by Eq.~\equ{Ublock}.
 If we set $\A = \Cstar$ we obtain coarse grid link variables which can
 be used for an alternative definition of the coarse grid operator
 $D_1$ in a modified variational MG algorithm.
 With the Laplacian choice of $C$ \equ{Ublock} gives a unique
 definition of $\U$;%
 \footnote{If $C$ were determined by Diracian ground-state projection,
           there would automatically be nonvanishing ``link'' variables
           $\U (x,y)$ with $y = x \pm \txeh L_b (\emu \pm e_{\nu})$,
           $\mu \neq \nu$.
           In case of the Galerkin operator $-C \Dirac^2 \Cstar$
           this happens already with the Laplacian choice of~$C$.}
 there are $(1/L_b^d)$-times as many link variables on $\Lone$ than on
 $\Lnull$.

 We define $D_1 = \delta^{-1} (-\Dirac_{\subs{eff}}^2 +
 m^2_{\subs{eff}})$ with $\Dirac_{\subs{eff}} = C \Dirac \Cstar$.
 The effective mass term is unchanged compared to the previous section.
 The distinction to the Galerkin operator $-C \Dirac^2 \Cstar$ is the
 product $\Cstar C$ in $\Dirac_{\subs{eff}}^2$.
 This product introduces a fluctuating length into the matrix elements
 of $D_1$.
 In the limiting case of a pure gauge this length makes essentially
 no difference because it is site-independent.
 However, in nontrivial gauge fields the fluctuating length is
 site-dependent.

%..............
 \Subsubsection{Numerical results}
%..............
 The results obtained with this modified algorithm are as follows.
 It is essential to introduce the parameter $\delta$ of
 \equ{delta} into $D_1$.
 Otherwise one cannot cope with all gauge field configurations.
 The existence of such problematic configurations where MG fails to
 converge was also reported in Refs.~\cite{Benetal,PTMG_GMD,LauWit} in
 two-dimensional $SU(2)$ and $SU(3)$ gauge fields.

 The authors of Refs.~\cite{BenBraSol,HaretalLAT90,Benetal}
 report that in case of gauge group $U(1)$ their algorithm
 performs considerably better when they re-unitarize the blocked gauge
 field (matrix elements of the effective Dirac operator) such that it
 is again an element of the gauge group.

 This point was checked in four-dimensional $SU(2)$ with our alternative
 definition of the coarse grid operator.
 We compared the case of $\Dirac_{\subs{eff}}$ as described above
 with a definition of $\Dirac_{\subs{eff}}$ where $\U (x,y)$ is
 replaced by $\U (x,y) / \| \U (x,y) \|$.
 The results are such that the difference between using a dielectric
 and a unitary gauge field on coarser layers can be compensated by
 adjusting $\delta$ in $D_1$.
 By tuning $\delta$, one can re-unitarize the blocked gauge field
 ``on the average''.

 Yet, compared with variational MG one monitors a worse convergence,
 even with optimized values of $\delta$ and $\omega$.
 We ascribe this to the fact that the MG correction step does not
 necessarily lower the energy functional when $D_1$ is not the
 Galerkin operator.

%..............
 \Subsubsection{Improved coarse grid correction scheme}
%..............
 An idea of Sec.~\ref{SecRelatedImpr} was taken up.
 An improved MG coarse grid correction step was implemented according to
 (cf.\ \equ{ImprovedCorr})
 %----------------------------------------------------------------------
  \begin{equation}
    \chi^{(n)} (z) \mapsto \chi^{\prime\,(n)} \equiv
    \chi^{(n)} (z)\ + \vpn (z)\,\Theta (H(z)) \esk
  \label{ImprovedCorrSF}
  \end{equation}
 %----------------------------------------------------------------------
 where $\vpn$ is the interpolated solution of the residual equation
 on $\Lone$.
 In \equ{ImprovedCorrSF} we introduced $2^d = 16$ $\Nc\times\Nc$
 matrices $\Theta (H(z))$.
 These matrices depend on the pseudoflavor $H$ of $z$.
 They are determined automatically by the algorithm in such a way
 that the energy functional of $\chi^{\prime\,(n)}$ is minimized.
 This eliminates the parameter $\delta$.

 The finding is that the performance of the algorithm  with
 \equ{ImprovedCorrSF} is improved and becomes equivalent in numbers
 of iterations to variational MG, except that the optimal value of
 $\omega$ is a little bit lowered.
 Variational MG is however favored, because it needs less computational
 labor.

%..............
 \Subsubsection{Remark on the pseudoflavor dependence of the matrices
                $\Theta (H)$ in \equ{ImprovedCorrSF}}
%..............
 We add a comment on the matrices $\Theta (H(z))$ in
 \equ{ImprovedCorrSF} concerning the pseudoflavor dependence.

 In the limiting case of pure gauges the fermionic problem is
 equivalent to computing $2^d$ independent (uncoupled) bosonic
 propagators, one for each pseudoflavor.
 It is obvious that one should have different matrices $\Theta$
 for the different pseudoflavors.
 Hence, we make $\Theta$ dependent on $H(z)$, and we propose to
 retain this dependence also in nontrivial gauge fields.

 Compared with \equ{ImprovedCorr}, there are no matrices
 $\Omega (H(z))$ in \equ{ImprovedCorrSF}.
 The $\Omega (H(z))$'s were left in order to avoid unnecessarily
 complex programming.
 In case of bosons it was found that the performance of
 \equ{ImprovedCorr} with fixed $\Omega = \bbbone$ plus
 \equ{rescaleBOSE} is equivalent to \equ{ImprovedCorr} with automatic
 determination of $\Omega$\@.
 It is reasonable to expect a similar result for fermions.
 Therefore the full generalization of \equ{ImprovedCorr} could be
 studied in the framework of the next section.

%..............
 \Subsubsection{Remark on the gauge covariance properties of
                \equ{ImprovedCorrSF}}
%..............
 The $2^d$ $\Nc\times\Nc$ matrices $\Theta (H)$ in \equ{ImprovedCorrSF}
 are fixed by the requirement of minimization of the energy functional
 $K$ \equ{EnergyFunctional}.
 The energy functional is gauge invariant.
 By computing the partial derivatives of $K [ \chi^{\prime\,(n)} ]$
 with respect to the variables which parameterize the matrices $\Theta
 (H)$, and equating this gradient with zero, one obtains a linear
 system of equations whose solution yields the $\Theta (H)$'s.

 Since $K$ is gauge invariant, the solution of the linear system of
 equations will exhibit gauge covariance.
 For a more comprehensive discussion we refer to the analogous
 consideration in the next subsection.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsectiontocentry{Inclusion of Updating on a Multigrid Layer
                     Consisting of a Single Site}
                    {Inclusion of Updating on a Multigrid Layer
                     \protect\\ Consisting of a Single Site
 \label{SecLPfermi}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}
          {{\rm\thesubsection.}\ {\sl Inclusion of Updating on a
                                      Single-Site MG Layer}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 As we saw in Sec.~\ref{SecLPbose}, CSD of asymptotic relaxation times
 in computations of bosonic propagators by variational MG could
 practically be eliminated, except for a reasonable volume effect, by
 including \equ{rescaleBOSE} in the algorithm.
 If a similar finding held also in case of staggered fermions,
 an efficient algorithm for propagators would have been found.

 First of all, however, \equ{rescaleBOSE} should not be used
 straightforwardly for staggered fermions.
 The ``last site'' has to be chosen as a $2^d$-point
 basis of the staggered lattice (cf.\ Sec.~\ref{SecBSforSF}
 for the $2^d$-point basis).

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 \SubSubsection{Generalization of the Proposal of
                Section \protect\ref{SecLP} for Fermions}
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 We resume the discussion from the end of the preceding section.
 In case of staggered fermions we have to take pseudoflavor into
 account.

%..............
 \Subsubsection{The case of pure gauges}
%..............
 In the limiting case of vanishing gauge coupling, Eq.~\equ{propagator}
 is an equation for $2^d$ uncoupled bosonic propagators, one for each
 pseudoflavor~$H$.
 This consideration leads us to introduce pseudoflavor dependent
 rescaling matrices $\Omega$\@.
 We generalize the global rescaling in \equ{rescaleBOSE} according to
 %----------------------------------------------------------------------
  \begin{equation}
    \chi^{(n)} (z) \mapsto \chi^{(n)} (z)\,\Omega (H(z)) \esp
  \label{rescaleFermi}
  \end{equation}
 %----------------------------------------------------------------------
 Here the $\Nc\times\Nc$ matrices $\Omega$ depend on pseudoflavor~$H$,
 and $\chi^{(n)}(z)$ is rescaled with $\Omega (H)$ when $H$ is the
 pseudoflavor $H(z)$ of~$z$.

 The $2^d$ matrices $\Omega (H)$ are determined by the requirement
 that the energy functional $K$ \equ{EnergyFunctional} of
 $[\chin\,\Omega ]$ gets minimized.
 In the case of pure gauges there is no field strength term $F_{\mu\nu}$
 in the square of the Dirac operator, and the energy functional
 decomposes into a sum of $2^d$ energy functionals.
 Each of these $2^d$ terms is an energy functional for a free bosonic
 propagator on a particular pseudoflavor sublattice.
 Hence, the $\Omega (H)$'s are given by expressions as in
 \equ{rescaleBOSE}, but $\phin$ has to be replaced by $\chin$ restricted
 to the pseudoflavor sublattices $\Lambda_a^H$.

%..............
 \Subsubsection{The case of nontrivial gauge fields}
%..............
 In case of nontrivial gauge fields we propose to retain
 \equ{rescaleFermi}, and to call it ``updating on a last site'' for
 staggered fermions.
 As remarked above the ``last site'' is a $2^d$-point basis of the
 lattice of staggered fermions.

 We shall also retain the way by which the $2^d$ $\Nc\times\Nc$
 matrices $\Omega (H)$ are determined.
 They are fixed automatically by the algorithm through the requirement
 of minimization of the energy functional $K$ of the rescaled
 propagator.

 \smallskip
 In nontrivial gauge fields the expressions for the matrices $\Omega
 (H)$ are more complicated than the expression given in
 \equ{rescaleBOSE} for $\Omega$ in case of bosons.
 By computing the partial derivatives of $K [ \chin\,\Omega ]$ with
 respect to the variables which parameterize the matrices $\Omega (H)$,
 and equating this gradient with zero, one obtains a linear system
 of equations.
 Let us call this
                 %$\Nc^2 2^d \times \Nc^2 2^d$
                                               system $\Sigma$\@.
 The solution of $\Sigma$ yields the $\Omega (H)_{i,j}$, $i,j = 1 ,
 \ldots , \Nc$, for the $2^d$ pseudoflavors~$H$.

 In practice the $\Omega (H)_{i,j}$ can be computed by solving $\Sigma$
 by means of the CG algorithm.
 One could make use of the fact that the square of the Dirac operator
 couples pseudoflavors $H$ and $K$ only when the sublattices
 $\Lambda_a^H$ and $\Lambda_a^K$ are both subsets either of the even
 or of the odd sublattice of $\Lah$.
 Therefore $\Sigma$ can be decoupled into two systems.

 With either choice, the expensive part in this calculation is not the
 solution of linear systems by CG, but the computation of the matrices
 of coefficients of these systems.

 We remark that $\Sigma$ decouples into $2^d$ systems in the limiting
 case of vanishing gauge coupling.
 Then the solution for $\Omega (H)$ is given by the expression in
 \equ{rescaleBOSE} where one has to take for $\phin$ the approximation
 $\chin$ restricted to the pseudoflavor lattice $\Lambda_a^H$, as
 discussed above.

%..............
 \Subsubsection{Gauge covariance}
%..............
 Concerning the aspect of gauge covariance of the proposal
 \equ{rescaleFermi}, one could almost repeat the discussion of
 Sec.~\ref{SecLP}.
 Basically, gauge covariance follows from the gauge invariance of
 the energy functional $K$ \equ{EnergyFunctional} which is to be
 minimized.

 When $f$ is a pseudofermion field, the coefficients in the matrix of
 the linear system $\Sigma$ and also the \rhs of $\Sigma$
 are gauge invariant.
 Therefore the solution of $\Sigma$, i.~e.\ the $2^d$ matrices
 $\Omega (H)$, are gauge invariant.
 It follows that \equ{rescaleFermi} is a gauge covariant operation.
 Analogously to the bosonic case one does not have to identify any
 reference sites $\hat{x}_N \in \Lah$ with the ``last site''.
 [Cf.\ the discussion below for a $\delta$-function~$f$.]

 We remark that gauge covariance can be exactly ensured in practice.
 It was proposed to use CG for the solution of $\Sigma$.
 When the initial guess in CG is fixed to zero, and because CG
 is a gauge covariant iteration prescription, it follows that
 all CG iterates $\Omega (H)^{(n)}$ and the iterates
 ${}^{g}\,\!\Omega (H)^{(n)}$ in a gauge transformed configuration are
 exactly connected by the $1:1$-mapping~$g$.
 If the CG iteration is stopped when the norm of the residual of
 $\Omega (H)^{(n)}$ has reached a given precision, then CG would be
 stopped at the same iteration number ${}^{(n)}$ in the gauge
 transformed configuration, because the norms of the residuals of all
 $\Omega (H)^{(n)}$ and ${}^{g}\,\!\Omega (H)^{(n)}$ are equal because
 of gauge covariance.
 Hence, the solutions $\Omega (H)$ and ${}^{g}\,\!\Omega (H)$ can
 indeed be mapped onto one another through the gauge transformation~$g$.
 Of course this whole discussion is valid up to round-off errors,
 but these are not relevant in practice.

 \smallskip
 In case that $f(z) = \delta_{z,w}$, the coefficients in the matrix of
 the linear system $\Sigma$ and also the \rhs of $\Sigma$
 transform under gauge transformations like a matter field in the
 adjoint representation sitting at site $w$.
 Therefore also the solution matrices $\Omega (H)$ will have this
 gauge covariance property, i.~e.\ if $\Omega (H)$ is the solution
 of $\Sigma$ in a particular gauge field configuration, then
 $g(w)\,\Omega (H)\,g(w)^{-1}$ is the solution in the $g$-transformed
 configuration.
 Analogously to the bosonic case it follows that \equ{rescaleFermi}
 is a gauge covariant prescription.
 [When $w$ is a site in the even sublattice of $\Lah$,
 then $\chin (z)$ will be zero for odd~$z$, and vice versa.]

 We add a comment on semantics.
 Since we defined $D = (-\Dirac^2 + m^2)$ for staggered fermions
 and $(-\Dirac^2 + m^2) = (\Dirac + m) ( -\Dirac + m)$,
 strictly speaking the propagator $(\Dirac + m)^{-1}(z,w)$ is not
 $\chi (z)$ for $f(z) = \delta_{z,w}$, but $([-\Dirac + m]\,\chi )(z)$.
 Nevertheless, gauge covariance is ensured.

 \smallskip
 We argued in the bosonic case that $w$ is a distinguished site when
 $f(z) = \delta_{z,w}$, and we identified this site $w$ with the
 reference site $\hat{x}_N$ of the ``last layer'' $\LN = \{ x_n \}$.
 The fermionic analog of this identification in case of a
 $\delta$-function~$f$ requires some discussion.

 Our interpolation kernel is the approximate propagator $\chin$, and
 $\chin$ transforms under a gauge transformation~$g$ according to
 $\chin (z) \mapsto g(z)\,\chin (z)\,g(w)^{-1}$.
 Hence, $\chin$ regarded as a kernel has the desired property
 \equ{CovKernels} with $\hat{x} = w$.
 So we have to identify the argument~$x$ which represents in the
 interpolation kernel $\A(z,x)$ ``the'' site in the last layer with~$w$.
 It is only a subtlety but not an inconsistency that the last site
 appears here as a particular site in $\Lah$ whereas it appeared before
 as a $2^d$-point basis of the staggered lattice.

%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 \SubSubsection{Numerical Results}
%:::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
 Let us now look at the numerical implementation of \equ{rescaleFermi}.

 Unfortunately, the inclusion of \equ{rescaleFermi} has not such a
 striking effect as it has in case of bosons.
 This might be (at least partially) due to the fact that we use
 lexicographic ordering in SOR instead of checkerboard updating.

 Global rescaling \equ{rescaleFermi} does not pay for positive $m^2$ on
 small lattices ($\lsim 18^4$).

 The $1 / \Dm$ divergence of {\em asymptotic} relaxation times can be
 eliminated in a fixed volume.
 As in the bosonic case one finds also in case of staggered fermions
 that $\Omega (H) = \bbbone$ (for all $H$) as soon as $|| r ||$ decays
 exponentially.
 Then the step \equ{rescaleFermi} could be switched off.
 However, this finding is of no practical importance because of two
 points.
 Firstly, there remains a volume effect with respect to how long it
 takes until errors decay exponentially, and this volume effect is
 larger than it is for bosons.
 Secondly, the asymptotic decay rate does not stay constant when the
 lattice size is increased, in contrast to the bosonic case.

 Fig.~$7.4$ displays the dependence on the relaxation parameter
 in variational MG SOR for $\Dm = 0.0001$ on a $12^4$ lattice at $\beta
 = 2.7$.
 The optimal value $\omega = 1.96$ was fixed, and the dependence on
 $\Dm$ was investigated.
 Results are in Fig.~$7.5$.
 For comparison, Fig.~$7.6$ gives results for a one-grid
 relaxation plus \equ{rescaleFermi}.
 Comparison with CG on $12^4$ and $18^4$ lattices is done in
 Fig.~$7.7$ for $\Dm = 10^{-6}$.
 Table~$7.2$ gives a survey of convergence on $12^4$ and $18^4$
 lattices.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
         {Dependence on $\omega$ in variational MG SOR (lexicographic
          ordering) plus \protect\equ{rescaleFermi}:
         Computation of a propagator of staggered fermions
         $(-\Dirac^2 + \mcr + \Dm )^{-1}$ on a $12^4$
         lattice with $\Dm = 10^{-4}$ in a quenched four-dimensional
         $SU(2)$ gauge field at $\beta = 2.7$ ($\mcr = -0.0368447$).
         The numbers 1--7 refer to the following values of $\omega$:
         $1.83$, $1.88$, $1.90$, $1.92$, $1.94$, $1.96$, and $1.98$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
         {Dependence on $\Dm$ in variational MG SOR (lexicographic
          ordering, $\omega = 1.96$) plus \protect\equ{rescaleFermi}:
         Computation of propagators of staggered fermions
         $(-\Dirac^2 + \mcr + \Dm )^{-1}$ on a $12^4$
         lattice in a quenched four-\-dimensional $SU(2)$ gauge field at
         $\beta = 2.7$ ($\mcr = -0.0368447$).
         The six curves correspond to $\Dm = 0.1, 0.01, \ldots ,
         10^{-6}$ with $\Dm$ decreasing from left to right.
         (The curves for $\Dm = 0.1$ and $\Dm = 0.01$ lie on top
          of each other.)}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
         {Dependence on $\Dm$ in one-grid SOR (lexicographic
          ordering, $\omega = 1.90$) plus \protect\equ{rescaleFermi}:
         Computation of propagators of staggered fermions
         $(-\Dirac^2 + \mcr + \Dm )^{-1}$ on a $12^4$
         lattice in a quenched four-\-dimensional $SU(2)$ gauge field at
         $\beta = 2.7$ ($\mcr = -0.0368447$).
         The six curves correspond to $\Dm = 0.1, 0.01, \ldots ,
         10^{-6}$ with $\Dm$ decreasing from left to right.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 \clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Figure{9.0cm}
        {Convergence for propagators of staggered fermions
         $(-\Dirac^2 + \mcr + \Dm )^{-1}$ with $\Dm =
         10^{-6}$ in quenched four-dimensional $SU(2)$ gauge
         fields at $\beta = 2.7$.
         The numbers refer to the following algorithms:
         1/2: variational MG SOR ($\omega = 1.96$) plus
         \protect\equ{rescaleFermi} on a $12^4$/$18^4$ lattice;
         3/4: one-grid SOR ($\omega = 1.90$) plus
         \protect\equ{rescaleFermi} on a $12^4$/$18^4$ lattice;
         5/6: CG on a $12^4$/$18^4$ lattice.
         Relaxation algorithms are swept in lexicographic ordering.
         The critical masses are $\mcr = -0.0368447$/$-0.0096640$.
         Without \protect\equ{rescaleFermi} MG SOR and one-grid SOR have
         $\tau$'s of $O(10^5)$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

\mbox{}\vfill
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsection{Modified Minimal Residual Algorithms
  \label{SecMGMR}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}
          {{\rm\thesubsection.}\ {\sl Modified Minimal Residual
                                      Algorithms}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The conventional minimal residual (MR) algorithm works as follows.
 One replaces $\chin$ by $\chinpone = \chin + \alpha\,\rn$, where
 the number $\alpha$ is chosen such that the energy functional of
 $\chinpone$ is minimized.

 In Sec.~\ref{SecFermiVMG} we have already ruled out the MG MR
 algorithm.
 But an improvement from the variational point of view was tested.

 We proposed in Sec.~\ref{SecRelatedImpr} to generalize the MR method
 analogously to \equ{ImprovedCorr} by introducing two matrices
 $\Omega$ and $\Theta$.
 In case of staggered fermions this proposal should of course be
 generalized to working with pseudoflavor dependent matrices
 $\Omega (H)$ and $\Theta (H)$\@.

 However, the numerical result is disappointing.
 Working with pseudoflavor dependent matrices leads to no practical
 improvement.
 Also the inclusion of \equ{rescaleFermi} does not make MG MR and
 the modified MG MR competitive to MG SOR.

 Over-relaxed MR versions have not been investigated yet.

 \clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{1.2}
 \Table{\begin{tabular}{|l||r|r|r|r|r|r|}
 \hline
 \multicolumn{7}{|c|}{pure gauge configurations ($\beta = \infty$)} \\
 \hline
               & \multicolumn{6}{|c|}{$m^2 =$} \\
 algorithm and lattice size
               & $10^{-1}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ &
                 $10^{-5}$ & $10^{-6}$ \\
 \hline\hline
 CG on $12^4$  & $17$  & $17$  & $17$  & $17$  & $17$  & $17$ \\
 \hline
 CG on $18^4$  & $28$  & $30$  & $33$  & $35$  & $37$  & $39$ \\
 \hline\hline
 one-grid SOR plus \equ{rescaleFermi}, $\omega = 1.90$, on $12^4$
               & $105$ & $125$ & $155$ & $195$ & $230$ & $270$\\
 \hline
 one-grid SOR plus \equ{rescaleFermi}, $\omega = 1.90$, on $18^4$
               & $110$ & $125$ & $155$ & $195$ & $230$ & $270$\\
 \hline\hline
 MG SOR without \equ{rescaleFermi}, $\omega = 1.09$, on $12^4$
               & $21$ & $23$ & $23$ & $23$ & $23$ & $23$\\
 \hline
 MG SOR without \equ{rescaleFermi}, $\omega = 1.09$, on $18^4$
               & $20$ & $23$ & $23$ & $23$ & $23$ & $23$\\
 \hline\hline
 \multicolumn{7}{|c|}{nontrivial gauge fields ($\beta = 2.7$)} \\
 \hline
               & \multicolumn{6}{|c|}{$\Dm =$} \\
 algorithm and lattice size
               & $10^{-1}$ & $10^{-2}$ & $10^{-3}$ & $10^{-4}$ &
                 $10^{-5}$ & $10^{-6}$ \\
 \hline\hline
 CG on $12^4$  & $65$  & $175$ & $265$ & $300$ & $320$ & $340$\\
 \hline
 CG on $18^4$  & $65$  & $180$ & $350$ & $415$ & $455$ & $495$\\
 \hline\hline
 one-grid SOR plus \equ{rescaleFermi}, $\omega = 1.90$, on $12^4$
               & $100$ & $130$ & $530$ & $560$ & $630$ & $710$\\
 \hline
 one-grid SOR plus \equ{rescaleFermi}, $\omega = 1.90$, on $18^4$
               &  $95$ & $125$ & $710$ & $1090$& $1320$& $1540$\\
 \hline\hline
 MG SOR plus \equ{rescaleFermi}, $\omega = 1.96$, on $12^4$
               & $180$ & $185$ & $385$ & $425$ & $475$ & $535$\\
 \hline
 MG SOR plus \equ{rescaleFermi}, $\omega = 1.96$, on $18^4$
               & $180$ & $185$ & $530$ & $775$ & $950$ & $1070$\\
 \hline\hline
 \end{tabular}}
       {Convergence in  computations of propagators
        $(-\protect\Dirac^2 + \protect\mcr + \protect\Dm )^{-1}$
        of staggered fermions in four-dimensional $SU(2)$ gauge fields.
        Given is the number of iterations necessary for reducing
        $\ln \| r^{(0)} \|$ by 10.
        One-grid SOR and MG SOR are swept in lexicographic ordering.
        The critical mass of the nontrivial gauge field configuration
        on the $\protect 12^4/18^4$ lattice is
        $\protect\mcr = -0.0368447/-0.0096640$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 \mbox{}\vfill\mbox{}

 \clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \Subsectiontocentry{Blocking and Interpolation with Overlap:
                     $\protect\sqrt{3}$ -- Scheme}
                    {Blocking and Interpolation with Overlap:
                     $\protect\sqrt{3}$ -- Scheme
 \label{SecSqrt3}}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\rm\thesection.}\ {\sc Computation of Propagators of
                                   Staggered Fermions}}
          {{\rm\thesubsection.}\ {\sl Blocking and Interpolation with
                                 Overlap: $\protect\sqrt{3}$ -- Scheme}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The contents of this section has been reported before on occasion of a
 DFG colloquium in Leipzig \cite{KalLeipzig}.

 Ben-Av et al.\
 \cite{BenBraSol,HaretalLAT90,Benetal,Benthesis,PTMG_GMD,LauWit}
 used a blocking procedure where only equal pseudoflavors are averaged,
 but where the blocks of one half of the pseudoflavors have an overlap.
 Overlap means that $\chi (z)$ at a site $z$ makes a contribution
 to more than one block spin $(C \chi )(x)$.
 It is reasonable that an overlap of blocks makes the MG approach in
 some sense ``smoother'', since the arbitrary block structure appears
 then less forced upon.

 The author tested an MG algorithm with an alternative way of
 implementing overlapping blocks where the scale factor
 $L_b$ is $\sqrt{3}$.
 This blocking was introduced by Cordery, Gupta, and Novotny
 \cite{CorGupNov} in the context of Monte Carlo renormalization group
 studies of four-dimensional gauge theories.

%..............
 \Subsubsection{Definition of the $\sqrt{3}$ blocking scheme}
%..............
 In this blocking procedure the block lattice $\Lone$ has $(1/9)$-times
 as many sites as $\Lnull$.
 Also in the $\sqrt{3}$--scheme the sites of $\Lone$ may be considered
 as a sublattice of $\Lnull$.
 Block centers $\hat{x}$ are the sites considered in
 Sec.~\ref{SecBSforSF} (encircled symbols in Fig.~$3.4$), and all
 translates $\bar{x}$ of them, $\bar{x} = \hat{x} + a\,\tilde{e}_{\mu}$,
 $\mu = \pm 1 , \ldots , \pm  d$, by one of the following vectors
%------------------- equation ------------------------------------------
 \begin{displaymath}
   \tilde{e}_1 = (0,1,1,1) \esk\quad  \tilde{e}_2 = (1,0,1,-1) \esk\quad
   \tilde{e}_3 = (1,-1,0,1) \esk\quad  \tilde{e}_4 = (1,1,-1,0)\esk
 \end{displaymath}
%------------------- equation ------------------------------------------
 and $\tilde{e}_{-\mu} = - \tilde{e}_{\mu}$.

 We retain an extension of the blocks of three lattice spacings in every
 direction along the axis of the fundamental lattice, so that every
 block spin $(C \chi )(x)$ receives contributions from $3^4$ $\chi (z)$.
 In this way every $\chi (z)$ makes a contribution to the block spin
 at nine sites~$x$.
 The reverse is true for interpolation in the variational method with
 $\A = \Cstar$.

 Note that the support property \equ{SupportC} of averaging is
 preserved for the Laplacian choice of~$C$, i.~e.\ a block spin at~$x$
 receives contributions only from sites~$z$ with the same pseudoflavor.

%..............
 \Subsubsection{Problems with variational MG in $\sqrt{3}$ -- blocking}
%..............
 Due to the overlap of blocks, there is now a severe problem with
 ``simple'' MG with $\A = \Cstar$.
 The locality properties of the (square of the) Dirac operator are not
 preserved on the block lattice.
 Every block~$x$ is coupled to a large number of other blocks~$y$.
 This leads to the situation that there are much more gauge field
 variables on the block lattice than on the original lattice.
 Also, the mass term $C m^2 \Cstar$ becomes now a non-diagonal
 mass matrix.

 \smallskip
 A crude but simple approximation to variational MG with $\L = \sqrt{3}$
 was tested numerically.
 Averaging kernels $C$ were computed according to the Laplacian
 choice \equ{EVequationCSF}.
 A coarse grid Dirac operator was defined as $C \Dirac \Cstar$,
 cf.\ Sec.~\ref{SecDeffViaU}.
 Then every block~$x$ is coupled to 216 other blocks~$y$.
 Most of the 216 matrix elements of $C \Dirac \Cstar$ were neglected.
 Only those matrix elements $(C \Dirac \Cstar )(x,y)$ were retained
 where $y = x + \frac{3}{2} \emu$.
 This means that the gauge field degrees of freedom are reduced by
 the usual factor of $1/\L^d = 1/9$.
 All but the diagonal elements of the effective mass matrix were
 neglected.

%..............
 \Subsubsection{Numerical results}
%..............
 Numerical results are as follows.
 On an $18^4$ lattice at $\beta = 2.7$ convergence for $m^2= 0$ and
 $m^2 = 0.01$ could be speeded up by a factor of about $4.5$.
 This confirms the conjecture that an overlap of blocks accelerates
 the algorithm.
 However, this is of no practical relevance because the gain in
 convergence speed could not outweigh the costs of additional
 computational labor.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \Section{Summary and Outlook
 \label{SecSummary}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \markboth{{\rm\thesection.}\ {\sc Summary and Outlook}}{}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 In the present work gauge covariant generalizations of multigrid
 methods for propagators in lattice gauge fields were investigated.
 Covariant averaging operations for bosons, for staggered fermions,
 and for gauge fields were discussed.
 These averaging operations can be used not only in deterministic and
 stochastic MG computations, but also for Monte Carlo renormalization
 group studies of gauge theories.

 \smallskip
 In case of staggered fermions the blocking procedure is not obvious.
 We required the definition of averaging maps~$C$ for fermions
 to be such that as much as possible is preserved of the residual
 internal and space-time symmetries on the lattice in the limiting
 case of vanishing gauge coupling (free fermions).
 The block spins proposed in the present thesis lead back to
 staggered fermions on coarser MG layers.

 \smallskip
 For the purpose of numerical computations we proposed to use the
 ground-state projection MG method.
 This method is applicable in arbitrary space-time dimension~$d$ and
 for arbitrary gauge group.
 We discussed why ``ground-state projection'' is not an a priori
 defined scheme because of the boundary conditions which one has to
 impose on ``block-local Hamiltonians''.
 Reasons were given for the choice of Neumann boundary conditions.
 With this choice one knows analytically that CSD is completely
 eliminated by variational MG in the limiting case of vanishing gauge
 coupling.

 \smallskip
 In ground-state projection MG the (adjoint of the) averaging
 kernel~$C$ satisfies a gauge covariant eigenvalue equation.
 We presented an efficient numerical algorithm for the solution of this
 eigenvalue equation.
 This algorithm is so efficient that we can perform exact ground-state
 projecting computations.
 This has the advantage that we do not have to fix any gauge.

 \smallskip
 In case of staggered fermions two qualitatively different proposals
 were made for the averaging kernel~$C$ -- the ``Laplacian choice'' and
 the ``Diracian choice'' -- which both reduce to ``piecewise-constant''
 kernels in the absence of gauge fields.
 Only the Laplacian choice of~$C$ has been implemented on a computer
 yet.

 \smallskip
 Actual numerical computations were performed in four-dimensional
 $SU(2)$ gauge fields.
 It was proved that ground-state projection defines a good block spin,
 both for bosons and for the Laplacian choice of $C$ in case of
 staggered fermions.
 The proof uses arguments from the renormalization group which involve
 an optimal interpolation kernel $\A$ which is associated with~$C$.
 This $\A$ is a gauge covariant generalization of a kernel which was
 used successfully in rigorous works on constructive quantum field
 theory.

 \smallskip
 The same optimal interpolation kernel $\A$ was used in an idealized
 MG algorithm for bosonic propagators.
 By means of this idealized MG algorithm it was proved that
 {\em the MG method can cope in principle with systems with disorder\/}.
 MG computations of propagators without CSD in nontrivial gauge
 fields are possible, in principle.
 This statement is true for {\em any} value of the gauge coupling,
 including the case of completely random gauge fields.
 The success of these computations gives ample evidence from the
 deterministic side that Mack's contention concerning the need for
 smooth and overlapping interpolation kernels is correct.

 \smallskip
 Unfortunately, the idealized MG algorithm is not practical because
 of computational complexity and storage space requirements.
 But it was important to answer questions of principle.

 \smallskip
 The ultimate goal of the present thesis is the development of an
 efficient MG method for the computation of gauge covariant propagators
 of staggered fermions.
 The MG method has to be so efficient that it outperforms the best
 algorithm known, which is CG\@.

 \smallskip
 A practical MG method is variational coarsening.
 In the toy model of bosonic propagators the results of this method
 are as follows.
 Variational MG is able to outperform CG, also with respect to
 computer time.
 A practical modification which can be thought of as ``updating on an
 MG layer consisting of a single site'' succeeds in eliminating CSD
 of {\em asymptotic} relaxation times.
 A remaining volume effect with respect to many iterations it takes
 until the asymptotic regime is reached is reasonably mild.
 The method costs some additional computational labor, but as soon as
 errors decay exponentially, updating at the last site can be
 switched off.
 Therefore additional work must only be invested in the initial and
 in an intermediate stage of computations.

 \smallskip
 We have not succeeded yet in implementing a method which is
 competitive with the CG algorithm in case of staggered fermions,
 at least for lattice sizes up to $18^4$.

 \smallskip
 Numerical results for staggered fermions can be summarized as follows.
 The scaling relation $\tau = \mbox{const} / \Dm$ holds for one-grid
 relaxations and for variational MG with the Laplacian choice of~$C$.
 $\mbox{const}$ is independent of the lattice size.
 (For bosonic one-grid relaxations this result is known analytically.)
 Therefore we conclude that those variational MG algorithm will not be
 able to eliminate CSD on large lattices.

 \smallskip
 The fermionic generalization of the ``updating at a last site''
 is successful only in so far that it also eliminates CSD of {\em
 asymptotic} relaxation times in a fixed volume.
 However, this is of no practical relevance because there remains not
 only a relatively large volume effect with respect to how long it
 takes until errors decay exponentially, but also the asymptotic decay
 rate is not independent of the lattice size
 (in contrast to the situation for bosons).

 \smallskip
 The implementation of the $\sqrt{3}$ blocking scheme showed that
 a nontrivial overlap of blocks can lead to an acceleration of
 convergence.
 Unfortunately, the acceleration in number of iterations could not
 outweigh the extra costs of more computational labor.

 \smallskip
 But other overlapping blocking procedures might be more successful.
 We recall that the Diracian choice of~$C$ has not been
 implemented and investigated yet.
 {}From the physical point of view this proposal, although
 computationally quite demanding, is preferable.
 It is also closer to the philosophy of ground-state projection MG\@.
 In the Diracian choice the averaging kernel $C(x,z)$ can be
 nonvanishing in nontrivial gauge fields when $z$ and $x$ carry
 different pseudoflavors.
 This might be a crucial point, because it is a qualitatively new
 kind of overlap of blocks compared with the $\sqrt{3}$ -- scheme.
 It is planned to test the Diracian proposal.
 However, this has to be deferred to a future publication.
 One may also think of a further refinement where larger blocks
 (e.\ g.\ $5^4$ blocks) overlap already in the limiting case of pure
 gauges and where $C(x,z)$ may be nonvanishing in nontrivial gauge
 fields when $z$ and $x$ carry different pseudoflavors.

 \smallskip
 Finally we note that fruitful results are expected when MG methods
 are combined with ideas from neural net computations
 \cite{MacKalPalSpe,BaeKalMacSpe,MacSpe,Bae}.

%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 \markboth{{\sc Acknowledgments}}{}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 \clearpage

 \addcontentsline{toc}{section}{\protect\numberline{}
                 {\hspace*{-5pt} Acknowledgments}}

 {\noindent\mbox{}\hfill{\sc Acknowledgments}\hfill\mbox{}}

 {\small
         \noindent
 I would like to thank Professor Gerhard Mack for many stimulating
 discussions, and for constant support and encouragement.
 I appreciate being involved in the frontier of the exciting
 adventure of making MG methods usable for gauge theories.
 \newline\noindent
 I am also indebted to many others who contributed with helpful
 discussions and conversations, in particular the members of the
 ``Hamburg Multigrid Group'', and R.C.\,Brower, R.G.\,Edwards,
 H.G.\,Evertz, S.\,Meyer, K.\,Pinn, C.\,Rebbi, A.D.\,Sokal,
 and H.-J.\,Timme.
 \newline\noindent
 I wish to thank J.\,Smit and S.\,Solomon for encouraging me to
 continue the study of MG methods for fermionic propagators.
 \newline\noindent
 Financial support by Deutsche Forschungsgemeinschaft
 is gratefully acknowledged.
 \newline\noindent
 The computations reported in this article were performed on the
 Siemens 7882 of the University of Hamburg, on the IBM 3090 of
 DESY, and on the CRAY Y--MP of HLRZ J\"ulich.
 The staff of these three Computing Centers provided useful advices.
 }
 \renewcommand{\thesection}{\Alph{section}}
 \renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection}.}
 \setcounter{section}{0}
 \renewcommand{\thefootnote}{\protect\alph{footnote})}
 \setcounter{footnote}{0}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \Appendix{Appendix \thesection: Staggered Fermions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \markboth{{\sc Appendix \thesection: Staggered Fermions}}{}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl This appendix comprises a summary of Euclidean staggered fermions.
      It consists of two parts.
      In the first one the better-known spin-diagonalization technique
      is summarized, while the second part shows the connection to the
      Dirac-K\"ahler formalism.}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \SubAppendix{Staggered Fermions from Spin-Diagonalization}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\sc Appendix \thesection: Staggered Fermions}}
    {\thesubsection\ {\sl Staggered Fermions from Spin-Diagonalization}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 We will mainly follow the position space treatment of Kluberg-Stern et
 al.~\cite{KluMorNapPet}, see also the review given in Ref.~\cite{Rot}.
 A momentum space treatment can be found in  Ref.~\cite{ShaThuWei}.
 The notations and conventions used in this thesis are also
 summarized here.

 In order to be concrete, let the dimension $d$ of space-time be 4.
 The Euclidean time $z_4$ and the Minkowski time $t$ are connected
 through $z_4 = i t$.
 Euclidean $\gamma$-matrices are defined by $\gamma_4 = \gamma_0^M$,
 $\gamma_k = i \gamma_k^M$, $k=1,2,3$, where the superscript $^M$
 refers to Minkowski space.
 The Euclidean $\gamma$-matrices are Hermitean, $\gamma_{\mu}^{\dagger}
 = \gamma_{\mu}$, and fulfill the Clifford algebra $\{ \gamma_{\mu} ,
 \gamma_{\nu} \} = 2\,\delta_{\mu\nu} \bbbone$, $\mu , \nu = 1,2,3,4$\@.
 We also define $\gamma_5 = \gamma_1 \gamma_2 \gamma_3 \gamma_4$,
 and $\gamma_{-\mu} = -\gamma_{\mu}$.

 The naive action for free Dirac fermions $\Psi$ on a
 lattice $\Lambda$ of lattice spacing $a$ is
%------------------- equation ------------------------------------------
  \begin{equation}
   \H ( \bar{\Psi} , \Psi ) = \int_z \frac{1}{2a} \bar{\Psi} (z)
      \sum_{\mu} \gamma_{\mu}\,\left[ \Psi ( z + \emu ) - \Psi
      ( z - \emu ) \right]\ +\ m \int_z \bar{\Psi} (z)\,\Psi (z) \esp
  \label{NaiveAction}
  \end{equation}
%------------------- equation ------------------------------------------
 The continuum derivative has to be approximated by the central
 difference quotient in order that the (anti-)Hermiticity properties
 of the action are preserved on the lattice.

 The lattice integration $\int_z$ means $a^d \sum_{z\in\Lambda}$, and
 $\emu$ denotes a lattice vector of length $a$ in $\mu$-direction.
 It is convenient to define also lattice vectors for negative
 directions, $e_{-\mu} = - e_{\mu}$, and $e_0 = 0$.

 The key step for the staggered formulation is a
 ``spin-diagonalization'' of the naive action
 \cite{ShaThuWei,KluMorNapPet}:
 One performs a unitary transformation of the Dirac field,
%------------------- equation ------------------------------------------
  \begin{equation}
    \Psi (z) = T(z)\,\Xi (z)\esk\quad
     \bar{\Psi} (z) = \bar{\Xi} (z)\,T(z)^{-1} \esk
  \label{UnitaryTransformation}
  \end{equation}
%------------------- equation ------------------------------------------
 where the $T(z)$ are unitary $2^{d/2} \times 2^{d/2}$ matrices,
 chosen such that
%------------------- equation ------------------------------------------
  \begin{equation}
   T(z)^{-1}\,\gamma_{\mu}\,T(z+\emu ) = \etamu (z) \bbbone \esp
  \label{Tmatrices}
  \end{equation}
%------------------- equation ------------------------------------------
 $\etamu (z)$ are complex numbers of modulus 1.
 These are not completely arbitrary.
 For instance the product of $\etamu$'s around a plaquette must always
 equal $-1$, but the various possible choices are all equivalent
 \cite{KluMorNapPet}.
 Since we defined $\gamma_{-\mu} = -\gamma_{\mu}$, it follows that
 $\eta_{-\mu} (z) = -\eta_{\mu} (z - \emu)$.
 One realization of \equ{Tmatrices} is ($z = a (n_1 , n_2 , n_3 , n_4
 )$)
%------------------- equation ------------------------------------------
  \begin{equation}
    T (z) =
    \gamma_1^{n_1}\,\gamma_2^{n_2}\,\gamma_3^{n_3}\,\gamma_4^{n_4} \esk
  \label{realizationT}
  \end{equation}
%------------------- equation ------------------------------------------
 yielding for the phase factors
%------------------- equation ------------------------------------------
  \begin{equation}
   \eta_1 (z) = 1, \quad \eta_2 (z) = (-1)^{n_1}, \quad
                         \eta_3 (z) = (-1)^{n_1+n_2}, \quad
                         \eta_4 (z) = (-1)^{n_1+n_2+n_3} \esp
  \label{etamus}
  \end{equation}
%------------------- equation ------------------------------------------
 In this representation $\etamu (z)$ is independent of the
 $\mu$-component of $z$, and hence $\eta_{-\mu} (z) = - \etamu (z)$.

 Through the transformation \equ{UnitaryTransformation} the action
 \equ{NaiveAction} has become diagonal in the Dirac indices $\alpha$.
 Originally, $\alpha = 1 , \ldots , 2^{d/2}$\@.
 Staggered fermions are defined by retaining only the
 action for one of the $\Xi^{\alpha}$ components.
 An important point is that the decoupling of the $\Xi^{\alpha}$
 components also holds when gauge fields are introduced.
 The arbitrarily chosen retained component $\Xi^{\alpha}$ will be called
 $\chi$\@.
 Hence, the staggered fermion action is
%------------------- equation ------------------------------------------
  \begin{equation}
   \H ( \bar{\chi} , \chi ) = \int_z \frac{1}{a}\sum_{\mu} \etamu (z)\,%
      \bar{\chi} (z)\,\left[ \chi ( z + \txeh\emu ) - \chi ( z -
      \txeh\emu ) \right]\ +\ m \int_z \bar{\chi} (z)\,\chi (z) \esp
  \label{StaggeredAction}
  \end{equation}
%------------------- equation ------------------------------------------

 In the staggered fermion formulation $\chi$ is not a field with a
 physical continuum limit.
 A (naive) continuum limit which yields Dirac fermions can only be
 taken for a field $\psi$ which is a superposition of $\chi(z)$ and
 which is defined on a lattice that has twice the lattice spacing of
 $\Lambda$.
 We have already considered this fact in Eq.~\equ{StaggeredAction},
 were we redefined $a$ to half its value.
 ($\emu$ remains to be a vector of length $a$.)

 The lattice on which $\chi$ is defined will be called $\Lah$.
 $\int_z$ in \equ{StaggeredAction} means $(a/2)^d \sum_{\in\Lah}$.
 For a construction of the $\psi$ field, divide $\Lah$ into hypercubes
 $\tilde{y}$ consisting of $2^d$ sites $z$.
 Sites within one hypercube are distinguished by their ``pseudoflavor''
 $H$, cf.\ Eqs.~\equ{PF}, \equ{zPF}, and
 Fig.~\theSecPFlattice.\theFigPFlattice.
 Hence, $\Lah$ is made up of $2^d$ pseudoflavor lattices $\Lambda_a^H$
 whose sites have all the same pseudoflavor $H$ and whose lattice
 spacing is $a$.
 We write $z\in\ty$ if $z$ is a site in hypercube $\ty$.
 The lattice $\{ \ty \}$ will be denoted by $\Lambda_a$\@.

 In terms of crystallography as used in solid state physics
 \cite{AshMer}, the lattice of staggered fermions is a hypercubic
 lattice $\Lambda_a$ of unit cells of lattice spacing~$a$ with a
 $2^d$-point basis.
 The basis is given by the sites of a hypercube of volume $(a/2)^d$.
 Sites within the basis are distinguished by their ``pseudoflavor''~$H$.
 Different pseudoflavors would correspond to different species of
 atoms or ions in the solid state analog.

 $\psi ( \ty )$ will be a linear combination of $\chi (z)$ with
 $z\in\ty$.
 It is defined by
%------------------- equation ------------------------------------------
  \begin{equation}
   \psi_{\alpha}^f ( \ty ) = 2^{-3d/2}
      \sum_{z\,\in\,\ty} \Gamma_{\alpha f} (z)\,\chi (z)\esk\quad
   \bar{\psi}_{\alpha}^f ( \ty ) = 2^{-3d/2}
      \sum_{z\,\in\,\ty}
                     \bar{\chi} (z)\,\Gamma_{\alpha f}^{\dagger} (z)\esp
  \label{QuarkField}
  \end{equation}
%------------------- equation ------------------------------------------
 The indices $\alpha$ and $f$ take values $1 , \ldots , 2^{d/2}$.
 $\Gamma_{\alpha f}$ are unitary $\zhdh\times\zhdh$ matrices which
 shall fulfill
%------------------- equation ------------------------------------------
  \begin{equation}
    \Gamma ( z + \emu ) = \Gamma (z) \esk\quad\mbox{and}\quad
    \Tr\left[ \Gamma (z_1)^{\dagger} \Gamma (z_2) \right] = \left\{
     \begin{array}{cl} \zhdh & \mbox{if $H(z_1) = H(z_2)$,} \\
           0 & \mbox{otherwise.} \end{array} \right.
  \label{OrthogonalityGamma}
  \end{equation}
%------------------- equation ------------------------------------------
 $H(z)$ denotes the pseudoflavor of $z$.
 Because of \equ{OrthogonalityGamma} the transformation
 \equ{QuarkField} becomes invertable:
%------------------- equation ------------------------------------------
  \begin{equation}
   \chi (z) = 2^{d/4} \sum_{\alpha , f}
         \Gamma_{f\alpha}^{\dagger}(z)\,\psi_{\alpha}^f ( \ty )\esk\quad
   \bar{\chi} (z) = 2^{d/4} \sum_{\alpha , f}
         \bar{\psi}_{\alpha}^f ( \ty )\,\Gamma_{\alpha f} (z)\esk
  \label{StaggeredField}
  \end{equation}
%------------------- equation ------------------------------------------
 for $z\in\ty$.
 A possible representation for $\Gamma (z)$ is the same as for $T(z)$,
 Eq.~\equ{realizationT}.
 Inserting Eq.~\equ{StaggeredField} into the
 action~\equ{StaggeredAction} yields
%------------------- equation ------------------------------------------
  \begin{eqnarray}
   \H ( \bar{\psi} , \psi ) & = & \int_{\ty} \bar{\psi} ( \ty )
       \sum_{\mu} \left[ ( \gamma_{\mu}\otimes\bbbone ) \partial_{\mu}
          \psi ( \ty )
   +\frac{a}{2} ( \gamma_5\otimes\gamma_{\mu}\gamma_5 )
       ( \partial\partial )_{\mu}  \psi ( \ty ) \right]  \nonumber\\
   & & + m  \int_{\ty}
     \bar{\psi} ( \ty ) ( \bbbone\otimes\bbbone ) \psi ( \ty ) \esp
  \label{QuarkAction}
  \end{eqnarray}
%------------------- equation ------------------------------------------
 Here $\int_{\ty} = a^d \sum_{\ty}$\,,
 $\partial_{\mu}$ and $( \partial\partial )_{\mu}$ are first and second
 central derivatives on $\Lambda_a$:\
 $\partial_{\mu} \psi ( \ty ) = a^{-1} [ \psi ( \ty + \emu ) - \psi
 ( \ty - \emu ) ]$, and $( \partial\partial )_{\mu} \psi ( \ty ) =
 a^{-2} [ \psi ( \ty + \emu ) - 2 \psi ( \ty ) + \psi ( \ty - \emu )]$.

 Formula \equ{QuarkAction} is the basis for the interpretation of
 staggered fermions \cite{KluMorNapPet}.
 The direct products of matrices are understood such that the first
 matrix acts on Greek indices and the second one on Latin indices.
 Greek indices are interpreted as spinorial indices, while Latin
 indices are regarded as labeling flavor degrees of freedom.
 In the naive continuum limit the action \equ{QuarkAction} describes
 $\zhdh$ degenerate flavors of Dirac fermions.
 The flavors are coupled by the second term in \equ{QuarkAction},
 even if this term vanishes for $a \rightarrow 0$.

 The free propagator of $\psi$ reads in momentum space:
%------------------- equation ------------------------------------------
  \begin{equation}
   S (p) = \frac{\d{\frac{i}{a} \sum_{\mu} \left[ ( \gamma_{\mu}\otimes
                 \bbbone ) \sin (p_{\mu} a) + \frac{2}{a}
                 \sin^2 \left(\frac{p_{\mu} a}{2}\right) ( \gamma_5
                 \otimes \gamma_{\mu} \gamma_5 ) \right] \
                 +\ m ( \bbbone\otimes\bbbone )}}%
                {\d{\frac{4}{a^2} \sum_{\mu} \sin^2
                 \left(\frac{p_{\mu}a}{2}\right) + m^2}} \esp
  \label{QuarkPropagator}
  \end{equation}
%------------------- equation ------------------------------------------
 The denominator in \equ{QuarkPropagator} has only one pole in the
 first Brillouin zone.
 In the naive continuum limit $a\rightarrow 0$ one has
%------------------- equation ------------------------------------------
  \begin{equation}
   S (p)\ {\raisebox{-4pt}{$\stackrel{\longrightarrow}
           {\scriptscriptstyle a \rightarrow 0}$}}\
         = \frac{\d{i \sum_{\mu} ( \gamma_{\mu}\otimes \bbbone )p_{\mu}
                 +\ m ( \bbbone\otimes\bbbone )}}
                {\d{p^2 + m^2}} \esk
  \end{equation}
%------------------- equation ------------------------------------------
 which is the correct propagator describing $\zhdh$ degenerate
 Dirac fermions.

 It is instructive to compare with Wilson's formulation of lattice
 fermions \cite{WilsonFermions}.
 The action for $\zhdh$ degenerate flavors of Wilson fermions reads
 as Eq.~\equ{QuarkAction}, except that the matrix $(\gamma_5\otimes
 \gamma_{\mu}\gamma_5 )$ in the second term in the sum over $\mu$ is
 replaced by $(\bbbone\otimes\bbbone )$.
 Both terms vanish for $a \rightarrow 0$.
 But whereas for Wilson fermions axial symmetry is completely lost
 for finite $a$, staggered fermions preserve at least a nontrivial
 piece of the full chiral symmetry for $m=0$.
 The action \equ{QuarkAction} with $m=0$ is invariant under
%------------------- equation ------------------------------------------
  \begin{displaymath}
   \psi (\ty ) \rightarrow e^{i \theta (\gamma_5\otimes\gamma_5 )}
   \psi (\ty ) \esk\quad
   \bar{\psi} (\ty ) \rightarrow \bar{\psi} (\ty )
              e^{i \theta (\gamma_5\otimes\gamma_5 )} \esk
  \end{displaymath}
%------------------- equation ------------------------------------------
 where $\theta$ is an arbitrary real parameter.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \SubAppendix{Staggered Fermions and the Dirac-K\"ahler Equation}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\sc Appendix \thesection: Staggered Fermions}}
    {\thesubsection\ {\sl Staggered Fermions and the
                          Dirac-K\"ahler Equation}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 The outline in this section follows Refs.~\cite{BecJoo,JooSch}.
 In the Dirac-K\"ahler formalism the Dirac field (in the continuum)
 is described by a differential form~$\Phi$,
%------------------- equation ------------------------------------------
 \begin{equation}
  \Phi = \sum_H \varphi (y,H)\,dy^H \quad\mbox{with}\quad
   dy^H = dy^{\mu_1} \wedge \cdots \wedge dy^{\mu_h}
                                 \esk
 \label{DiffForm}
 \end{equation}
%------------------- equation ------------------------------------------
 where $H$ is the ordered set of indices which specifies
 pseudoflavor, cf.\ Eq.~\equ{PF}.
 There are $2^d$ such sets $H$\@.
 It is understood that $dy^{\emptyset} = 1$.
 $\Phi$ may be decomposed into $\zhdh$ independent Dirac fields
 $\psi^f$, in such a way that iff $\Phi$ satisfies the Dirac-K\"ahler
 equation
%------------------- equation ------------------------------------------
 \begin{equation}
   ( d - \delta + m) \Phi = 0 \esk
 \label{DKE}
 \end{equation}
%------------------- equation ------------------------------------------
 then the $\psi^f$ are solutions of the Dirac equations
%------------------- equation ------------------------------------------
 \begin{equation}
   ( \mbox{$\not\!\partial$} + m) \psi^f = 0 \esk\quad f = 1 , \ldots ,
                  \zhdh \esp
 \label{DiracEq}
 \end{equation}
%------------------- equation ------------------------------------------
 The symbols $d$ and $\delta$ in Eq.~\equ{DKE} denote exterior
 differentiation and the codifferential operator, respectively.

 In the multi-index notation one defines the matrices
%------------------- equation ------------------------------------------
 \begin{equation}
   \gamma^H \equiv \gamma^{\mu_1} \cdots \gamma^{\mu_h} \esk\quad
   \gamma^{\emptyset} = \bbbone\esp
 \label{gammaH}
 \end{equation}
%------------------- equation ------------------------------------------
 Note that these matrices are the same which were used in
 Appendix~\theappSF.1\ for a representation of the $\Gamma$
 matrices in \equ{QuarkField}--\equ{StaggeredField}.
 We have the equality $\Gamma (z) = \gamma^H$ when $H$ is the
 pseudoflavor of $z$.
 One defines a matrix $Z = (Z_{f \alpha})$ of forms,
%------------------- equation ------------------------------------------
 \begin{equation}
   Z = 2^{d/4} \sum_H \left( \gamma^H \right)^{\dagger} dy^H \esp
 \label{Zmatrix}
 \end{equation}
%------------------- equation ------------------------------------------
 The Dirac fields $\psi^f$ are then defined by
%------------------- equation ------------------------------------------
 \begin{equation}
  \Phi = \sum_H \varphi (y,H)\,dy^H
       = \sum_{f , \alpha} \psi^f_{\alpha} (y) Z_{f \alpha} \esp
 \label{DKfields}
 \end{equation}
%------------------- equation ------------------------------------------
 With the help of the definition of the Clifford product $\vee$ of
 forms, $dy^{\mu} \vee dy^{\nu} = dy^{\mu} \wedge dy^{\nu} +
 \delta^{\mu\nu}$, the Dirac-K\"ahler operator $(d - \delta )$ can be
 brought into the form $(d - \delta ) \Phi = dy^{\mu} \vee
 \partial_{\mu} \Phi$.
 By explicit calculation one verifies that $\psi^f$, $f=1,\ldots,\zhdh$,
 satisfy the Dirac equation iff $\Phi$ solves the Dirac-K\"ahler
 equation.

 Since the Dirac-K\"ahler equation is a differential geometric
 equation, its lattice transcription is straightforward
 \cite{BecJoo,JooSch}.
 The lattice Dirac-K\"ahler field becomes a staggered fermion field
 $\chi$ if one identifies $\chi (z) = \varphi (\ty,H)$, for
 $z = \ty + \txeh e_H$, with $e_H$ as in \equ{zPF}.
 (Compare Eq.~\equ{DKfields} with \equ{StaggeredField}.)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \Appendix{Appendix \thesection: Kernels in ``Optimal'' Multigrid}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \markboth{{\sc Appendix \thesection: Kernels in ``Optimal'' Multigrid}}
          {}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 {\sl This Appendix deals with kernels in MG algorithms.
      There are three parts: $(i)$ a review of the kernels in the
      optimal MG algorithm, $(ii)$ their Fourier representations (in
      the absence of gauge fields), and $(iii)$ some tables giving
      numerical values.}

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \SubAppendix{Review of the Gaw\c{e}dzki-Kupiainen Kernels}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\sc Appendix \thesection: Kernels in ``Optimal'' Multigrid}}
    {\thesubsection\ {\sl Review of the Gaw\c{e}dzki-Kupiainen Kernels}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 In this appendix the choice of kernels in the ``optimal'' MG algorithm
 is reviewed.
 Equations for the ideal interpolation kernel $\A$, given an averaging
 kernel $C$, are derived.
 This $\A$ appeared for the first time in the works \cite{GawKup}
 of \Gaw and Kupiainen.
 They gave rigorous proofs of the existence of the continuum limit of
 some lattice field theories without gauge fields, using block spin
 renormalization group methods.
 Mack \cite{MacCargese} pointed out that the use of smooth interpolation
 kernels in numerical MG work will be essential for fighting CSD.
 He proposed the Gaw\c{e}dzki-Kupiainen kernels as a starting point.
 We will follow in our exposition mainly the script \cite{Tim} of Timme.

 Consider a bosonic matter field $\phi$ which is defined on a
 $d$-dimensional Euclidean lattice $\Lambda = \Lnull$ of lattice
 spacing $a$.
 Gauge fields are not yet included, although their inclusion is
 straightforward; cf.\ the remarks at the end of this section.
 Let $\H ( \phi) = \txeh < \phi , v^{-1} \phi > +\ \V ( \phi )$ be
 the action.
 $v$ is the free propagator.
 (In connection with the notations of Sec.~\ref{SecMGmethods}, $v^{-1}
 = D$.)
 The partition function is
%------------------- equation ------------------------------------------
  \begin{equation}
   Z = \int \dmuv\ e^{-\V (\phi )} \esk
  \label{Z}
  \end{equation}
%------------------- equation ------------------------------------------
 where $\dmuv$ denotes the normalized Gaussian measure \cite{GliJaf}
 with covariance $v$,
%------------------- equation ------------------------------------------
  \begin{equation}
   \dmuv  =  \det (2 \pi v )^{-1/2} \prod_{z\,\in\,\Lnull} [d\phi (z)]\
             e^{-\txeh < \phi , v^{-1} \phi >} \esp
  \label{dmuv}
  \end{equation}
%------------------- equation ------------------------------------------
 A Gaussian block spin transformation is attained by inserting
%------------------- equation ------------------------------------------
  \begin{equation}
   1 = \int \prod_{x\,\in\,\Lone} [d\Phi (x)\ {\textstyle \left(
        \frac{\kappa (L_b a)^d}{2\pi} \right)^{1/2} } ]\
        \exp \left( - \frac{\kappa}{2} \| \Phi - C \phi \|^2 \right)
  \label{GaussianBS}
  \end{equation}
%------------------- equation ------------------------------------------
 into the partition function .
 Here $\Lone$ is a block lattice of lattice spacing $L_b a$,
 $\Phi$ is called the block spin which is defined on $\Lone$, and
 $\| \Phi - C \phi \|^2 = < \Phi - C \phi , \Phi - C \phi >$\@.
 $C$ is a linear averaging operator, with kernel \equ{CwithoutGF},
 for instance.
 $C$ associates a block spin $C\phi$ with every field $\phi$.
 In the limit that the real parameter $\kappa$ tends to infinity,
 \equ{GaussianBS} reduces to a $\delta$ block spin transformation,
%------------------- equation ------------------------------------------
  \begin{equation}
   1 = \int \prod_{x\,\in\,\Lone} \left[d\Phi (x)\
        \delta \left( \Phi (x) - ( C \phi ) (x) \right) \right] \esp
  \label{deltaBS}
  \end{equation}
%------------------- equation ------------------------------------------

 The idea of the real space renormalization group approach to quantum
 field theory is to split the field $\phi$ on the original lattice into
 a low frequency part $\psi$ and a high frequency part $\zeta$ and to
 integrate out the high frequency field $\zeta$ in order to obtain an
 effective action.
 $\psi$ and $\zeta$ are called ``background field'' and ``fluctuation
 field'', respectively.
 $\psi$ should be smooth and it is determined by the block spin $\Phi$.
 The split of the field becomes
%------------------- equation ------------------------------------------
  \begin{equation}
    \phi = \A \Phi + \zeta \esp
  \label{split}
  \end{equation}
%------------------- equation ------------------------------------------
 $\A$ is an interpolation kernel which maps fields on $\Lone$
 into fields on $\Lnull$.
 By means of the split \equ{split} the kinetic term of the action
 $\H$ becomes
%------------------- equation ------------------------------------------
  \begin{equation}
   \txeh < \phi , v^{-1} \phi >\ =\ \txeh < \A \Phi , v^{-1} \A \Phi >\
   +\ \txeh < \zeta , v^{-1} \zeta >\ +\ < v^{-1} \A \Phi , \zeta > \esp
  \label{Hsplit}
  \end{equation}
%------------------- equation ------------------------------------------

 It is an easy exercise to show that
%------------------- equation ------------------------------------------
  \begin{equation}
   \Q [ \phi ]\ =\ \txeh < \phi , v^{-1} \phi >\ +\ \frac{\kappa}{2}\,%
                 \| \Phi - C \phi \|^2
  \label{q}
  \end{equation}
%------------------- equation ------------------------------------------
 can be rewritten as
%------------------- equation ------------------------------------------
  \begin{equation}
   \Q [ \phi ]\ =\ \txeh \| \Gamma^{-1/2} \phi - \kappa \Gamma^{1/2}
                          \Cstar \Phi \|^2
               + \txeh < \Phi , u^{-1} \Phi >  \esp
  \label{qrewritten}
  \end{equation}
%------------------- equation ------------------------------------------
 In Eq.~\equ{qrewritten} we defined the free propagator $u$ of the block
 spin field $\Phi$,
%------------------- equation ------------------------------------------
  \begin{equation}
    u = \left( \kappa \bbbone - \kappa^2\,C\,\Gamma\,\Cstar \right)^{-1}
    \esk
  \label{u}
  \end{equation}
%------------------- equation ------------------------------------------
 and the free propagator $\Gamma$ of the fluctuation field $\zeta$,
%------------------- equation ------------------------------------------
  \begin{equation}
    \Gamma = \left( v^{-1} + \kappa\,\Cstar C \right)^{-1} \esp
  \label{Gamma}
  \end{equation}
%------------------- equation ------------------------------------------
 $\Cstar$ denotes the adjoint of $C$.

 Let us now require that $\A$ is determined such that $\A \Phi$
 is the classical field configuration for the Hamiltonian $\Q$, i.\ e.\
 $\phi = \A \Phi$ minimizes $\Q$.
 This immediately yields
%------------------- equation ------------------------------------------
  \begin{equation}
    \A = \kappa\,\Gamma\,\Cstar \esp
  \label{A}
  \end{equation}
%------------------- equation ------------------------------------------
 As a consequence
%------------------- equation ------------------------------------------
  \begin{equation}
   \Q [\phi = \A \Phi + \zeta ]\ =\ \txeh < \zeta , \Gamma^{-1} \zeta >
                               \ +\ \txeh < \Phi , u^{-1} \Phi > \esp
  \label{qseparated}
  \end{equation}
%------------------- equation ------------------------------------------
 One also readily verifies,
%------------------- equation ------------------------------------------
  \begin{eqnarray}
         \A & = & v\,\Cstar\,u^{-1}\esk \label{Arew} \\
          u & = & C\,v\,\Cstar + \kappa^{-1}\label{urew} \esk \\
          v & = & \Gamma + \A\,u\,\A^{\ast}\esp \label{flucprop}
  \end{eqnarray}
%------------------- equation ------------------------------------------

 It follows that $C \A = \bbbone$ and $u^{-1} = (C\Cstar )^{-1} C v^{-1}
 \A = \A^{\ast} v^{-1} \A$ for $\kappa \rightarrow \infty$.
 In this limit the fluctuation field $\zeta$ has vanishing block
 averages, $C\zeta = 0$.
 Then, as a consequence of Eq.~\equ{Arew}, the mixed term $< v^{-1} \A
 \Phi , \zeta >$ in \equ{Hsplit} vanishes.
 Thus, there is no coupling between high and low frequencies in the
 free Hamiltonian.

 Another property of the $\A$-kernel is
%------------------- equation ------------------------------------------
 \begin{equation}
   \int_x \A (z,x) = 1 \quad\mbox{for all $z \in \Lnull$}\esk
 \label{CorrectConstant}
 \end{equation}
%------------------- equation ------------------------------------------
 where $\int_x = (\L a)^d \sum_{x \in \Lone}$.
 This equation can be proved by using the Fourier representation of
 $\A$, cf.\ Eq.~\equ{FourierA}.

 Eq.~\equ{flucprop} means that the split \equ{split} of the field $\phi$
 implies a split of the propagator $v$ into a propagator $\Gamma$ for
 the high frequency field $\zeta$ and a propagator $\A u \Astar$
 for the low frequency field $\psi$.
 This is valid for any value of $\kappa$ and it allows the application
 of the convolution formula for Gaussian measures,
%------------------- equation ------------------------------------------
  \begin{equation}
   \dmuv = \dmuu\,\dmuG \esp
  \label{convolution}
  \end{equation}
%------------------- equation ------------------------------------------
 This factorization may be checked with the help of the formula
 for the characteristic functional of a Gaussian measure \cite{GliJaf},
 $\int \dmuv\ e^{i < J,\phi >} = e^{-\txeh < J , v J >}$.

 In summary we have shown that the partition function \equ{Z}
 can be rewritten as
%------------------- equation ------------------------------------------
  \begin{equation}
   Z = \int \dmuu  \int \dmuG\ e^{-\V ( \A \Phi + \zeta )} \esp
  \label{Zrewritten}
  \end{equation}
%------------------- equation ------------------------------------------
 This rewriting may be iterated \cite{MacCargese}.
 It leads to a mapping of a (nearly) critical system on $\Lnull$
 onto a noncritical system on the MG\@.
 Eq.~\equ{Zrewritten} serves as a staring point for nonperturbative
 calculations in constructive quantum field theory
 \cite{GawKup,GawKupLH,BalProp,BalLGT}.
 For the success of these analytical works it is essential that
 effective Hamiltonians have good locality properties, to all orders
 in perturbation theory.
 Good locality properties follow from the decay properties of kernels.
 When $C$ is the ``piecewise-constant'' kernel of Eq.~\equ{CwithoutGF},
 $\Gamma (z,w)$ decays exponentially with distance $|z-w|$, with
 decay length of order one block lattice spacing $L_b a$.
 This means that $\zeta$ is a field with an infrared cutoff (i.\ e.\
 with a ``mass'').
 The fall-off properties of $\Gamma$ are shared by $\A (z,x)$ and by
 the effective Laplacian (plus mass term) $u^{-1}$.
 This can be proved by using their Fourier representations, and
 shifting the path of the momentum integration into the complex plane
 \cite{GawKup}.
 If the kernels decay exponentially, it will be said that $C$ defines a
 good block spin.
 It is plausible that a good block spin in this sense is also essential
 in MG computations of gauge covariant propagators.
 In an interacting theory exponential decay of $\Gamma$ and $\A$ is
 preserved to all orders of perturbation theory.
 In special cases, this has also been shown nonperturbatively
 \cite{GawKup,BalProp}.

 We conclude with remarks on the consequences of introducing gauge
 fields.
 In $v^{-1} = (-\Delta + m^2)$ the Laplacian will become the gauge
 covariant Laplacian \equ{LaplaceKernel}.
 The averaging kernel $C$ may be given by the ground-state projection
 definition \equ{EVequationC}.
 It enjoys gauge covariance \equ{CovKernels}.
 This alone implies gauge covariance of $\Gamma$, $u$, and $\A$.
 All of the above equations remain valid and are gauge covariant.
 Translational invariance of the kernels is of course lost in the
 presence of gauge fields, but the fall-off properties
 are retained, see Sec.~\ref{SecOptA} and the tables in
 Appendix~\theappKernels.3.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \SubAppendix{Fourier Representations of Kernels}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\sc Appendix B: Kernels in ``Optimal'' Multigrid}}
          {\thesubsection\ {\sl Fourier Representations of Kernels}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 We will now quote the Fourier representations of integral kernels
 in the absence of gauge fields, for the $\delta$ block spin
 transformation ($\kappa = \infty$).
 In arbitrary pure gauges the kernels are given by the same formulas,
 multiplied with (arbitrary) parallel transporters from $w_2$ to
 $w_1$ for a kernel with arguments $(w_1,w_2)$.

%..............
 \Subsubsection{Notations}
%..............
 We consider a $d$-dimensional hypercubic lattice $\Lambda = \Lnull$ of
 lattice spacing $a$ and with sites $z$, with an extension of $N$ sites
 in each direction.
 For functions on this $N^d$ lattice we impose periodic boundary
 conditions.
 The momenta of the reciprocal lattice will be denoted by $p$.
 We superimpose a block lattice $\Lone$ by blocking $\Lnull$ with an
 integer scale fac\-tor $\L$.
 The momenta of the reciprocal block lattice are denoted by $q$.

 We define lattice integrations
%------------------- equation ------------------------------------------
 \begin{equation}
  \int_z\ =\ a^d \sum_{z\in\Lnull}\quad\quad\mbox{and}\quad\quad
  \intp\ =\ \frac{a^{-d}}{| \Lnull |} \sum_{p\,\in\,BZ} \esk
 \label{LatticeIntegrations}
 \end{equation}
%------------------- equation ------------------------------------------
 and analogously for the block lattice.
 The expressions in \equ{LatticeIntegrations} reduce in the limit $a
 \rightarrow 0$ to the usual continuum integrals.
 Summation in the momentum integral is over all momenta in the first
 Brillouin zone ($BZ$)\@.

 The $\delta$ distributions are on the lattice
%------------------- equation ------------------------------------------
 \begin{equation}
  \delta (z_1 - z_2 ) = a^{-d}\,\delta_{z_1\,,\,z_2}
   \quad\quad\mbox{and}\quad\quad
  \delta (p_1 - p_2 ) = \frac{| \Lnull |}{( 2\pi )^d}\,%
                        a^d\,\delta_{p_1\,,\,p_2} \esp
 \label{deltadistr}
 \end{equation}
%------------------- equation ------------------------------------------
 We will need the formulas
%------------------- equation ------------------------------------------
 \begin{equation}
   \intz e^{ipz} = \delta (p)
   \quad\quad\mbox{and}\quad\quad
   \intp e^{-ipz} = \delta (z) \esk
 \label{deltas}
 \end{equation}
%------------------- equation ------------------------------------------
 and Poisson's resummation formula \cite{GelSch} whose lattice
 version reads
%------------------- equation ------------------------------------------
 \begin{equation}
  \int_{x \in \Lone}  e^{iqx}\ =\ ( 2\pi )^d \sumn \delta ( q +
   \frac{2\pi}{\L a} n ) \esk
 \label{PRF}
 \end{equation}
%------------------- equation ------------------------------------------
 where $\delta ( q + \frac{2\pi}{\L a} n ) = \prod_{\mu = 1}^d
 \delta ( q_{\mu} + \frac{2\pi}{\L a} n_{\mu} )$.

%..............
 \Subsubsection{Integral Kernels}
%..............
 With these preparations one finds the Fourier transformation
 of the kernel $C$ of Eq.~\equ{CwithoutGF},
%------------------- equation ------------------------------------------
 \begin{equation}
   C(x,z) = \intp \tC (p)\,e^{-i p (x-z)}
                          \quad\quad\mbox{with}\quad\quad
   \tC (p) = \alpha (p) \prod_{\mu} \frac{\sin\left(\frac{p_{\mu}\L a}%
   {2}\right)}{\L \sin\left(\frac{p_{\mu} a}{2}\right)} \esk
 \label{FourierC}
 \end{equation}
%------------------- equation ------------------------------------------
 where $\alpha (p) = 1$ for odd $\L$, and $\alpha (p) = \exp ( -i
 \sum_{\mu} p_{\mu} a / 2 )$ otherwise.

 The Klein-Gordan operator $a^{-2} D = -\Delta + m^2$ has the Fourier
 representation
%------------------- equation ------------------------------------------
 \begin{equation}
   D(z_1 , z_2 ) = \intp \tD (p)\,e^{-i p (z_1 - z_2)}
     \quad\quad\mbox{with}\quad\quad
   \tD (p) = \frac{4}{a^2} \sum_{\mu}\sin^2\left(\frac{p_{\mu} a}{2}
             \right) + m^2 \esp
 \label{FourierD}
 \end{equation}
%------------------- equation ------------------------------------------

 The inverse of the optimal effective Klein-Gordan operator $\Deff$
 is given by (cf.\ \equ{urew}, $u \equiv \Deff^{-1}$)
%------------------- equation ------------------------------------------
 \begin{equation}
   \Deff^{-1} ( x , y ) = \intq \tu (q)\,e^{-i q (x - y)}
     \quad\quad\mbox{with}\quad\quad
   \tu (q) = \sumn\ \frac{| \tC ( q + \frac{2\pi}{\L a} n ) |^2}%
                        {\tD ( q + \frac{2\pi}{\L a} n )} \esp
 \label{FourierDeff}
 \end{equation}
%------------------- equation ------------------------------------------

 For the optimal interpolation kernel $\A$ one finds
%------------------- equation ------------------------------------------
 \begin{eqnarray}
   \A ( z , x ) & = & \intq \tA (z,q)\,e^{-i q (z - x)}\nonumber\\
     \mbox{with} & & \label{FourierA} \\
   \tA (z,q) & =&  \frac{1}{\tu (q)} \sumn\
          \frac{\tC ( q + \frac{2\pi}{\L a} n )}%
               {\tD ( q + \frac{2\pi}{\L a} n )}\,%
   e^{-i 2\pi n z / (\L a)} \esp  \nonumber
 \end{eqnarray}
%------------------- equation ------------------------------------------
 With the help of Eqs.~\equ{FourierC} and \equ{FourierA} one can
 explicitly verify that $(C\A )(x,y) = \delta (x-y)$.
 One also readily verifies Eq.~\equ{CorrectConstant}.

 Finally we quote the kernel of the Galerkin operator $C D \Cstar$:
%------------------- equation ------------------------------------------
 \begin{eqnarray}
   (C D \Cstar )( x , y ) & = & \intq \tGal (q)\,e^{-i q (x - y)}
     \nonumber\\ \mbox{with} & & \label{FourierDGal}\\
   \tGal (q) & = & \sumn\ {\tD ( q + \frac{2\pi}{\L a} n )}
              {| \tC ( q + \frac{2\pi}{\L a} n ) |^2} \esp \nonumber
 \end{eqnarray}
%------------------- equation ------------------------------------------
 Note the distinction between the Fourier transforms $\tu^{-1}$
 and $\tGal$ of the optimal coarse grid operator and of the Galerkin
 operator.

 By using the Fourier representations given here one can easily
 compute the two-grid iteration matrix $\M$.
 It is easy to check that that $\M$ annihilates the slowest mode
 of the one-grid iteration matrix $M$, both in the optimal MG scheme
 and in case of variational MG\@.

 \vfill
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \SubAppendix{Numerical Values of Integral Kernels}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \markboth{{\sc Appendix B: Kernels in ``Optimal'' Multigrid}}
          {\thesubsection\ {\sl Numerical Values of Integral Kernels}}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 This section comprises a summary in tabular form of numerical values
 for integral kernels.
 Given are the optimal $\A$-kernel and the optimal effective Laplacian
 $C \Delta \A = \Astar\Delta\A$
 on $9^4$, $12^4$, and $18^4$ lattices in the absence of gauge fields.
 We also give the values for the ``Ohrenkern'' (which has
 support on one block and its eight nearest neighbors;
 cf.\ Sec.~\ref{SecApproxA}), and for the
 resulting effective Laplacian on a $12^4$ lattice.
 The last two tables contain examples of an optimal effective gauge
 covariant Laplacian and a square of the Dirac operator in nontrivial
 gauge fields.
 The corresponding $\A$-kernels are shown in
 Fig.~\theSecAkernel.\theFigAbose.
%and~\theSecAkernel.\theFigAfermi.
 All $\A$-kernels are ``critical'' kernels.
 They were computed as solution of Eq.~\equ{optimalA} with
 $m^2 = \mcr$, $\kappa = 100\,000$.

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc Optimal interpolation kernel $\A$ in the absence of
             gauge fields,

                           $9^4$ lattice.}
 \vspace{2mm}

 \begin{tabular}{|rrr|rrr|}
 \hline
 $-0.1638$&$-0.1910$&$-0.1638$ & $-0.0441$&$-0.0103$&$-0.0038$ \\
 $-0.0625$&$-0.0688$&$-0.0625$ &  $0.0020$&$-0.0010$&$-0.0103$ \\
  $0.2432$& $0.3014$& $0.2432$ &  $0.1063$& $0.0020$&$-0.0441$ \\
 \hline
  $1.1018$& $1.3063$& $1.1018$ &  $0.2432$&$-0.0625$&$-0.1638$ \\
  $1.3063$& \fbox{$1.5543$}& $1.3063$ &  $0.3014$&$-0.0688$&$-0.1910$ \\
  $1.1018$& $1.3063$& $1.1018$ &  $0.2432$&$-0.0625$&$-0.1638$ \\
 \hline
 \end{tabular}}
 {Optimal interpolation kernel $(L_b a)^4 \A (z,0)$ in the absence
  of gauge fields on a $9^4$ lattice for block size $L_b=3$, at
  $z=(z_1,z_2,1,1)$ for $z_1,z_2 = 0 , \ldots , 5$.
  The largest value is the framed one at $z=(1,1,1,1)$.
  The non-given values of $\A (z,x)$ follow from translational
  invariance and periodicity.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc Optimal interpolation kernel $\A$ in the absence of
             gauge fields,

                           $12^4$ lattice.}

 \vspace{2mm}
 \begin{tabular}{|rrr|rrr|rrr|}
 \hline
 $-0.0113$&$-0.0152$&$-0.0113$ & $-0.0069$&$-0.0006$& $0.0017$ &
  $0.0002$& $0.0000$& $0.0002$ \\
  $0.0179$& $0.0192$& $0.0179$ &  $0.0032$& $0.0026$& $0.0029$ &
  $0.0000$&$-0.0005$& $0.0000$ \\
 $-0.0113$&$-0.0152$&$-0.0113$ & $-0.0069$&$-0.0006$& $0.0017$ &
  $0.0002$& $0.0000$& $0.0002$ \\
 \hline
 $-0.1303$&$-0.1498$&$-0.1303$ & $-0.0313$&$-0.0076$&$-0.0020$ &
  $0.0017$& $0.0029$& $0.0017$ \\
 $-0.0718$&$-0.0777$&$-0.0718$ & $-0.0028$&$-0.0038$&$-0.0076$ &
 $-0.0006$& $0.0026$&$-0.0006$ \\
  $0.2246$& $0.2824$& $0.2246$ &  $0.0937$&$-0.0028$&$-0.0313$ &
 $-0.0069$& $0.0032$&$-0.0069$ \\
 \hline
  $1.1036$& $1.3124$& $1.1036$ &  $0.2246$&$-0.0718$&$-0.1303$ &
 $-0.0113$& $0.0179$&$-0.0113$ \\
  $1.3124$& \fbox{$1.5660$}& $1.3124$ &  $0.2824$&$-0.0777$&$-0.1498$ &
 $-0.0152$& $0.0192$&$-0.0152$ \\
  $1.1036$& $1.3124$& $1.1036$ &  $0.2246$&$-0.0718$&$-0.1303$ &
 $-0.0113$& $0.0179$&$-0.0113$ \\
 \hline
 \end{tabular}}
 {Optimal interpolation kernel $(L_b a)^4 \A (z,0)$ in the absence
  of gauge fields on a $12^4$ lattice for block size $L_b=3$, at
  $z=(z_1,z_2,1,1)$ for $z_1,z_2 = 0 , \ldots , 8$.
  The largest value is the framed one at $z=(1,1,1,1)$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 \clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc Optimal interpolation kernel $\A$ in the absence of
             gauge fields,

                           $18^4$ lattice.}

 \vspace{2mm}
 \begin{tabular}{|rrr|rrr|rrr|}
 \hline
  $0.2267$& $0.2845$& $0.2267$ &  $0.0955$&$-0.0019$&$-0.0330$ &
 $-0.0127$& $0.0016$& $0.0057$ \\
 $-0.0708$&$-0.0768$&$-0.0708$ & $-0.0019$&$-0.0033$&$-0.0082$ &
 $-0.0034$& $0.0014$& $0.0028$ \\
 $-0.1342$&$-0.1545$&$-0.1342$ & $-0.0330$&$-0.0082$&$-0.0027$ &
 $-0.0002$& $0.0015$& $0.0018$ \\
 \hline
 $-0.0281$&$-0.0343$&$-0.0281$ & $-0.0127$&$-0.0034$&$-0.0002$ &
 $-0.0002$& $0.0002$& $0.0003$ \\
  $0.0091$& $0.0098$& $0.0091$ &  $0.0016$& $0.0014$& $0.0015$ &
  $0.0002$&$-0.0001$&$-0.0002$ \\
  $0.0166$& $0.0188$& $0.0166$ &  $0.0057$& $0.0028$& $0.0018$ &
  $0.0003$&$-0.0002$&$-0.0002$ \\
 \hline
  $0.0015$& $0.0019$& $0.0015$ &  $0.0010$& $0.0003$&$-0.0001$ &
  $0.0000$& $0.0000$& $0.0000$ \\
 $-0.0024$&$-0.0026$&$-0.0024$ & $-0.0006$&$-0.0006$&$-0.0006$ &
 $-0.0001$& $0.0000$& $0.0000$ \\
  $0.0015$& $0.0019$& $0.0015$ &  $0.0010$& $0.0003$&$-0.0001$ &
  $0.0000$& $0.0000$& $0.0000$ \\
 \hline
  $0.0166$& $0.0188$& $0.0166$ &  $0.0057$& $0.0028$& $0.0018$ &
  $0.0003$&$-0.0002$&$-0.0002$ \\
  $0.0091$& $0.0098$& $0.0091$ &  $0.0016$& $0.0014$& $0.0015$ &
  $0.0002$&$-0.0001$&$-0.0002$ \\
 $-0.0281$&$-0.0343$&$-0.0281$ & $-0.0127$&$-0.0034$&$-0.0002$ &
 $-0.0002$& $0.0002$& $0.0003$ \\
 \hline
 $-0.1342$&$-0.1545$&$-0.1342$ & $-0.0330$&$-0.0082$&$-0.0027$ &
 $-0.0002$& $0.0015$& $0.0018$ \\
 $-0.0708$&$-0.0768$&$-0.0708$ & $-0.0019$&$-0.0033$&$-0.0082$ &
 $-0.0034$& $0.0014$& $0.0028$ \\
  $0.2267$& $0.2845$& $0.2267$ &  $0.0955$&$-0.0019$&$-0.0330$ &
 $-0.0127$& $0.0016$& $0.0057$ \\
 \hline
  $1.1034$& $1.3116$& $1.1034$ &  $0.2267$&$-0.0708$&$-0.1342$ &
 $-0.0281$& $0.0091$& $0.0166$ \\
  $1.3116$& \fbox{$1.5645$}& $1.3116$ &  $0.2845$&$-0.0768$&$-0.1545$ &
 $-0.0343$& $0.0098$& $0.0188$ \\
  $1.1034$& $1.3116$& $1.1034$ &  $0.2267$&$-0.0708$&$-0.1342$ &
 $-0.0281$& $0.0091$& $0.0166$ \\
 \hline
 \end{tabular}}
 {Optimal interpolation kernel $(L_b a)^4 \A (z,0)$ in the absence
  of gauge fields on an $18^4$ lattice for block size $L_b=3$, at
  $z=(z_1,z_2,1,1)$ for $z_1 = 0 , \ldots , 8$, and
  $z_2 = 0 , \ldots , 17$.
  The largest value is the framed one at $z=(1,1,1,1)$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

 \clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc Optimal effective Laplacian $\Delta_{\subs{eff}}$ in the
             absence of gauge fields,

                                      $3^4$ block lattice.}

 \vspace{2mm}
 \begin{tabular}{|r|r|r|}
 \hline
 $-2.5691$& $0.0841$& $0.0841$ \\
 \hline
 $-2.5691$& $0.0841$& $0.0841$ \\
 \hline
 \fbox{$17.8535$}&$-2.5691$&$-2.5691$ \\
 \hline
 \end{tabular}}
 {Kernel $(L_b a)^6 (-\Delta_{\subs{eff}}) (0,y)$, $y=(y_1,y_2,0,0)$
  of the optimal effective Laplacian $\Astar\Delta\A = C\Delta\A$ in the
  absence of gauge fields on a $3^4$ block lattice, obtained from
  blocking a $9^4$ lattice with $L_b=3$.
  $y_1,y_2=0,1,2$.
  The value of $(L_b a)^6 (-\Delta_{\subs{eff}}) (0,0)$ is framed.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc Optimal effective Laplacian $\Delta_{\subs{eff}}$ in the
             absence of gauge fields,

                                      $4^4$ block lattice.}

 \vspace{2mm}
 \begin{tabular}{|r|r|r|r|}
 \hline
 $-2.9089$& $0.0192$& $0.0601$& $0.0192$ \\
 \hline
  $0.6911$& $0.0601$&$-0.0214$& $0.0601$ \\
 \hline
 $-2.9089$& $0.0192$& $0.0601$& $0.0192$ \\
 \hline
 \fbox{$18.2590$}&$-2.9089$& $0.6911$&$-2.9089$ \\
 \hline
 \end{tabular}}
 {Kernel $(L_b a)^6 (-\Delta_{\subs{eff}}) (0,y)$, $y=(y_1,y_2,0,0)$
  of the optimal effective Laplacian $\Astar\Delta\A = C\Delta\A$ in the
  absence of gauge fields on a $4^4$ block lattice, obtained from
  blocking a $12^4$ lattice with $L_b=3$.
  $y_1,y_2=0,1,2,3$.
  The value of $(L_b a)^6 (-\Delta_{\subs{eff}}) (0,0)$ is framed.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc Optimal effective Laplacian $\Delta_{\subs{eff}}$ in the
             absence of gauge fields,

                                      $6^4$ block lattice.}

 \vspace{2mm}
 \begin{tabular}{|r|r|r|r|r|r|}
 \hline
 $-2.8742$& $0.0336$& $0.0312$&$-0.0165$& $0.0312$& $0.0336$ \\
 \hline
  $0.3515$& $0.0312$&$-0.0053$& $0.0010$&$-0.0053$& $0.0312$ \\
 \hline
 $-0.0893$&$-0.0165$& $0.0010$& $0.0000$& $0.0010$&$-0.0165$ \\
 \hline
  $0.3515$& $0.0312$&$-0.0053$& $0.0010$&$-0.0053$& $0.0312$ \\
 \hline
 $-2.8742$& $0.0336$& $0.0312$&$-0.0165$& $0.0312$& $0.0336$ \\
 \hline
 \fbox{$18.2109$}&$-2.8742$& $0.3515$&$-0.0893$& $0.3515$&$-2.8742$ \\
 \hline
 \end{tabular}}
 {Kernel $(L_b a)^6 (-\Delta_{\subs{eff}}) (0,y)$, $y=(y_1,y_2,0,0)$
  of the optimal effective Laplacian $\Astar\Delta\A = C\Delta\A$ in the
  absence of gauge fields on a $6^4$ block lattice, obtained from
  blocking an $18^4$ lattice with $L_b=3$.
  $y_1,y_2=0,1,2,3,4,5$.
  The value of $(L_b a)^6 (-\Delta_{\protect\subs{eff}}) (0,0)$ is
  framed.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

\clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc ``Ohrenkern'' in the absence of gauge fields.}

 \vspace{2mm}
 \begin{tabular}{|rrr|rrr|}
 \hline
 $-0.1070$&$-0.1262$&$-0.1070$ &  $0.0000$& $0.0000$& $0.0000$ \\
 $-0.0644$&$-0.0678$&$-0.0644$ &  $0.0000$& $0.0000$& $0.0000$ \\
  $0.2011$& $0.2706$& $0.2011$ &  $0.0000$& $0.0000$& $0.0000$ \\
 \hline
  $1.1081$& $1.3256$& $1.1081$ &  $0.2011$&$-0.0644$&$-0.1070$ \\
  $1.3256$& \fbox{$1.5877$}& $1.3256$ &  $0.2706$&$-0.0678$&$-0.1262$ \\
  $1.1081$& $1.3256$& $1.1081$ &  $0.2011$&$-0.0644$&$-0.1070$ \\
 \hline
 \end{tabular}}
 { ``Ohrenkern'' $(L_b a)^4 \A (z,0)$ in the absence of gauge fields
  for block size $L_b=3$, at $z=(z_1,z_2,1,1)$ for $z_1,z_2 = 0 ,
  \ldots , 5$.
  This interpolation kernel has support only on block $x=0$ and its
  eight nearest neighbors.
  It is the solution of Eq.~\protect\equ{BoseA} with $\Delta$ replaced
  by the Laplacian with Dirichlet boundary conditions on the boundary of
  the desired support of $\A$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc Effective Laplacian associated with the ``Ohrenkern''

             in the absence of gauge
             fields on a $4^4$ block lattice.}

 \vspace{2mm}
 \begin{tabular}{|r|r|r|r|}
 \hline
 $-2.8416$& $0.0342$& $0.0356$& $0.0342$ \\
 \hline
  $0.5313$& $0.0356$& $0.0000$& $0.0356$ \\
 \hline
 $-2.8416$& $0.0342$& $0.0356$& $0.0342$ \\
 \hline
 \fbox{$18.8755$}&$-2.8416$& $0.5313$&$-2.8416$ \\
 \hline
 \end{tabular}}
 {Kernel $(L_b a)^6 (-\Delta_{\subs{eff}}) (0,y)$, $y=(y_1,y_2,0,0)$
  of the effective Laplacian $\Astar\Delta\A$ in the absence of gauge
  fields on a $4^4$ block lattice, obtained from blocking a $12^4$
  lattice with $L_b = 3$.
  Here $\A$ is the kernel of Table~\PreviousPreviousTable.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++


\clearpage
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc An optimal effective Laplacian $\Delta_{\subs{eff}}$ in
             a four-dimensional $SU(2)$ gauge field,

             $\beta=2.7$, $6^4$ block lattice.}

 \vspace{2mm}
 \begin{tabular}{|r|r|r|r|r|r|}
 \hline
  $2.2616$& $0.3173$& $0.0304$& $0.0171$& $0.0536$& $0.2360$ \\
 \hline
  $0.2722$& $0.0495$& $0.0069$& $0.0017$& $0.0050$& $0.0288$ \\
 \hline
  $0.0501$& $0.0187$& $0.0013$& $0.0004$& $0.0014$& $0.0116$ \\
 \hline
  $0.3084$& $0.0272$& $0.0045$& $0.0014$& $0.0040$& $0.0353$ \\
 \hline
  $2.4617$& $0.2733$& $0.0509$& $0.0105$& $0.0410$& $0.1610$ \\
 \hline
 \fbox{$14.2018$}& $2.1237$& $0.2655$& $0.0387$& $0.2726$& $2.3101$ \\
 \hline
 \end{tabular}}
 {Kernel $(L_b a)^6 \protect\| (-\Delta_{\subs{eff}}) (0,y)\protect\|$,
  $y=(y_1,y_2,0,0)$
  of an optimal effective Laplacian $\Astar\Delta\A = C\Delta\A$ in
  a four-dimensional $SU(2)$ gauge field at $\beta=2.7$ on a $6^4$ block
  lattice, obtained from blocking an $18^4$ lattice with $L_b=3$.
  $y_1,y_2 = 0,1,2,3,4,5$.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \renewcommand{\arraystretch}{2.0}
 \Table{{\sc An optimal effective Diracian $\Dirac_{\subs{eff}}^2$ in
             a four-dimensional $SU(2)$ gauge field,

             $\beta=2.7$, $6^4$ block lattice.}

 \vspace{2mm}
 \begin{tabular}{|r|r|r|r|r|r|}
 \hline
  $0.0000$& $0.6121$& $0.0000$& $0.1195$& $0.0000$& $0.4612$ \\
 \hline
  $1.1497$& $0.0000$& $0.1096$& $0.0000$& $0.1348$& $0.0000$ \\
 \hline
  $0.0000$& $0.1565$& $0.0000$& $0.0425$& $0.0000$& $0.1134$ \\
 \hline
  $1.4623$& $0.0000$& $0.1722$& $0.0000$& $0.0711$& $0.0000$ \\
 \hline
  $0.0000$& $0.2583$& $0.0000$& $0.1256$& $0.0000$& $0.2931$\\
 \hline
  \fbox{$9.7798$}& $0.0000$& $2.1071$& $0.0000$& $1.0994$& $0.0000$ \\
 \hline
 \end{tabular}}
 {Kernel $(L_b a)^6\| (-\Dirac^2_{\subs{eff}}) (0,y)\|$,
  $y=(y_1,y_2,0,0)$ of an optimal effective squared Dirac operator
  $\Astar\Dirac^2\A = C\Dirac^2\A$ in
  a four-dimensional $SU(2)$ gauge field at $\beta=2.7$ on a $6^4$ block
  lattice, obtained from blocking an $18^4$ lattice with $L_b=3$.
  $y_1,y_2=0,1,2,3,4,5$.
  Note the support property: the kernel is only nonvanishing on even
  lattice sites.}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
 \begin{singlespace}
 \addcontentsline{toc}{section}{\protect\numberline{}
                 {\hspace*{-5pt} References}}
 \begin{thebibliography}{150}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 \markboth{{\sc References}}{}
%xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
 \small{
 \bibitem{Wil}
              K.G.\,Wilson,
              {\em Confinement of quarks\/},
              Phys. Rev. D10 (1974) 2445

 \bibitem{ItzZub}
              C.\,Itzykson and J.-B.\,Zuber,
              {\em Quantum field theory\/}, second printing
              (McGraw-Hill, Singapore, 1986)

 \bibitem{Ryd}
              L.H.\,Ryder,
              {\em Quantum field theory\/}
              (Cambridge University Press, Cambridge, 1985)

 \bibitem{Sym}
              K.\,Symanzik,
              {\em Euclidean quantum field theory\/},
              Varenna 1968,
              in: Local quantum theory,
              ed.\ R.\,Jost
              (Academic Press, New York, 1969)


 \bibitem{OstSch}
              K.\,Osterwalder and R.\,Schrader,
              {\em Euclidean Fermi fields and a Feynman-Kac formula
                   for boson-fermion models\/},
              Helv. Phys. Acta 46 (1973) 277

 \bibitem{OstSei}
              K.\,Osterwalder and E.\,Seiler,
              {\em Gauge field theories on a lattice\/},
              Ann. Phys. 110 (1978) 440

 \bibitem{Sei}
              E.\,Seiler,
              {\em Gauge theories as a problem of constructive
                   quantum field theory and statistical mechanics\/},
              Lecture Notes in Physics 159
              (Springer-Verlag, Berlin, 1982)

 \bibitem{GliJaf}
              J.\,Glimm and A.\,Jaffe,
              {\em Quantum physics\/}, second edition
              (Springer-Verlag, New York, 1987)

 \bibitem{Hua}
              K.\,Huang,
              {\em Statistical mechanics\/}, second edition
              (John Wiley \& Sons, New York, 1987)

 \bibitem{Jer}
              J.\,Jers\'ak,
              {\em Path integral method in quantum theory\/},
              in: Path integral method, lattice gauge theory and
              critical phenomena,
              Proceedings of the Autumn College on Techniques in Many
              Body Problems, Lahore, Pakistan, 1987
              (World Scientific, Singapore, 1989)

 \bibitem{Roe}
              G.\,Roepstorff,
              {\em Pfadintegrale in der Quantenphysik\/},
              (F.\,Vieweg \& Sohn, Braunschweig, 1991)

 \bibitem{LueWei}
              M.\,L\"uscher and P.\,Weisz,
              {\em Scaling laws and triviality bounds in the lattice
                   $\phi^4$ theory.
                   I.\,One-component model in the symmetric phase\/},
              Nucl. Phys. B290 [FS20] (1987) 25;

              M.\,L\"uscher and P.\,Weisz,
              {\em Scaling laws and triviality bounds in the lattice
                   $\phi^4$ theory.
                  II.\,One-component model in the phase with
                       spontaneous symmetry breaking\/},
              Nucl. Phys. B295 [FS21] (1988) 65;

              M.\,L\"uscher and P.\,Weisz,
              {\em Scaling laws and triviality bounds in the lattice
                   $\phi^4$ theory.
                 III.\,$n$-component model\/},
              Nucl. Phys. B318 (1989) 705

 \bibitem{HamHan}
              J.M.\,Hammersley and D.C.\,Handscomb,
              {\em Monte Carlo methods\/}
              (Methuen \& Co Ltd, London 1965)

 \bibitem{Bin}
              K.\,Binder,
              {\em Monte Carlo investigations of phase transitions and
                   critical phenomena\/},
              in: Phase transitions and critical phenomena, Vol.5b,
                  eds.\ C.\,Domb, M.S.\,Green
              (Academic Press, New York, 1976);

              K.\,Binder (ed.),
              {\em Monte Carlo methods in statistical physics\/},
              Topics in Current Physics 7, second edition
              (Springer-Verlag, Berlin, 1986);

              K.\,Binder (ed.),
              {\em Applications of the Monte Carlo method in statistical
                   physics\/},
               Topics in Current Physics 36, second edition
              (Springer-Verlag, Berlin, 1987)

 \bibitem{CreJacReb}
              M.\,Creutz, L.\,Jacobs, and C.\,Rebbi,
              {\em Monte Carlo computations in lattice gauge
                   theories\/},
              Phys. Rep. 95 (1983) 201

 \bibitem{Hee}
              D.W.\,Heermann,
              {\em Computer simulation methods in theoretical physics\/}
              (Springer-Verlag, Berlin, 1986)

 \bibitem{Reb}
              C.\,Rebbi,
              {\em Lattice gauge theories and Monte Carlo simulations\/}
              (World Scientific, Singapore, 1983)

 \bibitem{KogSpin}
              J.B.\,Kogut,
              {\em An introduction to lattice gauge theory
                   and spin systems\/},
              Rev. Mod. Phys. 51 (1979) 659

 \bibitem{KogQCD}
              J.B.\,Kogut,
              {\em The lattice gauge theory approach to quantum
                   chromodynamics\/},
              Rev. Mod. Phys. 55 (1983) 775

 \bibitem{CreBook}
              M.\,Creutz,
              {\em Quarks, gluons and lattices\/}
              (Cambridge University Press, Cambridge, 1983)

 \bibitem{Rot}
              H.J.\,Rothe,
              {\em Lattice gauge theories\/}
              (World Scientific, Singapore, 1992)

 \bibitem{SweWan}
              R.H.\,Swendsen and J.-S.\,Wang,
              {\em Nonuniversal critical
                   dynamics in Monte Carlo simulations\/},
              Phys. Rev. Lett. 58 (1987) 86

 \bibitem {Isi}
              E.\,Ising,
              {\em Beitrag zur Theorie des Ferromagnetismus\/},
              Z. Phys. 31 (1925) 253

 \bibitem {Wol}
              U.\,Wolff,
              {\em Collective Monte Carlo Updating for Spin Systems\/},
              Phys. Rev. Lett. 62 (1989) 361

 \bibitem {Has}
              M.\,Hasenbusch,
              {\em Improved estimators for a cluster updating of
                   $O(N)$ spin models\/},
              Nucl. Phys. B333 (1990) 581

 \bibitem{ClusterReviews}
              U.\,Wolff,
              {\em Critical slowing down\/},
              Nucl. Phys. B (Proc. Suppl.) 17 (1990) 93;

              A.D.\,Sokal,
              {\em How to beat critical slowing down: 1990 update\/},
              Nucl. Phys. B (Proc. Suppl.) 20 (1991) 55

 \bibitem{Par}
              G.\,Parisi,
              {\em Prolegomena to any future computer evaluation of
                   the QCD mass spectrum\/},
              Carg\`{e}se 1983,
              in: Progress in gauge field theory,
              eds.\ G.\,'t Hooft et al.\
              (Plenum Press, New York, 1984)

 \bibitem{HMO}
              H.\,Meyer-Ortmanns,
              {\em Proposal of a new upgrading procedure for Monte
                   Carlo experiments\/},
              Z. Phys. C27 (1985) 553

 \bibitem{GooSok}
              J.\,Goodman and A.D.\,Sokal,
              {\em Multigrid Monte Carlo for lattice field theories\/},
              Phys. Rev. Lett. 56 (1986) 1015

 \bibitem{HSVGSP}
              A.\,Hulsebos, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid Monte Carlo in an external $U(1)$
                   gauge field\/},
              Nucl. Phys. B (Proc. Suppl.) 9 (1989) 512;

              A.\,Hulsebos, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid Monte Carlo for a Bose field
                   in an external gauge field\/},
              Nucl. Phys. B331 (1990) 531

 \bibitem{HSVXY}
              A.\,Hulsebos, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid method for the 2-$D$ $XY$ model\/},
              Nucl. Phys. B (Proc. Suppl.) 17 (1990) 354;

              A.\,Hulsebos, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid simulation of the $XY$ model\/},
              Nucl. Phys. B356 (1991) 775

 \bibitem{GooSokSeries}
              R.G.\,Edwards, J.\,Goodman, and A.D.\,Sokal,
              {\em Multigrid Monte Carlo.
                   2.\,Two-dimensional $XY$ model\/},
              Nucl. Phys. B354 (1991) 289;

              R.G.\,Edwards, S.J.\,Ferreira, J.\,Goodman, and
              A.D.\,Sokal,
              {\em Multigrid Monte Carlo.
                   3.\,Two-dimensional $O(4)$ symmetric nonlinear
                       $\sigma$-model\/},
              Nucl. Phys. B380 (1992) 621

 \bibitem{LauVin}
              M.L.\,Laursen, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid updating of $U(1)$ gauge fields},
             Phys. Lett. B262 (1991) 467;

              M.L.\,Laursen and J.C.\,Vink,
              {\em Multigrid updating of compact $U(1)$ gauge fields
                   in 4 dimensions\/},
              KFA J\"ulich preprint HLRZ--92--14 (March 1992)

 \bibitem{MacCargese}
              G.\,Mack,
              {\em Multigrid methods in quantum field theory\/},
              Carg\`{e}se 1987,
              in: Nonperturbative quantum field theory,
              eds.\ G.\,'t Hooft et al.\
              (Plenum Press, New York, 1988)

 \bibitem {WilKog}
              K.G.\,Wilson,
              {\em Renormalization group and strong interactions\/},
              Phys. Rev. D3 (1971) 1818;

              K.G.\,Wilson and J.\,Kogut,
              {\em The renormalization group and the $\varepsilon$
              expansion\/},
              Phys. Rep. 12C (1974) 75;

              K.G.\,Wilson,
              {\em The renormalization group and critical phenomena\/},
              Rev. Mod. Phys. 55 (1983) 583

 \bibitem {Ami}
              D.J.\,Amit,
              {\em Field theory, the renormalization group and
                   critical phenomena\/}
              (World Scientific, Singapore, 1984)

 \bibitem {Binetal}
              J.J.\,Binney, N.J.\,Dowrick, A.J.\,Fisher, and
              M.E.J.\,Newman,
              {\em The theory of critical phenomena.
                   An introduction to the renormalization group\/}
              (Clarendon Press, Oxford, 1992)

 \bibitem{GruKun}
              C.\,Gruber and H.\,Kunz,
              {\em General properties of polymer systems\/},
              Commun. Math. Phys. 22 (1971) 133

 \bibitem{MacRGandME}
              G.\,Mack,
              {\em Renormalization group and Mayer expansions\/},
              Carg\`{e}se 1983,
              in: Progress in gauge field theory,
              eds.\ G.\,'t Hooft et al.\
              (Plenum Press, New York, 1984)

 \bibitem{MacPor}
              G.\,Mack and A.\,Pordt,
              {\em Convergent perturbation expansions for Euclidean
                   quantum field theory\/},
              Commun. Math. Phys. 97 (1985) 267

 \bibitem{MacMey}
              G.\,Mack and S.\,Meyer,
              {\em The effective action from multigrid Monte Carlo\/},
              Nucl. Phys. B (Proc. Suppl.) 17 (1990) 293

 \bibitem{Pal}
              G.\,Palma,
              {\em Finite size scaling analysis of the constraint
                   effective potential computed from multigrid
                   Monte Carlo\/},
              preprint DESY 90--083 (July 1990);

              G.\,Palma,
              {\em Renormalized loop expansion to compute finite size
                   effects of the constraint effective potential\/},
              Z. Phys. C54 (1992) 679;

              G.\,Palma,
              {\em Renormalized loop expansion for the gauge covariant
                   constraint effective Higgs potential on the
                   lattice\/},
              Ph.\,D.\ thesis and preprint DESY 92--031 (February 1990)

 \bibitem{HasMeyMac}
              M.\,Hasenbusch, S.\,Meyer, and G.\,Mack,
              {\em Noncritical multigrid Monte Carlo:
                   $O(3)$ non-linear $\sigma$ model\/},
              Nucl. Phys. B (Proc. Suppl.) 20 (1991) 110

 \bibitem{HasMey}
              M.\,Hasenbusch and S.\,Meyer,
              {\em Multigrid acceleration for asymptotically free
                   theories\/},
              Phys. Rev. Lett. 68 (1992) 435;

              M.\,Hasenbusch and S.\,Meyer,
              {\em Multigrid acceleration for asymptotically free
                   theories\/},
              Nucl. Phys. B (Proc. Suppl.) 26 (1992) 610;

              M.\,Hasenbusch and S.\,Meyer,
              {\em Testing accelerated algorithms in the lattice
                   $CP^3$ model\/},
              Phys. Rev. D45 (1992) 4376

 \bibitem{MacPin}
              G.\,Mack and K.\,Pinn:
              {\em A Monte Carlo procedure for Hamiltonians with
                   small nonlocal correction terms\/},
              Phys. Lett. B173 (1986) 434

 \bibitem{KalDiplom}
              T.\,Kalkreuter,
              {\em Simulation von Gitterfeldtheorien
                   mit Hilfe der Polymermethode\/},
              Di\-plo\-ma the\-sis, Universit\"at Hamburg (April 1989)

\bibitem {SymImprovedAction}
              K.\,Symanzik,
              {\em Continuum limit and improved action in lattice
                   theories, (I.) Principles and $\phi^4$-theory\/},
              Nucl. Phys. B226 (1983) 187;

              K.\,Symanzik,
              {\em Continuum limit and improved action in lattice
                   theories, (II.) O(N) non-linear sigma model in
                   perturbation theory\/},
              Nucl. Phys. B226 (1983) 205

 \bibitem{KalNP1}
              T.\,Kalkreuter,
              {\em Simulation of statistical systems with not
                   necessarily real and positive probabilities\/},
              Nucl. Phys. B352 (1991) 251

 \bibitem{Mon}
              I.\,Montvay,
              {\em Simulation of staggered fermions by polymer
                   averaging\/},
              Phys. Lett. B227 (1989) 260;

              I.\,Montvay,
              {\em Simulation of staggered fermions by polymer
                   algorithms\/},
              Carg\`{e}se 1989, in:
              P.H.\,Damgaard et al.\ (eds.), Probabilistic methods in
              quantum field theory and quantum gravity
              (Plenum Press, New York, 1990)

 \bibitem{Wei}
              D.\,Weingarten,
              {\em Monte Carlo algorithms for QCD\/},
              Nucl. Phys. B (Proc. Suppl.) 9 (1989) 447

 \bibitem{TouLAT91}
              D.\,Touissaint,
              {\em The QCD spectrum and phase diagram on the
                   lattice -- 1991\/},
              Nucl. Phys. B (Proc. Suppl.) 26 (1992) 3

 \bibitem{HybridMC}
              S.\,Duane, A.D.\,Kennedy, B.J.\,Pendleton,
              and D.\,Roweth,
              {\em Hybrid Monte Carlo\/},
              Phys. Lett. B195 (1987) 216;

              A.D.\,Kennedy,
              {\em Higher order Hybrid Monte Carlo\/},
              Nucl. Phys. B (Proc. Suppl.) 9 (1989) 457;

              A.D.\,Kennedy,
              {\em The theory of hybrid stochastic algorithms\/},
              Carg\`{e}se 1989,
              in: Probabilistic methods in quantum field theory and
                  quantum gravity,
              eds.\ P.H.\,Damgaard et al.
              (Plenum Press, New York, 1990)

 \bibitem{Sha}
              S.R.\,Sharpe,
              {\em Lattice QCD: Going beyond the mass spectrum\/},
              J. Stat. Phys. 43 (1986) 1129

 \bibitem{BraLAT91}
              A.\,Brandt,
              {\em Multigrid Methods in Lattice Field Computations\/},
              Nucl. Phys. B (Proc. Suppl.) 26 (1992) 137

 \bibitem{BroMorMyeReb}
              R.C.\,Brower, K.J.M.\,Moriarty, E.\,Myers, and C.\,Rebbi,
              {\em The multigrid method for fermion calculations
                   in quantum chromodynamics\/},
             %Princeton preprint 87--0335
              in: Multigrid Methods, ed.\ S.F.\,McCor\-mick
              (Marcel Dekker, New York, 1988)

 \bibitem{WilsonFermions}
              K.G.\,Wilson,
              {\em Quarks and strings on a lattice\/},
              Erice 1975,
              in: New phenomena in subnuclear physics,
              ed.\ A.\,Zichichi
              (Plenum Press, New York, 1977)

 \bibitem{NieNin}
              H.B.\,Nielsen and M.\,Ninomiya,
              {\em Absence of neutrinos on a lattice.
                   (I).\ Proof by homotopy theory\/},
              Nucl. Phys. B185 (1981) 20,\
              Errata ibid.\ B195 (1982) 541;\

              H.B.\,Nielsen and M.\,Ninomiya,
              {\em Absence of neutrinos on a lattice.
                   (II).\ Intuitive topological proof\/},
              Nucl. Phys. B193 (1981) 173;\

              H.B.\,Nielsen and M.\,Ninomiya,
              {\em A no-go theorem for regularizing chiral fermions\/},
              Phys. Lett. B105 (1981) 219;\

              L.H.\,Karsten,
              {\em Lattice fermions in Euclidean space-time\/},
              Phys. Lett. B104 (1981) 315

 \bibitem{SmiReviews}
              J.\,Smit,
              {\em Fermions on a lattice\/},
              Acta Phys. Pol. B17 (1986) 531;

              J.\,Smit,
              {\em Attempts to put the standard model on the lattice\/},
              Nucl. Phys. B (Proc. Suppl.) 4 (1988) 451;

              J.\,Smit,
              {\em Standard model and chiral gauge theories on the
                   lattice\/},
              Nucl. Phys. B (Proc. Suppl.) 17 (1990) 3

 \bibitem{KogSus}
              J.\,Kogut and L.\,Susskind,
              {\em Hamiltonian formulation of Wilson's lattice gauge
                   theory\/},
              Phys. Rev. D11 (1975) 395

 \bibitem{BanSusKog}
              T.\,Banks, L.\,Susskind, and J.\,Kogut,
              {\em Strong-coupling calculations of lattice gauge
                   theories: (1+1) dimensional exercise\/},
              Phys. Rev. D13 (1976) 1043

 \bibitem{Sus}
              L.\,Susskind,
              {\em Lattice fermions\/},
              Phys. Rev. D16 (1977) 3031

 \bibitem{ShaThuWei}
              H.\,Sharatchandra, H.\,Thun, and P.\,Weisz,
              {\em Susskind fermions on a Euclidean lattice\/},
              Nucl. Phys. B192 (1981) 205

 \bibitem{KluMorNapPet}
              H.\,Kluberg-Stern, A.\,Morel, O.\,Napoly, and
              P.\,Petersson,
              {\em Flavours of Lagrangian Susskind fermions\/},
              Nucl. Phys. B220 [FS8] (1983) 447

 \bibitem{BecJoo}
              P.\,Becher and H.\,Joos,
              {\em The Dirac-K\"ahler equation and fermions on the
              lattice\/},
              Z. Phys. C15 (1982) 343

 \bibitem{Oya}
              Y.\,Oyanagi,
              {\em An incomplete LDU decomposition of lattice fermions
                   and its application to conjugate reidual methods\/},
              Comput. Phys. Commun. 42 (1986) 333

 \bibitem{RosDavLep}
              P.\,Rossi, C.T.H.\,Davies, and G.P.\,Lepage,
              {\em A comparison of a variety of matrix inversion
                   algorithms for Wilson fermions on the lattice\/},
              Nucl. Phys. B297 (1988) 287

 \bibitem{DeGra}
              T.A.\,DeGrand,
              {\em A conditioning technique for matrix inversion for
                   Wilson fermions\/},
              Comput. Phys. Commun. 52 (1988) 161

 \bibitem {FFT}
              G.\,Katz, G.\,Batrouni, C.\,Davies, A.\,Kronfeld,
              P.\,Lepage, P.\,Rossi, B.\,Svetitsky, and K.\,Wilson,
              {\em Fourier acceleration in lattice gauge theories.
                   II.\,Matrix inversion and the quark propagator},
              Phys. Rev. D37 (1988) 1589

 \bibitem{RosDav}
              P.\,Rossi and C.T.H.\,Davies,
              {\em A comment on an attempt to Fourier accelerate
                   Kogut-Susskind fermions\/},
              Phys. Lett. B202 (1988) 547

 \bibitem{EdwGooSok}
              R.G.\,Edwards, J.\,Goodman and A.D.\,Sokal,
              {\em Multigrid method for the random resistor problem\/},
              Phys. Rev. Lett. 61 (1988) 1333;

              R.G.\,Edwards, J.\,Goodman and A.D.\,Sokal,
              {\em Algebraic Multi-grid method for disordered
                   systems\/},
              Nucl. Phys. B (Proc. Suppl.) 9 (1989) 521

\bibitem{Edw}
              R.G.\,Edwards,
              {\em Numerical simulations in lattice gauge theories
                   and statistical mechanics\/},
              Ph.\,D.\ thesis, New York University (June 1989)

 \bibitem{BenBraSol}
              R.\,Ben-Av, A.\,Brandt, and S.\,Solomon,
              {\em The fermionic matrix, instantons, zero modes
                   and multigrid\/},
              Nucl. Phys. B329 (1990) 193

 \bibitem{HSVLAT90}
              A.\,Hulsebos, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid inversion of the staggered fermion
                   matrix\/},
              Nucl. Phys. B (Proc. Suppl.) 20 (1991) 94

 \bibitem{BRVGSP}
              R.C.\,Brower, C.\,Rebbi, and E.\,Vicari,
              {\em Projective multigrid method for propagators in
                   lattice gauge theory\/},
              Phys. Rev. D43 (1991) 1965

 \bibitem{MacUnpublished}
              G.\,Mack, {\em unpublished\/}

 \bibitem{GawKup}
              K.\,\Gaw and A.\,Kupiainen,
              {\em A rigorous block spin approach to massless lattice
              theories\/},
              Commun. Math. Phys. 77 (1980) 31;\

              K.\,\Gaw and A.\,Kupiainen,
              {\em Massless lattice $\phi_4^4$ theory: Rigorous control
              of a renormalizable asymptotically free model\/},
              Commun. Math. Phys. 99 (1985) 197

 \bibitem{MacKen}
              P.B.\,Mackenzie,
              {\em Critique of practical methods for computer
                   evaluation of the hadron spectrum\/},
              Nucl. Phys. B (Proc. Suppl.) 17 (1990) 103

 \bibitem{Bitetal}
              K.M.  Bitar, R.G.  Edwards, U.M.  Heller, A.D.  Kennedy,
              T.A.  DeGrand, S.  Gottlieb,  A.  Kras\-nitz, J.B.  Kogut,
              W.  Liu, P.  Rossi, M.C.  Ogilvie, R.L.  Renken,
              D.K.  Sinclair, R.L.  Sugar, D.  Toussaint,
              and K.C.  Wang,
              {\em Hadron spectrum in QCD with valence Wilson fermions
                   and dynamical staggered fermionsat $6/g^2 = 5.6$\/},
              Phys. Rev. D46 (1992) 2169

 \bibitem{GooSokReview}
              J.\,Goodman and A.D.\,Sokal,
              {\em Multigrid Monte Carlo method. Conceptual
                   foundations\/},
              Phys. Rev. D40 (1989) 2035

 \bibitem{Var}
              R.S.\,Varga,
              {\em Matrix iterative analysis\/},
              (Prentice-Hall, Inc.\,, Englewood Cliffs, NJ, 1962)

 \bibitem{You}
              D.M.\,Young,
              {\em Iterative solution of large linear systems\/}
              (Academic Press, New York, 1971)

 \bibitem{StoBul}
              J.\,Stoer and R.\,Bulirsch,
              {\em Einf\"uhrung in die Numerische Mathematik II\/}
              (Springer-Verlag, Berlin, 1978)

 \bibitem{GolLoa}
              G.H.\,Golub and C.F.\,v.\,Loan,
              {\em Matrix computations\/}, second edition,
              (The Johns Hopkins University Press, Baltimore, 1990)

 \bibitem{HacLGS}
              W.\,Hackbusch,
              {\em Iterative L\"osung gro\3er schwachbesetzter
              Gleichungssysteme\/}
              (B.\ G.\ Teubner, Stuttgart, 1991)

 \bibitem{ChaKenRow}
              C.B.\,Chalmers, R.D.\,Kenway, and D.\,Roweth,
              {\em Algorithms for calculating quark propagators
                   on large lattices\/},
              J. Comp. Phys. 70 (1987) 500

 \bibitem{HenSetDav}
              D.\,Henty, R.\,Setoodeh, and C.T.H.\,Davies,
              {\em A study of block algorithms for fermions matrix
                   inversion\/},
              Nucl. Phys. B337 (1990) 487

 \bibitem{BurIrv}
              A.N.\,Burkitt and A.C.\,Irving,
              {\em Inversion of the fermion matrix and the equivalence
                   of the conjugate gradient and Lanczos algorithms\/},
              Comput. Phys. Commun. 59 (1990) 447

 \bibitem{KenJulich}
              A.D.\,Kennedy,
              {\em Hybrid Monte Carlo algorithm on the connection
                   machine\/},
              Int. J. Mod. Phys. C3 (1992) 1

 \bibitem{TFproject}
              S.  Aoki, R.  Shrock, B.  Berg, C.  Bernard, M.  Ogilvie,
              D.  Petcher, G.  Bhanot, P.  Rossi, K.  Bitar,
              R.  Edwards, U.M.  Heller, A.  Kennedy, S.  Sanielevici,
              R.  Brower, J.  Potvin, C.  Rebbi, F.R.  Brown,
              N.  Christ, R.  Mawhinney, C.  Detar, T.  Draper,
              K.-F.  Liu, S.  Gottlieb, H.  Hamber, G.  Kilcup,
              J.  Shigemitsu, J.  Kogut, A.  Kronfeld, I.-H.  Lee,
              J.  Negele, S.  Ohta, J.C.  Sexton, E.  Shuryak,
              D.K.  Sinclair, A.  Soni, and W.  Wilcox,
              {\em Physics goals of the QCD teraflop project\/},
              Int. J. Mod. Phys. C2 (1991) 829

 \bibitem{Columbia}
              F.R.\,Brown, H.\,Chen, N.H.\,Christ, Z.\,Dong,
              R.D.\,Mawhinney, W.\,Schaffer, and A.\,Vaccarino,
              {\em Lattice QCD with 8 light quark flavors\/},
              Columbia University preprint CU--TP--541 (May 1992)

 \bibitem{UKQCD}
              C.R.  Allton, H.  Duong, C.T.  Sachrajda, I.M.  Barbour,
              A.  Bell, C.T.H.  Davies, S.J.  Hands, E.  Klepfish,
              R.M.  Baxter, S.P.  Booth, K.C.  Bowler, S.  Collins,
              D.S.  Henty, R.D.  Kenway, C.  McNeile, B.J.  Pendleton,
              D.G.  Richards, J.N.  Simone, A.D.  Simpson, B.E.  Wilkes,
              J.E.J.  Bottomley, S.M.  Catterall, F.R.  Devlin,
              I.T.  Drummond, R.R.  Horgan, K.  Decker, A.  Hulsebos,
              A.C.  Irving, A.  McKerrell, C.  Michael, M.  Prisznyak,
              P.W.  Stephenson, G.  Martinelli, M.  Teper, and
              J.F.  Wheater,
              {\em First results from the UKQCD collaboration\/},
              Nucl. Phys. B (Proc. Suppl.) 26 (1992) 211

 \bibitem{Pol}
              E.\,Polak,
              {\em Computational methods in optimization\/}
              (Academic Press, New York, 1971)

 \bibitem{Preetal}
              W.H.\,Press, B.P.\,Flannery, S.A.\,Teukolsky, and
              W.T.\,Vetterling,
              {\em Numerical recipes\/}
              (Cambridge University Press, Cambridge, 1986)

 \bibitem{WilRei}
              J.H.\,Wilkinson and C.\,Reinsch,
              {\em Linear algebra\/}
              (Springer-Verlag, Berlin, 1971)

 \bibitem{MGclassical}
              A.\,Brandt,
              {\em Multi-level adaptive solutions to boundary-value
                   problems\/},
              Math. Comput. 31 (1977) 333;\

              K.\,St\"uben and U.\,Trottenberg,
              {\em Multigrid methods: fundamental algorithms,
                   model problem analysis and applications\/},
              in: Multigrid methods,
                  Lecture Notes in Mathematics 960,
              eds.\ W.\,Hackbusch and U.\,Trottenberg
              (Springer-Verlag, Berlin, 1982);\

              A.\,Brandt,
              {\em Multigrid techniques: 1984 guide
                   with applications to Fluid Dynamics\/},
              GMD-Studie No.\ 85

 \bibitem{HacMG}
              W.\,Hackbusch,
              {\em Multi-grid methods and applications\/},
              Springer Series in Computational Mathematics 4
              (Springer-Verlag, Berlin, 1985)

 \bibitem{McCor}
              S.F.\,McCormick,
              {\em Multilevel adaptive methods for partial differential
                   equations\/}
              (SIAM, Phi\-la\-delphia, 1989)

 \bibitem{Bri}
              W.L.\,Briggs,
              {\em A multigrid tutorial\/}
              (SIAM, Philadelphia, 1987)

 \bibitem{GawKupLH}
              K.\,\Gaw and A.\,Kupiainen,
              {\em Asymptotic freedom beyond perturbation theory\/},
              in: Critical phenomena, random systems, gauge theories,
              Les Houches 1984,
              eds.\ K.\,Osterwalder and R.\,Stora
              (North Holland, Amsterdam, 1986)

 \bibitem{HaretalLAT90}
              M.\,Harmatz, P.G.\,Lauwers, R.\,Ben-Av, A.\,Brandt,
              E.\,Katznelson, S.\,So\-lo\-mon, and  K.\,Wo\-lo\-wes\-ky,
              {\em Parallel-transported multigrid and its application
                   to the Schwinger model\/},
              Nucl. Phys. B (Proc. Suppl.) 20 (1991) 102

 \bibitem{Benthesis}
              R.\,Ben-Av,
              {\em Acceleration methods in MC simulations\/},
              Ph.\,D.\ thesis, The Weizmann Institute of Science
              (October 1991)

 \bibitem{PTMG_GMD}
              R.\,Ben-Av, M.\,Harmatz, P.G.\,Lauwers, and
              S.\,So\-lo\-mon,
              {\em Parallel-transported multigrid for inverting the
                   Dirac-operator: Variants of the method and their
                   efficiency\/},
              Arbeitspapiere der GMD~674 (August 1992)

 \bibitem{MacDLGT}
              G.\,Mack,
              {\em Dielectric lattice gauge theory\/},
              Nucl. Phys. B235 [FS11] (1984) 197

 \bibitem{BalProp}
              T.\,Ba{\l}aban,
              {\em Regularity and decay of lattice Green's functions\/},
              Commun. Math. Phys. 89 (1983) 571

 \bibitem{KalNP2}
              T.\,Kalkreuter,
              {\em Projective block spin transformations in
                   lattice gauge theory\/},
              Nucl. Phys. B376 (1992) 637

 \bibitem{KalLastPoint}
              T.\,Kalkreuter,
              {\em Improving multigrid and conventional relaxation
                   algorithms for propagators\/},
              preprint DESY 92--108 (July 1992),
              to appear in Int. J. Mod. Phys. C

 \bibitem{HSVNP}
              A.\,Hulsebos, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid inversion of lattice fermion operators\/},
              Nucl. Phys. B368 (1992) 379

 \bibitem{HSVJulich}
              A.\,Hulsebos, J.\,Smit, and J.C.\,Vink,
              {\em Multigrid inversion of the staggered fermion matrix
                   with $U(1)$ and $SU(2)$ gauge fields\/},
              Int. J. Mod. Phys. C3 (1992) 161

 \bibitem{Vin}
              J.C.\,Vink,
              {\em Multigrid inversion of staggered and Wilson fermion
               operators with $SU(2)$ gauge fields in two dimensions\/},
              Phys. Lett. B272 (1991) 81

 \bibitem{VinLAT91}
              J.C.\,Vink,
              {\em Multigrid inversion of fermion operators with $SU(2)$
                   gauge fields in two and four dimensions\/},
              Nucl. Phys. B (Proc. Suppl.) 26 (1992) 607

 \bibitem{BRVvariational}
              R.C.\,Brower, C.\,Rebbi, and E.\,Vicari,
              {\em Non-Abelian projective multigrid for
                   lattice gauge theory\/},
              Phys. Rev. Lett. 66 (1991) 1263;\

              R.C.\,Brower, K.J.M.\,Moriarty, C.\,Rebbi, and E.\,Vicari,
              {\em Variational multigrid for non-Abelian gauge
                   theory\/},
              Nucl. Phys. B (Proc. Suppl.) 20 (1991) 89

 \bibitem{KalMacSpe}
              T.\,Kalkreuter, G.\,Mack, and M.\,Speh,
              {\em Blockspin and multigrid for staggered fermions
                   in non-Abelian gauge fields\/},
              Int. J. Mod. Phys. C3 (1992) 121

 \bibitem{AshMer}
              N.W.\,Ashcroft and N.D.\,Mermin,
              {\em Solid state physics\/}
              (Holt-Saunders  Int.\ Ed.\,, Tokyo, 1976)

 \bibitem{JooSch}
              H.\,Joos and M.\,Schaefer,
              {\em The representation theory of the symmetry group of
              lattice fermions as a basis for kinematics in lattice
              QCD\/},
              Z. Phys. C34 (1987) 465

 \bibitem{Gol}
              M.F.L.\,Golterman,
              {\em Irreducible representations
                   of the staggered fermion symmetry group\/},
              Nucl. Phys. B278 (1986) 417

 \bibitem{Mai}
              G.\,Mai,
              {\em Ein Blockspin f\"ur $2^{d/2}$ Fermionen\/},
              Di\-plo\-ma the\-sis, Universit\"at Hamburg (October 1989)

 \bibitem{Benetal}
              R.\,Ben-Av, A.\,Brandt, M.\,Harmatz, E.\,Katznelson,
              P.G.\,Lauwers, S.\,So\-lo\-mon, and  K.\,Wo\-lo\-wes\-ky,
              {\em Fermion simulations using parallel transported
                   multigrid\/},
              Phys. Lett. B253 (1991) 185;

              P.G.\,Lauwers, R.\,Ben-Av, and S.\,So\-lo\-mon,
              {\em Inverting the Dirac matrix for $SU(2)$ lattice gauge
                   theory by means of parallel-transported multigrid\/},
              Nucl. Phys. B374 (1992) 249;

              S.\,So\-lo\-mon and P.G.\,Lauwers,
              {\em Parallel transported multigrid beats conjugate
                   gradient\/},
              Int. J. Mod. Phys. C3 (1992) 149

 \bibitem{LauWit}
              P.G.\,Lauwers and T.\,Wittlich,
              {\em Inversion of the fermion matrix in lattice QCD by
                   means of parallel-transported multigrid (PTMG)\/},
              preprint BONN 92--29 (September 1992);

              P.G.\,Lauwers and T.\,Wittlich,
              {\em Parallel-transported multigrid (PTMG) for
                   inverting the Dirac-operator in $SU(3)$
                   lattice gauge theory\/},
              to appear in Nucl. Phys. B (Proc. Suppl.) (LATTICE 92)

 \bibitem{BalLGT}
              T.\,Ba{\l}aban,
              {\em Propagators and renormalization transformations
                   for lattice gauge theories. I\/},
              Commun. Math. Phys. 95 (1984) 17;

              T.\,Ba{\l}aban,
              {\em Averaging operations for lattice gauge theories\/},
              Commun. Math. Phys. 98 (1985) 17;

              T.\,Ba{\l}aban,
              {\em Renormalization group approach to lattice gauge field
              theories: I.\ Generation of effective actions in a small
              field approximation and a coupling constant
              renormalization in four dimensions\/},
              Commun. Math. Phys. 109 (1987) 249

 \bibitem{BalJaf}
              T.\,Ba{\l}aban and A.\,Jaffe,
              {\em Constructive gauge theory\/},
              Erice 1985,
              in: Fundamental problems of gauge field theory,
              eds.\ G.\,Velo and A.S.\,Wightman
              (Plenum Press, New York, 1986)

 \bibitem{Wig}
              A.S.\,Wightman,
              {\em Constructive quantum field theory from I to II.
                   Remarks on what we have learned\/},
              in: Constructive quantum field theory II,
              eds.\ G.\,Velo and A.S.\,Wightman,
              Erice 1988
              (Plenum Press, New York, 1990)

 \bibitem{Imb}
              J.\,Imbrie,
              {\em Renormalization group methods in gauge field
                   theories\/},
              in: Critical phenomena, random systems, gauge theories,
              Les Houches 1984,
              eds.\ K.\,Osterwalder and R.\,Stora
              (North Holland, Amsterdam, 1986)

 \bibitem{Riv}
              V.\,Rivasseau,
              {\em From perturbative to constructive renormalization\/},
              Princeton Series in Physics
              (Princeton University Press, Princeton, 1991)

 \bibitem{ColEWA}
              L.\,Collatz,
              {\em Eigenwertaufgaben mit technischen Anwendungen\/}
              (Akademische Verlagsge\-sell\-schaft, Leipzig, 1963)

 \bibitem{ColFA}
              L.\,Collatz,
              {\em Funktionalanalysis und Numerische Mathematik\/}
              (Springer-Verlag, Berlin, 1964)

 \bibitem{CouHil}
              R.\,Courant and D.\,Hilbert,
              {\em Methoden der Mathematischen Physik I\/}
              (Springer-Verlag, Berlin, 1968)

 \bibitem{CreHB}
              M.\,Creutz,
              {\em Monte Carlo study of quantized $SU(2)$ gauge
                   theory\/},
              Phys. Rev. D21 (1980) 2308

 \bibitem{NAGLIB}
              NAGLIB, Numerical Algorithms Group, NAG Fortran
              (Vector) Library, Mark 13

 \bibitem{UniRechner}
              SIEMENS 7.\,882, Regionales Rechenzentrum der
              Universit\"at Hamburg

 \bibitem{DESYIBM}
              IBM 3084 Q, IBM 3090--150E,
              IBM ES 9000/720 VF (IBM 9021),
              DESY-Rechenzentrum

 \bibitem{CrePlaquette}
              M.\,Creutz,
              {\em Confinement and the critical dimensionality
                   of space-time\/},
              Phys. Rev. Lett. 43 (1979) 553

 \bibitem{CRAY}
              CRAY Y--MP8/832, HLRZ at KFA J\"ulich

 \bibitem{Pir}
              H.J.\,Pirner, J.\,Wroldsen, and M.\,Ilgenfritz,
              {\em Construction of an effective colour dielectric
                   lattice action from QCD by blocking\/},
              Nucl. Phys. B294 (1987) 905;

              H.J.\,Pirner,
              {\em Confinement in the color dielectric model\/},
              Nucl. Phys. B (Proc. Suppl.) 15 (1990) 207;

              B.\,Gro\3mann, H.J.\,Pirner, A.I.\,Signal, R.\,Baier, and
              J.\,Wroldsen,
              {\em Searching for an optimal lattice color dielectric
                   theory\/},
              Int. J. Mod. Phys. A6 (1991) 2649;

              B.\,Gro\3mann, H.J.\,Pirner, and J.\,Wroldsen,
              {\em Phase structure of $SU(2)$ lattice gauge theory
                   with fluctuating coupling\/},
              Nucl. Phys. B377 (1992) 424;

              H.J.\,Pirner,
              {\em The color dielectric model of QCD\/},
              Prog. Part. Nucl. Phys. 29 (1992) 33

 \bibitem{CalPet}
              D.J.E.\,Callaway and R.\,Petronzio,
              {\em Monte Carlo renormalization group trajectories
                   in lattice gauge theories\/},
              Phys. Lett. B145 (1984) 381

 \bibitem{PatGup}
              A.\,Patel and R.\,Gupta,
              {\em Monte Carlo renormalization group investigations
                   of the $SU(2)$ lattice gauge theory\/},
              Nucl. Phys. B251 [FS13] (1985) 789

 \bibitem{KalPL}
              T.\,Kalkreuter,
              {\em Ground-state projection multigrid for propagators
                   in four-dimensional $SU(2)$ gauge fields\/},
              Phys. Lett. B276 (1992) 485

 \bibitem{MacKalPalSpe}
              G.\,Mack, T.\,Kalkreuter, G.\,Palma, and M.\,Speh,
              {\em Effective Field Theories\/},
              preprint DESY 92--070 (May 1992),
              to appear in the proceedings of the 31st IUKT,
              Schladming, February 1992

 \bibitem{BaeKalMacSpe}
              M.\,B\"aker, T.\,Kalkreuter, G.\,Mack, and M.\,Speh,
              {\em Neural multigrid for gauge theories and other
                   disordered systems\/},
              preprint DESY 92--126 (September 1992),
              to appear in the proceedings of the 4th International
              Conference on Computational Physics PC92,
              Prague, August 1992

 \bibitem{HerKroPal}
              J.\,Hertz, A.\,Krogh, and R.G.\,Palmer,
              {\em Introduction to the theory of neural computation\/}
              (Addison-Wesley, Redwood City CA, 1991)

 \bibitem{MacSpe}
              G.\,Mack and M.\,Speh,
              {\em in preparation\/}

 \bibitem{Bae}
              M.\,B\"aker, Diploma thesis,
              {\em in preparation\/}

 \bibitem{BMRV}
              R.C.\,Brower, K.J.M.\,Moriarty, C.\,Rebbi, and E.\,Vicari,
              {\em Multigrid propagators in the presence of
                   disordered $U(1)$ gauge fields\/},
              Phys. Rev. D43 (1991) 1974

 \bibitem{Vya}
              V.\,Vyas,
              {\em A multigrid algorithm for calculating fermionic
                   propagators using Migdal-Kadanoff transformation\/},
              Wuppertal preprint WUB 91--10 (February 1991);

              V.\,Vyas,
              {\em Calculating the quark propagators using the
                   Migdal-Kadanoff transformation\/},
              Int. J. Mod. Phys. C3 (1992) 169

 \bibitem{BERV}
              R.C.\,Brower, R.G.\,Edwards, C.\,Rebbi, and E.\,Vicari,
              {\em Projective multigrid for Wilson fermions\/},
              Nucl. Phys. B366 (1991) 689

\bibitem{Hulthesis}
              A.\,Hulsebos,
              {\em Multigrid methods in quantum field theories\/},
              Ph.\,D.\ thesis, Universiteit van Amsterdam
              (September 1991)

 \bibitem{VyaSU3}
              V.\,Vyas,
              {\em An efficient algorithm for calculating the quark
                   propagators using Migdal-Kadanoff transformation\/},
              Wuppertal preprint WUB 92--30 (September 1992)

 \bibitem{BitetalLAT91}
              K.M.  Bitar, R.G.  Edwards, T.A.  DeGrand, S.  Gottlieb,
              U.M.  Heller, A.D.  Kennedy, J.B.  Kogut, A.  Krasnitz,
              W.  Liu, M.C.  Ogilvie, R.L.  Renken, D.K.  Sinclair,
              R.L.  Sugar, D.  Toussaint, and K.C.  Wang,
              {\em QCD hadron spectroscopy with staggered dynamical
                   quarks at $\beta =\,$5.6\/},
              Nucl. Phys. B (Proc. Suppl.) 26 (1992) 259

 \bibitem{deForGup}
              Ph.\,de Forcrand and R.\,Gupta,
              {\em Multigrid techniques for quark propagators\/},
              Nucl. Phys. B (Proc. Suppl.) 9 (1989) 516

 \bibitem{HulLauSmi}
              A.\,Hulsebos, M.L.\,Laursen, and J.\,Smit,
              {\em $SU(N)$ multigrid Landau gauge fixing\/},
              Phys. Lett. B291 (1992) 431

 \bibitem{GraPin}
              M.\,Grabenstein and K.\,Pinn,
              {\em Acceptance rates in multigrid Monte Carlo\/},
              Phys. Rev. D45 (1992) 4372;

              M.\,Grabenstein and K.\,Pinn,
              {\em Kinematics of multigrid Monte Carlo\/},
              preprint DESY 92--094 (July 1992)

 \bibitem{CorGupNov}
              R.\,Cordery, R.\,Gupta, and M.A.\,Novotny,
              {\em An improved renormalization group transformation
                   in four dimensions\/},
              Phys. Lett. B128 (1983) 425

 \bibitem{KalLeipzig}
              T.\,Kalkreuter,
              {\em Multigrid for staggered fermions in four-dimensional
                   $SU(2)$ gauge fields\/},
              talk presented at the DFG-Colloquium ``Dynamical
              Fermions'' held in Leipzig, March 1992

 \bibitem{KalLAT92}
              T.\,Kalkreuter,
              {\em Multigrid for propagators of staggered fermions
                   in four-dimensional $SU(2)$ gauge fields\/},
              to appear in Nucl. Phys. B (Proc. Suppl.) (LATTICE 92)

 \bibitem{Tim}
              H.-J.\,Timme,
              {\em Blockspintransformationen\/},
              unpublished (1987)

 \bibitem{GelSch}
              L.M.\,Gelfand and G.E.\,Schilow,
              {\em Verallgemeinerte Funktionen (Distributionen) I\/}
              (VEB Deut\-scher Verlag der Wissenschaften, Berlin, 1967)

 }

 \end{thebibliography}
 \end{singlespace}
 \clearpage
 \markboth{}{}
 \mbox{}

 \end{document}


